Studying distant galaxies: A Handbook of Methods and Analyses

Distant galaxies encapsulate the various stages of galaxy evolution and formation from over 95% of the development of the universe. As early as twenty-five years ago, little was known about them, however since the first systematic survey was completed in the 1990s, increasing amounts of resources have been devoted to their discovery and research. This book summarises for the first time the numerous techniques used for observing, analysing, and understanding the evolution and formation of these distant galaxies. In this rapidly expanding research field, this text is an every-day companion handbook for graduate students and active researchers. It provides guidelines in sample selection, imaging, integrated spectroscopy and 3D spectroscopy, which help to avoid the numerous pitfalls of observational and analysis techniques in use in extragalactic astronomy. It also paves the way for establishing relations between fundamental properties of distant galaxies. At each step, the reader is assisted with numerous practical examples and ready-to-use methodology to help understand and analyse research.

==> All_defglossary.tex <==
\newglossaryentry{Herschel}{name=Herschel, description={Herschel space
    telescope; IR and sub-mm 3.5m space telescope operated between
    2009 and 2013}}

\newglossaryentry{CANDELS}{name=CANDELS, description={Cosmic Assembly
    Near-infrared Deep Extragalactic Legacy Survey; Imaging survey
    conducted with the HST ACS and WFC3 cameras on several
    cosmological fields}}

\newglossaryentry{L*}{name=L*, description={Characteristic luminosity
    of the luminosity function at a given redshift; Luminosity
    describing the knee of the Luminosity Function, which corresponds
    to galaxies dominating the luminosity density at a given
    redshift}}

\newglossaryentry{GAMA}{name=GAMA, description={Galaxy And Mass
    \hbox{Assembly} survey; Spectroscopic survey of $\sim$300,000 galaxies
    carried out at the Anglo-Australian Telescope over 2008--2014}}

\newglossaryentry{PSF}{name=PSF, description={Point Spread Function;
    optical response of a system to a point-like source}}

\newglossaryentry{SMC}{name=SMC, description={Small Magellanic Cloud}}

\newglossaryentry{E-ELT}{name=E-ELT, description={European Extremely
    Large Telescope; Future ESO 39-meter telescope}}

\newglossaryentry{GSC}{name=GSC, description={Guide Star Catalog; also
    known as the Hubble Space Telescope, Guide Catalog}}

\newglossaryentry{QE}{name=QE, description={Quantum Efficiency;
    percentage of photons that are converted into charges by a
    detector}}

\newglossaryentry{FoV}{name=FoV, description={Field of View; solid
    angle through which a detector is sensitive to light}}

\newglossaryentry{HUDF}{name=HUDF, description={Hubble Ultra Deep
    Field; 2.4$\times$2.4 arcmin$^2$ region of the southern sky on
    which the deepest HST observations have been conducted}}

\newglossaryentry{WFPC2}{name=WFPC2, description={Wide Field and
    PLanetary Camera 2; Camera onboard the HST installed in 1993 and
    replaced in 2009 by the WFC3. This camera, which is sensitive to
    wavelengths from 120 to 1000\,nm, was used to image the Hubble
    Deep Field in 1995}}

\newglossaryentry{SPS}{name=SPS, description={Stellar Population
    Synthesis; set of methods and models used to compute the
    spectrophotometric properties of galaxies from those of the
    underlying stellar populations}}

\newglossaryentry{SSP}{name=SSP, description={Simple Stellar
    Population; theoretical population of stars used by Stellar
    Population Synthesis models assumed to be born at the same time
    from a single gas could according to a given IMF and having the
    same metallicity}}

\newglossaryentry{CSP}{name=CSP, description={Composite Stellar
    Population; Theoretical population of stars formed at different
    time and having different metallicities used by Stellar Population
    Synthesis models; Both ages and metallicities are usually obtained
    from the convolution of a Simple Stellar Population with a Star
    Formation History law}}

\newglossaryentry{ELT}{name=ELT, description={Extremely Large Telescope; Next-generation telescope with diameter larger than $\sim$20m}}

\newglossaryentry{MOS}{name=MOS, description={Multi-Object Spectrograph}}

\newglossaryentry{WiggleZ}{name=WiggleZ, description={WiggleZ Dark
    Energy Survey; large-scale galaxy redshift survey conducted
    between 2006 and 2011n which measured 240,000 galaxy redshifts
    over 1000 square degrees up to $z=1$}}

\newglossaryentry{BzK}{name=BzK, description={Distant galaxy selected based on
 $B-z$ and $z-K$ colors}}

\newglossaryentry{ERO}{name=ERO, description={Extremely Red Object}}

\newglossaryentry{JWST}{name=JWST, description={James Webb Space
    \hbox{Telescope}; 6.5m space telescope working between 0.6 and 28 $\mu$m
    to be launched in 2018}}

\newglossaryentry{SFR}{name=SFR, description={Star Formation Rate; rate at which a galaxy forms stars, in \hbox{${\rm M}_\odot\cdot{\rm yr}^{-1}$}}}

\newglossaryentry{SED}{name=SED, description={Spectral Energy Distribution; spectral distribution of flux/lumi- nosity of a galaxy as a function of wavelength and at very low spectral resolution}}

\newglossaryentry{UV}{name=UV, description={Ultraviolet; wavelengths in the range $\sim$10--400nm}}

\newglossaryentry{IR}{name=IR, description={Infrared; Wavelengths in the range $\sim$1--800 $\mu$m}}

\newglossaryentry{FIR}{name=FIR, description={Far Infrared; wavelengths in the range $\sim$25/40--200/350 $\mu$m}}

\newglossaryentry{LIRG}{name=LIRG, description={Luminous IR Galaxy; galaxy with $L_{IR}\geq10^{11}{\rm L}_\odot$}}

\newglossaryentry{ULIRG}{name=ULIRG, description={Ultra Luminous IR Galaxy; Galaxy with $L_{IR}\geq10^{12}{\rm L}_\odot$}}

\newglossaryentry{HST}{name=HST, description={Hubble Space Telescope; 2.4m space telescope working at UV-optical-NIR wavelengths}}

\newglossaryentry{GRB}{name=GRB, description={Gamma Ray Burst; extremely energetic emission of gamma rays in galaxies}}

\newglossaryentry{ALMA}{name=ALMA, description={Atacama Large Millimeter/ submillimeter Array}}

\newglossaryentry{DLA}{name=DLA, description={Damped Lyman-alpha system; absorption line saturating the spectra of distant sources and caused by HI column density above $2\times10^{20}$cm$^{-2}$}}

\newglossaryentry{GMASS}{name=GMASS, description={Galaxy Mass Assembly ultra-deep Spectroscopic Survey}}

\newglossaryentry{S/N}{name=S/N, description={Signal-to-Noise ratio}}

\newglossaryentry{GOODS}{name=GOODS, description={Great Observatories Origins Deep Survey}}

\newglossaryentry{CFHT}{name=CFHT, description={Canada France Hawaii Telescope}}

\newglossaryentry{CFRS}{name=CFRS, description={Canada France Redshift \hbox{Survey}}}

\newglossaryentry{CDFS}{name=CDFS, description={Chandra Deep Field South}}

\newglossaryentry{ISO}{name=ISO, description={Infrared Space
    Observatory; 0.6m telescope working between 2 and 200 $\mu$m,
    which was operated by ESA between 1995 and 1998}}

\newglossaryentry{LAE}{name=LAE, description={Lyman Alpha Emitter}}

\newglossaryentry{QSO}{name=QSO, description={Quasi Stellar Object or quasar}}

\newglossaryentry{LF}{name=LF, description={Luminosity Function}}

\newglossaryentry{DEEP2}{name=DEEP2, description={Deep Extragalactic Evolutionary Probe project, phase 2}}

\newglossaryentry{VVDS}{name=VVDS, description={VIMOS VLT Deep Survey}}

\newglossaryentry{COSMOS}{name=COSMOS, description={Cosmic Evolution Survey}}

\newglossaryentry{BAO}{name=BAO, description={Baryon Acoustic Oscillations}}

\newglossaryentry{SDSS}{name=SDSS, description={Sloan Digital Sky Survey}}

\newglossaryentry{BOSS}{name=BOSS, description={Baryon Oscillation Spectroscopis Survey, or SDSS-III}}

\newglossaryentry{FUV}{name=FUV, description={Far-UV wavelength domain Wavelengths in the range $\sim$100--200~nm}}

\newglossaryentry{NUV}{name=NUV, description={Near-UV wavelength domain Wavelengths in the range $\sim$200--300~nm}}

\newglossaryentry{LBG}{name=LBG, description={Lyman Break Galaxy}}

\newglossaryentry{DRG}{name=DRG, description={Distant Red Galaxy}}

\newglossaryentry{AGN}{name=AGN, description={Active Galactic Nucleus}}

\newglossaryentry{FWHM}{name=FWHM, description={Full Width at Half Maximum; Often used to define the width of a distribution}}

\newglossaryentry{CCD}{name=CCD, description={Charge-Coupled Device; Digital image sensor widely used in optical astronomy}}

\newglossaryentry{NIR}{name=NIR, description={Near-InfraRed; wavelengths in the range $\sim$0.7/1.0--2.5 $\mu$m}}

\newglossaryentry{CMOS}{name=CMOS, description={Complementary Metal-Oxide-Semiconductor; technology for constructing integrated circuits, including image NIR sensors}}

\newglossaryentry{IMF}{name=IMF, description={Initial Mass Function; distribution of stellar mass for a population of newly borned stars}}

\newglossaryentry{IRAF}{name=IRAF, description={Image Reduction and Analysis Facility; general purpose software system for the reduction and analysis of astronomical data, written and supported by the National Optical Astronomy Observatories (NOAO) in Tucson, Arizona}}

\newglossaryentry{SEXTRACTOR}{name=SEXTRACTOR, description={Program that builds a catalog of objects from an astronomical image, particularly oriented towards reduction of large scale galaxy-survey data or moderately crowded star fields}}

\newglossaryentry{GALFIT}{name=GALFIT, description={Program that fits 2D analytic functions to galaxies and point sources}}

\newglossaryentry{ACS}{name=ACS, description={Advanced Camera for Surveys onboard the HST}}

\newglossaryentry{WFC3}{name=WFC3, description={Wide Field Camera 3 onboard the HST}}

\newglossaryentry{GALEX}{name=GALEX, description={0.5m space telescope dedicated to the UV (NUV and FUV windows) operated from 2003 to 2012}}

\newglossaryentry{MIR}{name=MIR, description={Mid Infrared; wavelengths in the range $\sim$5--25/40 $\mu$m}}

\newglossaryentry{DS9}{name=DS9, description={Widely used Astronomical imaging and data visualization application, originally named SAOimage DS9}}

\newglossaryentry{IRAC}{name=IRAC, description={The Infrared Array Camera onboard the Spitzer telescope with four channels centered at 3.6, 4.5, 5.8, and 8.0 $\mu$m}}

\newglossaryentry{Spitzer}{name=Spitzer, description={0.85m space telescope launched in 2003 an dedicated to the IR with the IRAC and MIPS camera, and the IRS spectrograph}}

\newglossaryentry{MIPS}{name=MIPS, description={Multiband Imaging Photometer for Spitzer, is a IR camera onboard the Spitzer space telescope with two channels centered at 24 and 70 $\mu$m}}

\newglossaryentry{IRAS}{name=IRAS, description={The Infrared AStronomical Satellite was a 0.57m space telescope operated during 10 months in 1983. It performed the first all-sky survey in the IR at 12, 25, 60, and 100 $\mu$m}}

\newglossaryentry{P.A.}{name=P.A., description={Position Angle; on-sky orientation of a galaxy photometric major axis, counted anti-clockwise from North to East}}

\newglossaryentry{ADC}{name=ADC, description={Atmospheric Diffraction Corrector~--- Optical device used to correct from atmospheric diffraction in ground base instruments}}

\newglossaryentry{AM}{name=AM, description={ Airmass}}

\newglossaryentry{COG}{name=COG, description={ Curve-of-Growth. Method to measure the column density of a specie from the absorption equivalent width}}

\newglossaryentry{ETC}{name=ETC, description={Exposure Time Calculator}}

\newglossaryentry{FORS2}{name=FORS2, description={FOcal Reducer/low dispersion Spectrograph 2 at the VLT}}

\newglossaryentry{HIRES}{name=HIRES, description={High Resolution Echelle Spectrometer}}

\newglossaryentry{IGM}{name=IGM, description={Inter-Galactic Medium}}

\newglossaryentry{FLAMES/GIRAFFE}{name=FLAMES/GIRAFFE,
  description={Fiber-fed multi-object and multi-IFU medium resolution,
    optical spectrograph at the VLT}}

\newglossaryentry{SKA}{name=SKA, description={Skare Kilometer Array;
    project of radio telescope with a total collecting area of
    approximately one square kilometer}}

\newglossaryentry{ISM}{name=ISM, description={Inter-Stellar Medium}}

\newglossaryentry{TFR}{name=TFR, description={Tully--Fisher Relation;
    tight relation between the velocity width or rotation velocity of
    galaxies and their luminosity}}

\newglossaryentry{MW}{name=MW, description={ Milky Way}}

\newglossaryentry{LINER}{name=LINER, description={ Low Ionization Narrow Emission Line. Active Galactic nuclei galaxies characterized by a optical line ratios compatible with low ionization}}

%\newglossaryentry{LOSDV}{name=LOSDV, description={Line-of-sight dispersion velocities of stars}}

%\newglossaryentry{PPXF}{name=PPXF, description={ Penalized Pixel-Fitting method. Software to adjust stellar population models to an observed spectrum}}

\newglossaryentry{PWV}{name=PWV, description={ Precipitable water vapor. Amount of water vapor in the atmosphere, express in mm}}

\newglossaryentry{SFH}{name=SFH, description={Star-formation History}}

\newglossaryentry{STARLIGHT}{name=STARLIGHT, description={Software to adjust stellar population models to an observed spectrum}}

\newglossaryentry{VIMOS}{name=VIMOS, description={VIsible Multi-object Spectrograph at the VLT}}

\newglossaryentry{VLT}{name=VLT, description={European Southern Observatory Very Large Telescope}}

\newglossaryentry{USNO}{name=USNO, description={United States Naval
    Observatory}}

\newglossaryentry{UCAC}{name=UCAC, description={USNO CCD Astrograph Catalog}}

\newglossaryentry{WR}{name=WR, description={Wolf--Rayet star. Massive young stars with ages $<$10 Myr}}

\newglossaryentry{LSF}{name=LSF, description={Line Spread Function; Spectral response of a system to a point-like source}}

\newglossaryentry{IFU}{name=IFU, description={Integral Field Unit}}

\newglossaryentry{FRD}{name=FRD, description={Focal Ratio Degradation}}

\newglossaryentry{AO}{name=AO, description={Adaptive Optics;
    Technology used to improve the performances of optical systems by
    correcting the distortion of wavefronts due to the atmospheric
    turbulence}}

\newglossaryentry{GLAO}{name=GLAO, description={Ground-Layer
    Adaptive Optics; Adaptive Optics \hbox{system} in which only the lowest
    \hbox{altitude} turbulente layer, which usually \hbox{dominates} the overall
    atmospheric turbulence strength, is corrected}}

\newglossaryentry{MOAO}{name=MOAO, description={Multi-Object Adaptive
    Optics; Adaptive Optics system in which the correction is
    optimized along a limited number of directions in the FoV}}

\newglossaryentry{CTE}{name=CTE, description={Charge Transfer
    Efficiency; fraction of electrons that are successfully transferred
    from one pixel to another during one CCD read-out cycle}}

\newglossaryentry{ADU}{name=ADU, description={Analog--Digital Units;
    Digital unit in which the counts produced by a light detector are
    recorded. The conversion between the number of electrons acquired
    by the CCD and the ADUs is given by the detector gain}}

\newglossaryentry{RGB}{name=RGB, description={Red Giant Branch; Region
    of the Hertzsprung--Russel diagram corresponding to a stage in
    evolution of main sequence stars that have burnt all their
    hydrogen leading to a readjustement of the internal structure of
    the star, with expansion and subsequent reaction of the envelope.
    RGB stars are giant by their volume and luminosity but not by
    their masses}}

\newglossaryentry{AGB}{name=AGB, description={Asymptotic Giant Branch;
    Region of the Hertzsprung--Russel diagram corresponding to the
    final evolution stage of low- and intermediate-mass stars.
    This phase of evolution is characterized by
    nuclear burning of hydrogen and helium in thin shells on top of
    the electron-degenerate core of carbon and oxygen}}

\newglossaryentry{TP-AGB}{name=TP-AGB, description={Thermally Pulsing
    Asymptotic Giant Branch}}

\newglossaryentry{MS}{name=MS, description={Main Sequence stars; stars
    located along a continuous region of the Hertzsprung-Russel
    diagram that characterizes stars burning hydrogen into helium in a
    dense core. Generally, only low mass stars have lifetimes long
    enough to populate significatively the MS}}

\newglossaryentry{SGB}{name=SGB, description={Sub Giant Branch; Region
    of the Hertzsprung--Russel diagram that characterizes stars that
    have stopped burning hydrogen into helium in their core but have
    yet started doing so in a surrounding shell}}

\newglossaryentry{CHeB}{name=CHeB, description={Core Helium Burning
    phase; phase that marks the end of the RGB phase in stellar
    evolution, in which a star burns Helium in its core}}

\newglossaryentry{IMAGES}{name=IMAGES, description={ Intermediate  Mass Galaxy Evolution Sequence}}

\newglossaryentry{OSIRIS}{name=OSIRIS, description={Near-infrared integral field spectrograph designed for the Keck Adaptive Optics System}}

\newglossaryentry{KMOS}{name=KMOS, description={K band Multi-Object Spectrographat the VLT}}

%\newglossaryentry{Lstar}{name=Lstar, description={Luminosity scale above which%the central galaxy luminosity-halo mass relation flattens}}

\newglossaryentry{MOSAIC}{name=MOSAIC, description={E-ELT MOS for Astrophysics, IGM and Cosmology}}

\newglossaryentry{NICMOS}{name=NICMOS, description={Near Infrared Camera and Multi-Object Spectrometer}}

\newglossaryentry{OH}{name=OH, description={HydrOxyl radical; molecules that are responsible for the numerous sky emission lines in the NIR}}

\newglossaryentry{SINFONI}{name=SINFONI, description={Spectrograph for INtegral Field Observations in the Near Infrared at the VLT}}

\newglossaryentry{X-SHOOTER}{name=X-SHOOTER, description={UV to NIR single-target, intermediate-resolution spectrograph at the VLT}}

\newglossaryentry{MUSE}{name=MUSE, description={Optical integral field
    spectrograph at the VLT; MUSE is currently the IFU with the most
    extended FoV (i.e., up to 1$\times$1 arcmin$^2$)}}

\newglossaryentry{CGM}{name=CGM, description={Circum Galactic Medium}}

\newglossaryentry{SINS}{name=SINS, description={Spectroscopic Imaging survey in the Near-infrared with SINFONI}}


==> cross_sited.tex <==
%\providecommand\@newglossary[4]{}
%\@newglossary{main}{glg}{gls}{glo}
%\providecommand\@glsorder[1]{}
%\providecommand\@istfilename[1]{}
%\@istfilename{main_all.ist}
%\@glsorder{word}
\@writefile{toc}{\contentsline {schapter}{Foreword}{v}{schapter.1}}
\@writefile{toc}{\contentsline {schapter}{List of Figures}{xi}{schapter.2}}
\@writefile{toc}{\contentsline {schapter}{List of Tables}{xiv}{schapter.3}}
\@writefile{toc}{\contentsline {schapter}{List of Examples}{xv}{schapter.4}}
\@writefile{toc}{\contentsline {schapter}{Glossary}{xvii}{schapter.5}}
\gdef\bu@bibstyle{ws-book-har_custMP}
\@writefile{toc}{\contentsline {schapter}{Introduction}{1}{schapter.6}}
\gdef\bu@bibdata{C1_sample}
\@writefile{lof}{\addvspace {10\p@ }}
\@writefile{lot}{\addvspace {10\p@ }}
\@writefile{toc}{\contentsline {chapter}{\hbox to\@tempdima {1.\hfil }Samples and selection effects}{3}{chapter.1}}
\@writefile{toc}{\contentsline {section}{\numberline {1.1}Introduction: which sample for which science goal?}{3}{section.1.1}}
\newlabel{C1_Sect1.1}{{1.1}{3}{Introduction: which sample for which science goal?}{section.1.1}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.1.1}General rules to optimize the scientific returns from a survey of distant galaxies}{3}{subsection.1.1.1}}
\newlabel{C1_Sect1.1.1}{{1.1.1}{3}{General rules to optimize the scientific returns from a survey of distant galaxies}{subsection.1.1.1}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.1}\hspace  {2.5em}Introduction to the k-correction effects}{4}{example.1.1}}
%\zref@newlabel{mdf@pagelabel-1}{\default{1.1}\page{4}\abspage{25}\mdf@pagevalue{4}}
%%\pgfsyspdfmark {pgfid1}{8922493}{24609591}
\newlabel{RF1}{5}
\@writefile{lot}{\contentsline {table}{\numberline {1.1}{\ignorespaces Combination of measurements required for a robust determination of physical quantities of distant galaxies.\relax }}{5}{table.caption.8}}
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{C1_quantities_measurements}{{1.1}{5}{Combination of measurements required for a robust determination of physical quantities of distant galaxies.\relax }{table.caption.8}{}}
\newlabel{C1_mag}{{1.2}{6}{General rules for estimating magnitudes}{section.1.2}{}}
\@writefile{toc}{\contentsline {section}{\numberline {1.2}General rules for estimating magnitudes}{6}{section.1.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.2.1}Monochromatic and integrated magnitudes}{7}{subsection.1.2.1}}
\newlabel{C1_photsyst}{{1.2.2}{7}{Photometric systems}{subsection.1.2.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.2.2}Photometric systems}{7}{subsection.1.2.2}}
\newlabel{C1_AB}{{1.1}{8}{Photometric systems}{equation.1.2.1}{}}
\@writefile{lot}{\contentsline {table}{\numberline {1.2}{\ignorespaces Conversion factors between the AB and Vega systems\relax }}{8}{table.caption.9}}
\newlabel{C3_ABVega}{{1.2}{8}{Conversion factors between the AB and Vega systems\relax }{table.caption.9}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.2.3}Total magnitudes and proxies}{8}{subsection.1.2.3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.2.4}Absolute magnitudes}{9}{subsection.1.2.4}}
\@writefile{lot}{\contentsline {table}{\numberline {1.3}{\ignorespaces Solar absolute magnitudes in different bands for the Vega and AB systems\relax }}{10}{table.caption.10}}
\newlabel{C1_AbsMag}{{1.3}{10}{Solar absolute magnitudes in different bands for the Vega and AB systems\relax }{table.caption.10}{}}
\@writefile{toc}{\contentsline {section}{\numberline {1.3}Pre-selection of a sample prior to redshift measurement}{10}{section.1.3}}
\newlabel{C1_Sect1.2}{{1.3}{10}{Pre-selection of a sample prior to redshift measurement}{section.1.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.3.1}Photometric catalogues}{10}{subsection.1.3.1}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.3.2}Statistics: which size for a redshift survey? }{10}{subsection.1.3.2}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.2}\hspace  {2.5em}Statistical bias}{11}{example.1.2}}
%\zref@newlabel{mdf@pagelabel-2}{\default{1.2}\page{11}\abspage{32}\mdf@pagevalue{11}}
%%\pgfsyspdfmark {pgfid2}{8922493}{25195224}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.3}\hspace  {2.5em}The cone effect}{11}{example.1.3}}
%\zref@newlabel{mdf@pagelabel-3}{\default{1.3}\page{11}\abspage{32}\mdf@pagevalue{11}}
%%\pgfsyspdfmark {pgfid3}{8922493}{11102482}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.3.3}Cosmological variance}{12}{subsection.1.3.3}}
\newlabel{C1_Sect1.2.2}{{1.3.3}{12}{Cosmological variance}{subsection.1.3.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.3.4}Depth of the photometry and selection effects related to surface-brightness}{12}{subsection.1.3.4}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.4}\hspace  {2.5em}Photometric depth to recover z=0.9 spiral galaxies}{13}{example.1.4}}
%\zref@newlabel{mdf@pagelabel-4}{\default{1.4}\page{13}\abspage{34}\mdf@pagevalue{13}}
%%\pgfsyspdfmark {pgfid4}{8922493}{31523469}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.3.5}Other selection effects: Malmquist bias, Eddington bias and lensing effects}{13}{subsection.1.3.5}}
\@writefile{lof}{\contentsline {figure}{\numberline {1.1}{\ignorespaces Photometry of distant galaxies and related surface brightness selection effects}}{14}{figure.caption.11}}
\newlabel{C1_Fig1}{{1.1}{14}{Photometry of distant galaxies and related surface brightness selection effects}{figure.caption.11}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {1.3.5.1} Malmquist bias}{14}{subsubsection.1.3.5.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {1.2}{\ignorespaces Selection of galaxies to avoid Malmquist bias}}{15}{figure.caption.12}}
\newlabel{C1_Mr_z}{{1.2}{15}{Selection of galaxies to avoid Malmquist bias}{figure.caption.12}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {1.3.5.2}Eddington bias: magnitude errors near the magnitude limit}{15}{subsubsection.1.3.5.2}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.5}\hspace  {2.5em}The Eddington bias for intermediate redshift LIRGs observed by ISO in 1998}{16}{example.1.5}}
%\zref@newlabel{mdf@pagelabel-5}{\default{1.5}\page{16}\abspage{37}\mdf@pagevalue{16}}
%%\pgfsyspdfmark {pgfid5}{8922493}{21196765}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {1.3.5.3}Effect of gravitational lensing near the magnitude limit}{16}{subsubsection.1.3.5.3}}
\@writefile{lof}{\contentsline {figure}{\numberline {1.3}{\ignorespaces Number counts of ISO sources with S/N $>$ 3}}{17}{figure.caption.13}}
\newlabel{C1_Fig2_Flores99}{{1.3}{17}{Number counts of ISO sources with S/N $>$ 3}{figure.caption.13}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.3.6}K-correction and choice of the selecting magnitude}{17}{subsection.1.3.6}}
\newlabel{C1_Sect1.2.6}{{1.3.6}{17}{K-correction and choice of the selecting magnitude}{subsection.1.3.6}{}}
\newlabel{C1_absmag}{{1.2}{18}{K-correction and choice of the selecting magnitude}{equation.1.3.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1.4}{\ignorespaces Method to calculate k-corrections}}{18}{figure.caption.14}}
\newlabel{C1_kcorrect}{{1.4}{18}{Method to calculate k-corrections}{figure.caption.14}{}}
\newlabel{C1_kcorrection}{{1.3}{19}{K-correction and choice of the selecting magnitude}{equation.1.3.3}{}}
\newlabel{C1_simplekcorr}{{1.4}{19}{K-correction and choice of the selecting magnitude}{equation.1.3.4}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.6}\hspace  {2.5em}Selecting wavelength for comparing $z=0$ to $z=0.8$ galaxies}{20}{example.1.6}}
%\zref@newlabel{mdf@pagelabel-6}{\default{1.6}\page{20}\abspage{41}\mdf@pagevalue{20}}
%%\pgfsyspdfmark {pgfid6}{8922493}{20701198}
\@writefile{lof}{\contentsline {figure}{\numberline {1.5}{\ignorespaces k-corrections for 3 galaxy types}}{21}{figure.caption.15}}
\newlabel{C1_Fig2}{{1.5}{21}{k-corrections for 3 galaxy types}{figure.caption.15}{}}
\@writefile{toc}{\contentsline {section}{\numberline {1.4}Redshift surveys}{21}{section.1.4}}
\newlabel{C1_Sect1.3}{{1.4}{21}{Redshift surveys}{section.1.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.4.1}Redshift measurements and spectroscopic selection effects}{21}{subsection.1.4.1}}
\newlabel{C1_Sect1.3.1}{{1.4.1}{21}{Redshift measurements and spectroscopic selection effects}{subsection.1.4.1}{}}
\@writefile{lot}{\contentsline {table}{\numberline {1.4}{\ignorespaces Comparison of multi-spectrograph capabilities for redshift surveys.\relax }}{22}{table.caption.16}}
\newlabel{C1_spectro_qualities}{{1.4}{22}{Comparison of multi-spectrograph capabilities for redshift surveys.\relax }{table.caption.16}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.4.2}Determination of the luminosity function, uncertainties \& completeness tests}{24}{subsection.1.4.2}}
\newlabel{C1_Sect1.3.2}{{1.4.2}{24}{Determination of the luminosity function, uncertainties \& completeness tests}{subsection.1.4.2}{}}
\newlabel{C1_Vmax}{{1.5}{25}{Determination of the luminosity function, uncertainties \& completeness tests}{equation.1.4.5}{}}
\newlabel{C1_Vmax2}{{1.6}{25}{Determination of the luminosity function, uncertainties \& completeness tests}{equation.1.4.6}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.7}\hspace  {2.5em}Calculation of the rest-frame B-band luminosity function of the CFRS-like survey}{25}{example.1.7}}
%\zref@newlabel{mdf@pagelabel-7}{\default{1.7}\page{26}\abspage{47}\mdf@pagevalue{26}}
%%\pgfsyspdfmark {pgfid7}{8922493}{11749585}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.8}\hspace  {2.5em}Effect of large scale structures on the luminosity function and photometric redshifts}{27}{example.1.8}}
%\zref@newlabel{mdf@pagelabel-8}{\default{1.8}\page{27}\abspage{48}\mdf@pagevalue{27}}
%%\pgfsyspdfmark {pgfid8}{8922493}{11530398}
%\zref@newlabel{mdf@pagelabel-9}{\default{1.8}\page{28}\abspage{49}\mdf@pagevalue{28}}
%%\pgfsyspdfmark {pgfid9}{8922493}{32541967}
\@writefile{lof}{\contentsline {figure}{\numberline {1.6}{\ignorespaces Effect of large scale structures in the GOODS-S field}}{28}{figure.caption.17}}
\newlabel{C1_Fig_Ravikumar}{{1.6}{28}{Effect of large scale structures in the GOODS-S field}{figure.caption.17}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.4.3}Examples of surveys (CFRS, DEEP2, VVDS, zCOSMOS \& WIGGLEZ)}{29}{subsection.1.4.3}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.9}\hspace  {2.5em}Two sub-samples of distant galaxies from the VVDS}{30}{example.1.9}}
%\zref@newlabel{mdf@pagelabel-10}{\default{1.9}\page{30}\abspage{51}\mdf@pagevalue{30}}
%%\pgfsyspdfmark {pgfid10}{8922493}{11792542}
\newlabel{RF2}{31}
\@writefile{lot}{\contentsline {table}{\numberline {1.5}{\ignorespaces Comparison of several redshift surveys.\relax }}{31}{table.caption.18}}
\newlabel{C1_surveys}{{1.5}{31}{Comparison of several redshift surveys.\relax }{table.caption.18}{}}
%\zref@newlabel{mdf@pagelabel-11}{\default{1.9}\page{32}\abspage{53}\mdf@pagevalue{32}}
%\pgfsyspdfmark {pgfid11}{8922493}{34245903}
\@writefile{toc}{\contentsline {section}{\numberline {1.5} Photometric redshifts}{32}{section.1.5}}
\newlabel{C1_Sect1.4}{{1.5}{32}{Photometric redshifts}{section.1.5}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.10}\hspace  {2.5em}Stellar mass and star formation densities estimated through photo-z}{35}{example.1.10}}
%\zref@newlabel{mdf@pagelabel-12}{\default{1.10}\page{35}\abspage{56}\mdf@pagevalue{35}}
%\pgfsyspdfmark {pgfid12}{8922493}{20684814}
\@writefile{toc}{\contentsline {section}{\numberline {1.6} Selection of very distant galaxies at $z >>1$}{36}{section.1.6}}
\newlabel{C1_Sect1.5}{{1.6}{36}{Selection of very distant galaxies at $z >>1$}{section.1.6}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.6.1}Lyman break galaxies (LBGs)}{36}{subsection.1.6.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {1.7}{\ignorespaces Selection of Lyman break galaxies}}{37}{figure.caption.19}}
\newlabel{C1_Fig3}{{1.7}{37}{Selection of Lyman break galaxies}{figure.caption.19}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.6.2}Balmer and 400 nm break drop-out galaxies}{38}{subsection.1.6.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.6.3}Ly$\alpha $ emitters (LAEs)}{38}{subsection.1.6.3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.6.4}Indirect probes: damped Ly$\alpha $ systems (DLAs) and gamma ray burst hosts}{39}{subsection.1.6.4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.6.5}Dust-enshrouded galaxies}{40}{subsection.1.6.5}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.6.6}Towards an overview of the high-z galaxy population and a fair determination of the luminosity functions}{40}{subsection.1.6.6}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}1.11}\hspace  {2.5em}A sub-sample of z$\sim $ 2 galaxies for determining kinematics}{41}{example.1.11}}
%\zref@newlabel{mdf@pagelabel-13}{\default{1.11}\page{41}\abspage{62}\mdf@pagevalue{41}}
%\pgfsyspdfmark {pgfid13}{8922493}{18533213}
\@writefile{toc}{\contentsline {section}{\numberline {1.7} Relating distant \& nearby galaxies}{41}{section.1.7}}
\newlabel{C1_Sect1.6}{{1.7}{41}{Relating distant \& nearby galaxies}{section.1.7}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1.8}{\ignorespaces Evolution of Damped Lyman Alpha systems}}{43}{figure.caption.20}}
\newlabel{C1_Figure_Prochaska09}{{1.8}{43}{Evolution of Damped Lyman Alpha systems}{figure.caption.20}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1.9}{\ignorespaces Evolution of the Hubble Sequence}}{44}{figure.caption.21}}
\newlabel{C1_Figure_Delgado}{{1.9}{44}{Evolution of the Hubble Sequence}{figure.caption.21}{}}
\gdef\bu@bibdata{C2_imaging}
\@writefile{lof}{\addvspace {10\p@ }}
\@writefile{lot}{\addvspace {10\p@ }}
\@writefile{toc}{\contentsline {chapter}{\hbox to\@tempdima {2.\hfil }Imaging and Photometry}{48}{chapter.2}}
\@writefile{toc}{\contentsline {section}{\numberline {2.1}Introduction}{48}{section.2.1}}
\@writefile{lot}{\contentsline {table}{\numberline {2.1}{\ignorespaces Physical quantities that can be inferred from imaging data.\relax }}{49}{table.caption.23}}
\newlabel{C2_TabWhyImages}{{2.1}{49}{Physical quantities that can be inferred from imaging data.\relax }{table.caption.23}{}}
\newlabel{C2_caract}{{2.2}{50}{Basic Elements of imaging and image analysis}{section.2.2}{}}
\@writefile{toc}{\contentsline {section}{\numberline {2.2}Basic Elements of imaging and image analysis}{50}{section.2.2}}
\newlabel{C2_spatialres}{{2.2.1}{50}{Spatial resolution}{subsection.2.2.1}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2.1}Spatial resolution}{50}{subsection.2.2.1}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.1}\hspace  {2.5em}How to estimate the spatial resolution of an image?}{50}{example.2.1}}
%\zref@newlabel{mdf@pagelabel-14}{\default{2.1}\page{50}\abspage{71}\mdf@pagevalue{50}}
\newlabel{C2_ExFWHM}{{2.1}{50}{Spatial resolution}{example.2.1}{}}
%\pgfsyspdfmark {pgfid14}{8922493}{11507193}
%\zref@newlabel{mdf@pagelabel-15}{\default{2.1}\page{51}\abspage{72}\mdf@pagevalue{51}}
%\pgfsyspdfmark {pgfid15}{8922493}{36801807}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.1.1}PSF shape}{51}{subsubsection.2.2.1.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.1}{\ignorespaces Example of ground-based PSF profiles}}{52}{figure.caption.24}}
\newlabel{C2_AOPSF}{{2.1}{52}{Example of ground-based PSF profiles}{figure.caption.24}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.1.2}Resolution and sampling}{52}{subsubsection.2.2.1.2}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.1.3}Improving the resolution: dithering vs. deconvolution}{53}{subsubsection.2.2.1.3}}
\newlabel{C2_depth}{{2.2.2}{54}{Depth}{subsection.2.2.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2.2}Depth}{54}{subsection.2.2.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.2}{\ignorespaces Effect of the cosmological surface brightness dimming on the morphology of galaxies}}{54}{figure.caption.25}}
\newlabel{C2_FigSB}{{2.2}{54}{Effect of the cosmological surface brightness dimming on the morphology of galaxies}{figure.caption.25}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.2}\hspace  {2.5em}What are the deepest images ever?}{55}{example.2.2}}
%\zref@newlabel{mdf@pagelabel-16}{\default{2.2}\page{55}\abspage{76}\mdf@pagevalue{55}}
\newlabel{C2_ExDepth}{{2.2}{55}{Depth}{example.2.2}{}}
%\pgfsyspdfmark {pgfid16}{8922493}{26291603}
\newlabel{C2_detect}{{2.2.2.1}{55}{Detecting and analyzing galaxy structures}{subsubsection.2.2.2.1}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.2.1}Detecting and analyzing galaxy structures}{55}{subsubsection.2.2.2.1}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.3}\hspace  {2.5em}How to construct a source catalogue from an image?}{56}{example.2.3}}
%\zref@newlabel{mdf@pagelabel-17}{\default{2.3}\page{56}\abspage{77}\mdf@pagevalue{56}}
\newlabel{C2_ExSky}{{2.3}{56}{Detecting and analyzing galaxy structures}{example.2.3}{}}
%\pgfsyspdfmark {pgfid17}{8922493}{12975831}
%\zref@newlabel{mdf@pagelabel-18}{\default{2.3}\page{57}\abspage{78}\mdf@pagevalue{57}}
%\pgfsyspdfmark {pgfid18}{8922493}{12389647}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.2.2}Image post-processing techniques}{58}{subsubsection.2.2.2.2}}
\newlabel{C2_postproc}{{2.2.2.2}{58}{Image post-processing techniques}{subsubsection.2.2.2.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.3}{\ignorespaces Improving the detection threshold using several images in different bands}}{59}{figure.caption.26}}
\newlabel{C2_Detect}{{2.3}{59}{Improving the detection threshold using several images in different bands}{figure.caption.26}{}}
\newlabel{C2_spectralband}{{2.2.3}{59}{Spectral Bandwidth}{subsection.2.2.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2.3}Spectral Bandwidth}{59}{subsection.2.2.3}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.3.1}Photometric filters}{59}{subsubsection.2.2.3.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.4}{\ignorespaces Examples of broad and narrow-band filters}}{60}{figure.caption.27}}
\newlabel{C2_Filters}{{2.4}{60}{Examples of broad and narrow-band filters}{figure.caption.27}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.3.2}Rest-frame photometry}{61}{subsubsection.2.2.3.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.5}{\ignorespaces Impact of stellar populations on the luminosities and mass-to-light ratios.}}{62}{figure.caption.28}}
\newlabel{C2_Charlot97}{{2.5}{62}{Impact of stellar populations on the luminosities and mass-to-light ratios}{figure.caption.28}{}}
\newlabel{C2_obs}{{2.2.4}{62}{Observing with imagers}{subsection.2.2.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2.4}Observing with imagers}{62}{subsection.2.2.4}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.4.1}Space vs. ground-based imagers}{62}{subsubsection.2.2.4.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.6}{\ignorespaces Galaxy morphology as a function of wavelength}}{63}{figure.caption.29}}
\newlabel{C2_GalMorphoWavelength}{{2.6}{63}{Galaxy morphology as a function of wavelength}{figure.caption.29}{}}
\@writefile{lot}{\contentsline {table}{\numberline {2.2}{\ignorespaces Comparison between central wavelengths of SDSS and GOODS filters.\relax }}{63}{table.caption.30}}
\newlabel{C2_TabSDSS}{{2.2}{63}{Comparison between central wavelengths of SDSS and GOODS filters.\relax }{table.caption.30}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.4.2}Dithering}{64}{subsubsection.2.2.4.2}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.4.3}Observing with Adaptive Optics}{64}{subsubsection.2.2.4.3}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.2.4.4}Observing in the IR with ground-based telescopes}{65}{subsubsection.2.2.4.4}}
\newlabel{C2_reduction}{{2.3}{66}{Data Reduction}{section.2.3}{}}
\@writefile{toc}{\contentsline {section}{\numberline {2.3}Data Reduction}{66}{section.2.3}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.3.1}Basic principles}{66}{subsection.2.3.1}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.3.2}Description of basic calibration frames}{67}{subsection.2.3.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.3.3}Reducing and calibrating images}{68}{subsection.2.3.3}}
\newlabel{eqreduc}{{2.1}{68}{Reducing and calibrating images}{equation.2.3.1}{}}
\newlabel{C2_footnotesupersky}{{16}{68}{}{Hfootnote.26}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.4}\hspace  {2.5em}How to reduce an image?}{69}{example.2.4}}
%\zref@newlabel{mdf@pagelabel-19}{\default{2.4}\page{70}\abspage{91}\mdf@pagevalue{70}}
\newlabel{C3_ExDataReduction}{{2.4}{70}{Reducing and calibrating images}{example.2.4}{}}
%\pgfsyspdfmark {pgfid19}{8922493}{11432094}
%\zref@newlabel{mdf@pagelabel-20}{\default{2.4}\page{71}\abspage{92}\mdf@pagevalue{71}}
%\pgfsyspdfmark {pgfid20}{8922493}{41189078}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.3.3.1}Fringing and scattered light}{71}{subsubsection.2.3.3.1}}
\newlabel{C2_SNR}{{2.3.4}{72}{Signal-to-noise ratio}{subsection.2.3.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.3.4}Signal-to-noise ratio}{72}{subsection.2.3.4}}
\newlabel{fullccdeq}{{2.2}{72}{Signal-to-noise ratio}{equation.2.3.2}{}}
\newlabel{ccdeq}{{2.5}{73}{Signal-to-noise ratio}{equation.2.3.5}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.3.4.1}S/N regimes}{73}{subsubsection.2.3.4.1}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.5}\hspace  {2.5em}How to choose \emph  {dit} in the NIR?}{74}{example.2.5}}
%\zref@newlabel{mdf@pagelabel-21}{\default{2.5}\page{74}\abspage{95}\mdf@pagevalue{74}}
%\pgfsyspdfmark {pgfid21}{8922493}{21379053}
\newlabel{C2_morpho}{{2.4}{74}{Galaxy Morphology}{section.2.4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {2.4}Galaxy Morphology}{74}{section.2.4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4.1}Morphological classification}{75}{subsection.2.4.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.7}{\ignorespaces Example of morphological analysis on a distant spiral galaxy.}}{76}{figure.caption.31}}
\newlabel{C2_MorphoParam}{{2.7}{76}{Example of morphological analysis on a distant spiral galaxy}{figure.caption.31}{}}
\newlabel{C2_highzmorph}{{2.4.2}{77}{Characterizing morphology at high redshifts}{subsection.2.4.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4.2}Characterizing morphology at high redshifts}{77}{subsection.2.4.2}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.6}\hspace  {2.5em}Measuring the surface brightness profile and basic properties of a distant galaxy}{78}{example.2.6}}
%\zref@newlabel{mdf@pagelabel-22}{\default{2.6}\page{78}\abspage{99}\mdf@pagevalue{78}}
\newlabel{C2_SBprofile}{{2.6}{78}{Characterizing morphology at high redshifts}{example.2.6}{}}
%\pgfsyspdfmark {pgfid22}{8922493}{11686956}
%\zref@newlabel{mdf@pagelabel-23}{\default{2.6}\page{79}\abspage{100}\mdf@pagevalue{79}}
%\pgfsyspdfmark {pgfid23}{8922493}{14650639}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4.3}Empirical methods - Eyeball classifications}{80}{subsection.2.4.3}}
\newlabel{C2_lightdecomp}{{2.4.4}{80}{Light decomposition using software}{subsection.2.4.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4.4}Light decomposition using software}{80}{subsection.2.4.4}}
\@writefile{lot}{\contentsline {table}{\numberline {2.3}{\ignorespaces Popular programs used for parametric morphological decomposition\relax }}{81}{table.caption.32}}
\newlabel{C2_param}{{2.3}{81}{Popular programs used for parametric morphological decomposition\relax }{table.caption.32}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.7}\hspace  {2.5em}How to decompose a galaxy into a bulge and a disk using GALFIT?}{81}{example.2.7}}
%\zref@newlabel{mdf@pagelabel-24}{\default{2.7}\page{82}\abspage{103}\mdf@pagevalue{82}}
\newlabel{C2_ExGalfit}{{2.7}{82}{Light decomposition using software}{example.2.7}{}}
%\pgfsyspdfmark {pgfid24}{8922493}{11952741}
%\zref@newlabel{mdf@pagelabel-25}{\default{2.7}\page{83}\abspage{104}\mdf@pagevalue{83}}
%\pgfsyspdfmark {pgfid25}{8922493}{18874070}
\@writefile{lof}{\contentsline {figure}{\numberline {2.8}{\ignorespaces GALFIT decompositions and residual maps.}}{84}{figure.caption.33}}
\newlabel{C2_MorphoProfile}{{2.8}{84}{GALFIT decompositions and residual maps}{figure.caption.33}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4.5}Automatic methods with two or more parameters}{85}{subsection.2.4.5}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.4.5.1}Can we classify galaxy morphologies with automatic methods?}{85}{subsubsection.2.4.5.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.9}{\ignorespaces Comparison between parametric and non-parametric morphological classification methods.}}{86}{figure.caption.34}}
\newlabel{C2_MorphoComp}{{2.9}{86}{Comparison between parametric and non-parametric morphological classification methods}{figure.caption.34}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.4.5.2}Color bi-modality: an over-simplified approach}{87}{subsubsection.2.4.5.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.10}{\ignorespaces Morphological classification tree}}{88}{figure.caption.35}}
\newlabel{C2_FigClassifTree}{{2.10}{88}{Morphological classification tree}{figure.caption.35}{}}
\newlabel{C2_morphotree}{{2.4.6}{88}{A pragmatic and conservative approach to classify distant galaxies}{subsection.2.4.6}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4.6}A pragmatic and conservative approach to classify distant galaxies}{88}{subsection.2.4.6}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.8}\hspace  {2.5em}How to classify a galaxy morphology using a semi-empirical decision tree?}{88}{example.2.8}}
%\zref@newlabel{mdf@pagelabel-26}{\default{2.8}\page{88}\abspage{109}\mdf@pagevalue{88}}
\newlabel{C2_ClassifTree}{{2.8}{88}{A pragmatic and conservative approach to classify distant galaxies}{Item.41}{}}
%\pgfsyspdfmark {pgfid26}{8922493}{11534661}
%\zref@newlabel{mdf@pagelabel-27}{\default{2.8}\page{89}\abspage{110}\mdf@pagevalue{89}}
%\pgfsyspdfmark {pgfid27}{8922493}{11242767}
\newlabel{C2_Sectcolormaps}{{2.4.6.1}{91}{Color maps}{subsubsection.2.4.6.1}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.4.6.1}Color maps}{91}{subsubsection.2.4.6.1}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.9}\hspace  {2.5em}How to construct a color map?}{91}{example.2.9}}
%\zref@newlabel{mdf@pagelabel-28}{\default{2.9}\page{91}\abspage{112}\mdf@pagevalue{91}}
\newlabel{C2_ExColorImage}{{2.9}{91}{Color maps}{example.2.9}{}}
%\pgfsyspdfmark {pgfid28}{8922493}{13823707}
\@writefile{lof}{\contentsline {figure}{\numberline {2.11}{\ignorespaces Examples of color maps of z$\sim $0.6 galaxies.}}{92}{figure.caption.36}}
\newlabel{C2_ColorMap}{{2.11}{92}{Examples of color maps of z$\sim $0.6 galaxies}{figure.caption.36}{}}
%\zref@newlabel{mdf@pagelabel-29}{\default{2.9}\page{92}\abspage{113}\mdf@pagevalue{92}}
%\pgfsyspdfmark {pgfid29}{8922493}{13274466}
%\zref@newlabel{mdf@pagelabel-30}{\default{2.9}\page{93}\abspage{114}\mdf@pagevalue{93}}
%\pgfsyspdfmark {pgfid30}{8922493}{38469334}
\newlabel{C2_multiphot}{{2.5}{93}{Multi-wavelength photometry}{section.2.5}{}}
\@writefile{toc}{\contentsline {section}{\numberline {2.5}Multi-wavelength photometry}{93}{section.2.5}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.5.1}Cross-correlating images at different wavelengths}{93}{subsection.2.5.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.12}{\ignorespaces Comparing IR and optical images}}{94}{figure.caption.37}}
\newlabel{C2_counterpart1}{{2.12}{94}{Comparing IR and optical images}{figure.caption.37}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.10}\hspace  {2.5em}How to identify optical counterpart of IR sources?}{94}{example.2.10}}
%\zref@newlabel{mdf@pagelabel-31}{\default{2.10}\page{94}\abspage{115}\mdf@pagevalue{94}}
%\pgfsyspdfmark {pgfid31}{8922493}{16827901}
\@writefile{lof}{\contentsline {figure}{\numberline {2.13}{\ignorespaces Effects limiting the identification of optical counterparts in the IR}}{95}{figure.caption.38}}
\newlabel{C2_counterpart2}{{2.13}{95}{Effects limiting the identification of optical counterparts in the IR}{figure.caption.38}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.5.2}Aperture photometry}{95}{subsection.2.5.2}}
\newlabel{C2_apphot}{{2.5.2}{95}{Aperture photometry}{subsection.2.5.2}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.5.2.1}Aperture shape}{96}{subsubsection.2.5.2.1}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.5.2.2}Aperture size}{96}{subsubsection.2.5.2.2}}
\newlabel{C2_fluxmeasure}{{2.5.2.3}{97}{Flux measurement}{subsubsection.2.5.2.3}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.5.2.3}Flux measurement}{97}{subsubsection.2.5.2.3}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.14}{\ignorespaces Confusion at long wavelengths.}}{97}{figure.caption.39}}
\newlabel{C2_confusion}{{2.14}{97}{Confusion at long wavelengths}{figure.caption.39}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.15}{\ignorespaces Photometry with priors.}}{98}{figure.caption.40}}
\newlabel{C2_PhotPriors}{{2.15}{98}{Photometry with priors}{figure.caption.40}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.11}\hspace  {2.5em}How to measure photometry in the confusion limited regime?}{99}{example.2.11}}
%\zref@newlabel{mdf@pagelabel-32}{\default{2.11}\page{99}\abspage{120}\mdf@pagevalue{99}}
\newlabel{C2_ExConfusionPhot}{{2.11}{99}{Flux measurement}{example.2.11}{}}
%\pgfsyspdfmark {pgfid32}{8922493}{11719724}
%\zref@newlabel{mdf@pagelabel-33}{\default{2.11}\page{100}\abspage{121}\mdf@pagevalue{100}}
%\pgfsyspdfmark {pgfid33}{8922493}{40209679}
\newlabel{C2_apcorr}{{2.5.2.4}{100}{Can we recover total, multi-wavelength magnitudes ?}{subsubsection.2.5.2.4}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.5.2.4}Can we recover total, multi-wavelength magnitudes ?}{100}{subsubsection.2.5.2.4}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.5.2.5}Flux and color uncertainties}{100}{subsubsection.2.5.2.5}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.16}{\ignorespaces Random error in point-source photometry}}{101}{figure.caption.41}}
\newlabel{C2_photerro}{{2.16}{101}{Random error in point-source photometry}{figure.caption.41}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.12}\hspace  {2.5em}Biases in colors caused by uncontrolled aperture corrections}{102}{example.2.12}}
%\zref@newlabel{mdf@pagelabel-34}{\default{2.12}\page{102}\abspage{123}\mdf@pagevalue{102}}
%\pgfsyspdfmark {pgfid34}{8922493}{16081679}
\newlabel{C2_sed}{{2.6}{103}{Spectral Energy Distributions}{section.2.6}{}}
\@writefile{toc}{\contentsline {section}{\numberline {2.6}Spectral Energy Distributions}{103}{section.2.6}}
\newlabel{C2_sedstars}{{2.6.1}{103}{Impact of the stellar populations: which wavelength tells you what?}{subsection.2.6.1}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.6.1}Impact of the stellar populations: which wavelength tells you what?}{103}{subsection.2.6.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.17}{\ignorespaces Galaxy SED templates}}{104}{figure.caption.42}}
\newlabel{C2_SEDtempl}{{2.17}{104}{Galaxy SED templates}{figure.caption.42}{}}
\newlabel{C2_dust}{{2.6.2}{105}{Impact of dust and gas}{subsection.2.6.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.6.2}Impact of dust and gas}{105}{subsection.2.6.2}}
\@writefile{toc}{\contentsline {paragraph}{Galactic extinction}{105}{section*.43}}
\@writefile{toc}{\contentsline {paragraph}{Internal extinction}{105}{section*.44}}
\newlabel{C2_extdisk}{{2.6.2}{106}{The specific case of extinction in regular galactic disks}{section*.45}{}}
\@writefile{toc}{\contentsline {paragraph}{The specific case of extinction in regular galactic disks}{106}{section*.45}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.6.2.1}The impact of neutral HI absorption}{106}{subsubsection.2.6.2.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.18}{\ignorespaces Example of Lyman-Break Galaxy at z$\sim $8}}{107}{figure.caption.46}}
\newlabel{C2_lbg}{{2.18}{107}{Example of Lyman-Break Galaxy at z$\sim $8}{figure.caption.46}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.6.2.2}The impact of nebular emissions}{108}{subsubsection.2.6.2.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.6.3}Estimating galaxy properties from an SED}{108}{subsection.2.6.3}}
\newlabel{C2_SPSmodels}{{2.6.3.1}{108}{Use of Stellar Population Models}{subsubsection.2.6.3.1}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.6.3.1}Use of Stellar Population Models}{108}{subsubsection.2.6.3.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.19}{\ignorespaces Nebular to total continuum flux ratio.}}{109}{figure.caption.47}}
\newlabel{C2_NebCont}{{2.19}{109}{Nebular to total continuum flux ratio}{figure.caption.47}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.6.3.2}Issues related to SED fitting}{110}{subsubsection.2.6.3.2}}
\@writefile{toc}{\contentsline {paragraph}{Number of stellar populations.}{110}{section*.48}}
\@writefile{toc}{\contentsline {paragraph}{Aperture corrections.}{110}{section*.49}}
\@writefile{toc}{\contentsline {paragraph}{Numerical methods and uncertainties.}{110}{section*.50}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.20}{\ignorespaces SED fitting using the least-square method}}{111}{figure.caption.51}}
\newlabel{C2_SEDex}{{2.20}{111}{SED fitting using the least-square method}{figure.caption.51}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.13}\hspace  {2.5em}How to fit a galaxy SED?}{111}{example.2.13}}
%\zref@newlabel{mdf@pagelabel-35}{\default{2.13}\page{112}\abspage{133}\mdf@pagevalue{112}}
\newlabel{C2_ExFitSED}{{2.13}{112}{Numerical methods and uncertainties}{example.2.13}{}}
%\pgfsyspdfmark {pgfid35}{8922493}{19810513}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.6.4}Estimating stellar mass}{112}{subsection.2.6.4}}
\newlabel{C2_mass}{{2.6.4}{112}{Estimating stellar mass}{subsection.2.6.4}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.6.4.1}Using full SED fitting}{112}{subsubsection.2.6.4.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {2.21}{\ignorespaces Effect of the filter set on stellar mass estimates derived using SED fitting.}}{113}{figure.caption.52}}
\newlabel{C2_SEDfilters}{{2.21}{113}{Effect of the filter set on stellar mass estimates derived using SED fitting}{figure.caption.52}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.14}\hspace  {2.5em}How to estimate the stellar mass of a galaxy using SED fitting?}{114}{example.2.14}}
%\zref@newlabel{mdf@pagelabel-36}{\default{2.14}\page{114}\abspage{135}\mdf@pagevalue{114}}
\newlabel{C2_ExMstellar}{{2.14}{114}{Using full SED fitting}{example.2.14}{}}
%\pgfsyspdfmark {pgfid36}{8922493}{13847749}
%\zref@newlabel{mdf@pagelabel-37}{\default{2.14}\page{115}\abspage{136}\mdf@pagevalue{115}}
%\pgfsyspdfmark {pgfid37}{8922493}{24837846}
\@writefile{lof}{\contentsline {figure}{\numberline {2.22}{\ignorespaces Estimating the maximal contribution of the oldest populations in SED fitting.}}{116}{figure.caption.53}}
\newlabel{C2_SEDmax}{{2.22}{116}{Estimating the maximal contribution of the oldest populations in SED fitting}{figure.caption.53}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.6.4.2}Using the single color method}{116}{subsubsection.2.6.4.2}}
\@writefile{lot}{\contentsline {table}{\numberline {2.4}{\ignorespaces Optimal color-luminosity $M/L$ ratio calibrations.\relax }}{117}{table.caption.54}}
\newlabel{C2_TabBell}{{2.4}{117}{Optimal color-luminosity $M/L$ ratio calibrations.\relax }{table.caption.54}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.15}\hspace  {2.5em}How to get simple estimates of the stellar mass?}{118}{example.2.15}}
%\zref@newlabel{mdf@pagelabel-38}{\default{2.15}\page{118}\abspage{139}\mdf@pagevalue{118}}
\newlabel{C2_SimpleMAss}{{2.15}{118}{Using the single color method}{example.2.15}{}}
%\pgfsyspdfmark {pgfid38}{8922493}{24699244}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.6.5}Estimating galaxy SFRs}{118}{subsection.2.6.5}}
\newlabel{C2_sfr}{{2.6.5}{118}{Estimating galaxy SFRs}{subsection.2.6.5}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.6.5.1}SFR tracers}{118}{subsubsection.2.6.5.1}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {2.6.5.2}Estimating the SFR in distant galaxies}{119}{subsubsection.2.6.5.2}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}2.16}\hspace  {2.5em}How to estimate the SFR in a distant galaxy?}{120}{example.2.16}}
%\zref@newlabel{mdf@pagelabel-39}{\default{2.16}\page{120}\abspage{141}\mdf@pagevalue{120}}
\newlabel{C2_ExSFR}{{2.16}{120}{Estimating the SFR in distant galaxies}{example.2.16}{}}
%\pgfsyspdfmark {pgfid39}{8922493}{11792542}
%\zref@newlabel{mdf@pagelabel-40}{\default{2.16}\page{121}\abspage{142}\mdf@pagevalue{121}}
%\pgfsyspdfmark {pgfid40}{8922493}{35949839}
\@writefile{lof}{\contentsline {figure}{\numberline {2.23}{\ignorespaces Comparison between IR SFR estimates and spectroscopic measurements.}}{122}{figure.caption.55}}
\newlabel{C2_SFRcomp}{{2.23}{122}{Comparison between IR SFR estimates and spectroscopic measurements}{figure.caption.55}{}}
\gdef\bu@bibdata{C3_spectro}
\@writefile{lof}{\addvspace {10\p@ }}
\@writefile{lot}{\addvspace {10\p@ }}
\@writefile{toc}{\contentsline {chapter}{\hbox to\@tempdima {3.\hfil }Integrated Spectroscopy}{131}{chapter.3}}
\@writefile{toc}{\contentsline {section}{\numberline {3.1}Introduction}{131}{section.3.1}}
\newlabel{C3_Introduction}{{3.1}{131}{Introduction}{section.3.1}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1.1}Desiccating a galaxy spectrum}{132}{subsection.3.1.1}}
\newlabel{C3_Introduction_Desiccating}{{3.1.1}{132}{Desiccating a galaxy spectrum}{subsection.3.1.1}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.1.1.1}UV spectrum}{132}{subsubsection.3.1.1.1}}
\newlabel{RF3}{133}
\@writefile{lot}{\contentsline {table}{\numberline {3.1}{\ignorespaces Diagnostics to estimate the properties of the ISM in UV and optical spectra\relax }}{133}{table.caption.57}}
\newlabel{C3_Tab_Diagnostics_ISM}{{3.1}{133}{Diagnostics to estimate the properties of the ISM in UV and optical spectra\relax }{table.caption.57}{}}
\newlabel{RF4}{134}
\@writefile{lof}{\contentsline {figure}{\numberline {3.1}{\ignorespaces UV-to-Optical rest frame spectra of distant galaxies}}{134}{figure.caption.58}}
\newlabel{C3_Fig_spectres}{{3.1}{134}{UV-to-Optical rest frame spectra of distant galaxies}{figure.caption.58}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.1.1.2}Visible spectrum}{135}{subsubsection.3.1.1.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1.2}Integrated spectroscopy of distant targets}{136}{subsection.3.1.2}}
\newlabel{C3_Introduction_Integrated_spectroscopy}{{3.1.2}{136}{Integrated spectroscopy of distant targets}{subsection.3.1.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.2}{\ignorespaces Line position at observable frame as a function of redshift}}{137}{figure.caption.60}}
\newlabel{C3_Fig_Redshift_emiLines}{{3.2}{137}{Line position at observable frame as a function of redshift}{figure.caption.60}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3.2}Basics of spectroscopy}{138}{section.3.2}}
\newlabel{C3_Integrated_spectroscopy}{{3.2}{138}{Basics of spectroscopy}{section.3.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.3}{\ignorespaces Schematic view of a spectrograph}}{138}{figure.caption.61}}
\newlabel{C3_Spectrograph}{{3.3}{138}{Schematic view of a spectrograph}{figure.caption.61}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2.1}Multi-object spectrographs}{139}{subsection.3.2.1}}
\newlabel{C3_Integrated_spectroscopy_MOS}{{3.2.1}{139}{Multi-object spectrographs}{subsection.3.2.1}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2.2}Slit-less grism spectrographs}{140}{subsection.3.2.2}}
\newlabel{C3_Integrated_spectroscopy_Slitess}{{3.2.2}{140}{Slit-less grism spectrographs}{subsection.3.2.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2.3}Near-IR spectrographs}{140}{subsection.3.2.3}}
\newlabel{C3_Integrated_spectroscopy_NIR}{{3.2.3}{140}{Near-IR spectrographs}{subsection.3.2.3}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3.3}Preparing observations}{141}{section.3.3}}
\newlabel{C3_Prepare_Obs}{{3.3}{141}{Preparing observations}{section.3.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3.1}The choice of spectral resolution}{141}{subsection.3.3.1}}
\newlabel{C3_Prepare_Obs_R}{{3.3.1}{141}{The choice of spectral resolution}{subsection.3.3.1}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.1}\hspace  {2.5em}Effect of low spectral resolution on the estimated quantities}{141}{example.3.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.4}{\ignorespaces Spectra of distant galaxies: Low vs moderate spectral resolution}}{142}{figure.caption.62}}
\newlabel{C3_Fig_line_dilu}{{3.4}{142}{Spectra of distant galaxies: Low vs moderate spectral resolution}{figure.caption.62}{}}
%\zref@newlabel{mdf@pagelabel-41}{\default{3.1}\page{142}\abspage{163}\mdf@pagevalue{142}}
%\pgfsyspdfmark {pgfid41}{8922493}{11102482}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3.2}Optimization of the signal-to-noise ratio}{143}{subsection.3.3.2}}
\newlabel{C3_R_S/N}{{3.3.2}{143}{Optimization of the signal-to-noise ratio}{subsection.3.3.2}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.3.2.1}Limits on S/N and error propagation}{143}{subsubsection.3.3.2.1}}
\@writefile{lot}{\contentsline {table}{\numberline {3.2}{\ignorespaces Lower limits on S/N required to detect and measure spectral features\relax }}{143}{table.caption.63}}
\newlabel{C3_Tab_S/N_limit}{{3.2}{143}{Lower limits on S/N required to detect and measure spectral features\relax }{table.caption.63}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.3.2.2}Aperture losses}{144}{subsubsection.3.3.2.2}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.3.2.3}Air mass}{144}{subsubsection.3.3.2.3}}
\newlabel{airmass}{{3.2}{144}{Air mass}{equation.3.3.2}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.3.2.4}Atmospheric refraction }{144}{subsubsection.3.3.2.4}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.5}{\ignorespaces Atmospheric refraction}}{145}{figure.caption.64}}
\newlabel{C3_Fig_atmospheric_refraction}{{3.5}{145}{Atmospheric refraction}{figure.caption.64}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3.3}Minimizing the impact of the sky background}{146}{subsection.3.3.3}}
\newlabel{C3_Prepare_Sky}{{3.3.3}{146}{Minimizing the impact of the sky background}{subsection.3.3.3}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.6}{\ignorespaces Components of the night sky spectrum}}{147}{figure.caption.66}}
\newlabel{C3_Fig_Sky_bg}{{3.6}{147}{Components of the night sky spectrum}{figure.caption.66}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.7}{\ignorespaces Night sky spectrum}}{147}{figure.caption.67}}
\newlabel{C3_Fig_Sky_spectrum}{{3.7}{147}{Night sky spectrum}{figure.caption.67}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.8}{\ignorespaces Percentage of the spectral band available between OH sky lines}}{149}{figure.caption.69}}
\newlabel{C3_Sky_R}{{3.8}{149}{Percentage of the spectral band available between OH sky lines}{figure.caption.69}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.9}{\ignorespaces  Sky subtraction observational strategies}}{150}{figure.caption.70}}
\newlabel{C3_Fig_Sky_strategies}{{3.9}{150}{Sky subtraction observational strategies}{figure.caption.70}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.3.3.1}Water vapor column constrain}{150}{subsubsection.3.3.3.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.10}{\ignorespaces Transmission and emission of the atmosphere in the near IR bands. }}{151}{figure.caption.71}}
\newlabel{C3_Fig_PWV}{{3.10}{151}{Transmission and emission of the atmosphere in the near IR bands}{figure.caption.71}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3.4}Data reduction}{152}{section.3.4}}
\newlabel{C3_Data_analysis}{{3.4}{152}{Data reduction}{section.3.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.4.1}Main steps}{152}{subsection.3.4.1}}
\newlabel{C3_Data_analysis_main_steps}{{3.4.1}{152}{Main steps}{subsection.3.4.1}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.2}\hspace  {2.5em}The importance of being flux calibrated}{152}{example.3.2}}
%\zref@newlabel{mdf@pagelabel-42}{\default{3.2}\page{152}\abspage{173}\mdf@pagevalue{152}}
%\pgfsyspdfmark {pgfid42}{8922493}{11400698}
%\zref@newlabel{mdf@pagelabel-43}{\default{3.2}\page{153}\abspage{174}\mdf@pagevalue{153}}
%\pgfsyspdfmark {pgfid43}{8922493}{33357526}
\@writefile{lof}{\contentsline {figure}{\numberline {3.11}{\ignorespaces Extinction corrected from flux ratio versus equivalent width ratios}}{153}{figure.caption.73}}
\newlabel{C3_Fig_EW_metals}{{3.11}{153}{Extinction corrected from flux ratio versus equivalent width ratios}{figure.caption.73}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.3}\hspace  {2.5em}How to correct a spectrum from telluric absorption lines}{154}{example.3.3}}
%\zref@newlabel{mdf@pagelabel-44}{\default{3.3}\page{154}\abspage{175}\mdf@pagevalue{154}}
%\pgfsyspdfmark {pgfid44}{8922493}{11595934}
%\zref@newlabel{mdf@pagelabel-45}{\default{3.3}\page{155}\abspage{176}\mdf@pagevalue{155}}
%\pgfsyspdfmark {pgfid45}{8922493}{41189078}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.4.2}Characterize the quality of the data reduction}{155}{subsection.3.4.2}}
\newlabel{C3_Data_analysis_Qualite}{{3.4.2}{155}{Characterize the quality of the data reduction}{subsection.3.4.2}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.4.2.1}Effective spectral resolution and wavelength calibration accuracy}{155}{subsubsection.3.4.2.1}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.4.2.2}Signal-to-noise ratio of detection}{156}{subsubsection.3.4.2.2}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.4.2.3}Spectrophotometry and Aperture correction}{156}{subsubsection.3.4.2.3}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.4}\hspace  {2.5em}Fast method to control spectrophotometry using independent photometry}{156}{example.3.4}}
%\zref@newlabel{mdf@pagelabel-46}{\default{3.4}\page{157}\abspage{178}\mdf@pagevalue{157}}
%\pgfsyspdfmark {pgfid46}{8922493}{32502656}
\@writefile{lof}{\contentsline {figure}{\numberline {3.12}{\ignorespaces Spectrophotometric accuracy}}{157}{figure.caption.75}}
\newlabel{C3_Fig_photo_calib}{{3.12}{157}{Spectrophotometric accuracy}{figure.caption.75}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3.5}Emission lines}{158}{section.3.5}}
\newlabel{C3_Emission_lines}{{3.5}{158}{Emission lines}{section.3.5}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.5.1}Emission line properties}{158}{subsection.3.5.1}}
\newlabel{C3_Emission_lines_properties}{{3.5.1}{158}{Emission line properties}{subsection.3.5.1}{}}
\newlabel{C3_sigma_prop}{{3.5}{159}{Emission line properties}{equation.3.5.5}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.13}{\ignorespaces Emission line profiles}}{159}{figure.caption.76}}
\newlabel{C3_Fig_Line_Profiles}{{3.13}{159}{Emission line profiles}{figure.caption.76}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.5.2}Proper methods for measuring emission lines}{160}{subsection.3.5.2}}
\newlabel{C3_Emission_lines_measures}{{3.5.2}{160}{Proper methods for measuring emission lines}{subsection.3.5.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.14}{\ignorespaces Measure emission lines with {\sc  iraf}}}{160}{figure.caption.77}}
\newlabel{C3_Fig_Emission_iraf}{{3.14}{160}{Measure emission lines with {\sc iraf}}{figure.caption.77}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.15}{\ignorespaces Correcting from underlying absorption}}{161}{figure.caption.78}}
\newlabel{C3_Fig_Spectra_with_continum}{{3.15}{161}{Correcting from underlying absorption}{figure.caption.78}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.5}\hspace  {2.5em}Correcting from underlying absorption}{161}{example.3.5}}
%\zref@newlabel{mdf@pagelabel-47}{\default{3.5}\page{162}\abspage{183}\mdf@pagevalue{162}}
%\pgfsyspdfmark {pgfid47}{8922493}{11290099}
%\zref@newlabel{mdf@pagelabel-48}{\default{3.5}\page{163}\abspage{184}\mdf@pagevalue{163}}
%\pgfsyspdfmark {pgfid48}{8922493}{15630038}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.5.3}Low signal-to-noise regime: measurement bias}{164}{subsection.3.5.3}}
\newlabel{C3_Emission_lowSN}{{3.5.3}{164}{Low signal-to-noise regime: measurement bias}{subsection.3.5.3}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3.6}Emission diagnostics of the ionized ISM}{165}{section.3.6}}
\newlabel{C3_EmissionDiagnostics}{{3.6}{165}{Emission diagnostics of the ionized ISM}{section.3.6}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.6.1}Dust extinction}{165}{subsection.3.6.1}}
\newlabel{C3_EmissionDiagnostics_Dust}{{3.6.1}{165}{Dust extinction}{subsection.3.6.1}{}}
\newlabel{C3_Extinction}{{3.6.1}{165}{Dust extinction}{subsection.3.6.1}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.16}{\ignorespaces Flux limit of a non-detected line}}{166}{figure.caption.79}}
\newlabel{C3_Flux_limit}{{3.16}{166}{Flux limit of a non-detected line}{figure.caption.79}{}}
\newlabel{eq:optical_depth_abs}{{3.7}{166}{Extinction laws}{equation.3.6.7}{}}
\newlabel{eq:flux_dust_c}{{3.9}{167}{Extinction laws}{equation.3.6.9}{}}
\newlabel{eq:optical_depth_abs_A}{{3.10}{167}{Extinction laws}{equation.3.6.10}{}}
\@writefile{lot}{\contentsline {table}{\numberline {3.3}{\ignorespaces Values of the extinction curve at different wavelengths and for several extinction laws\relax }}{168}{table.caption.81}}
\newlabel{C3_Table_Extinction_law}{{3.3}{168}{Values of the extinction curve at different wavelengths and for several extinction laws\relax }{table.caption.81}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.17}{\ignorespaces Interstellar extinction curves }}{169}{figure.caption.82}}
\newlabel{C3_Fig_Extinction_law}{{3.17}{169}{Interstellar extinction curves}{figure.caption.82}{}}
\@writefile{lot}{\contentsline {table}{\numberline {3.4}{\ignorespaces Theoretical Balmer ratios\relax }}{169}{table.caption.84}}
\newlabel{C3_Table_Balmer_ratio}{{3.4}{169}{Theoretical Balmer ratios\relax }{table.caption.84}{}}
\newlabel{eq:IR-Hb}{{3.12}{169}{Global balance between IR and UV-$H\alpha $ SFR}{equation.3.6.12}{}}
\newlabel{eq:IR-UV}{{3.13}{170}{Global balance between IR and UV-$H\alpha $ SFR}{equation.3.6.13}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.18}{\ignorespaces  Relation between the extinction $A_V$ values derived by Balmer decrement and by SFR ratio }}{171}{figure.caption.86}}
\newlabel{C3_Fig_Extinction_FORS2}{{3.18}{171}{Relation between the extinction $A_V$ values derived by Balmer decrement and by SFR ratio}{figure.caption.86}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.6}\hspace  {2.5em}How to choose the extinction law in a compact distant galaxy}{172}{example.3.6}}
%\zref@newlabel{mdf@pagelabel-49}{\default{3.6}\page{172}\abspage{193}\mdf@pagevalue{172}}
%\pgfsyspdfmark {pgfid49}{8922493}{11304212}
%\zref@newlabel{mdf@pagelabel-50}{\default{3.6}\page{173}\abspage{194}\mdf@pagevalue{173}}
%\pgfsyspdfmark {pgfid50}{8922493}{39357711}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.6.2}Active galactic nuclei}{173}{subsection.3.6.2}}
\newlabel{C3_EmissionDiagnostics_AGN}{{3.6.2}{173}{Active galactic nuclei}{subsection.3.6.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.19}{\ignorespaces BPT diagnostic diagram}}{175}{figure.caption.91}}
\newlabel{C3_Fig_AGN_K03}{{3.19}{175}{BPT diagnostic diagram}{figure.caption.91}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.20}{\ignorespaces  Diagnostic diagram OII 3727/Hb vs OIII4959, 5007/Hb }}{176}{figure.caption.92}}
\newlabel{C3_Fig_AGN_FORS}{{3.20}{176}{Diagnostic diagram OII 3727/Hb vs OIII4959, 5007/Hb}{figure.caption.92}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.6.3}Star formation rates}{177}{subsection.3.6.3}}
\newlabel{C3_EmissionDiagnostics_SFR}{{3.6.3}{177}{Star formation rates}{subsection.3.6.3}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.6.3.1}Star formation rate from the H$\alpha $ line}{177}{subsubsection.3.6.3.1}}
\newlabel{C3_SFRHalpha}{{3.14}{177}{Star formation rate from the H$\alpha $ line}{equation.3.6.14}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.7}\hspace  {2.5em}Can we estimate SFR from the [\MakeUppercase  {O$\tmspace  +\thickmuskip {.2777em}$\textsc  {\rmfamily  ii}\relax }] line?}{177}{example.3.7}}
%\zref@newlabel{mdf@pagelabel-51}{\default{3.7}\page{178}\abspage{199}\mdf@pagevalue{178}}
%\pgfsyspdfmark {pgfid51}{8922493}{19930662}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.6.3.2}Star formation rate from the Ly$\alpha $ line}{178}{subsubsection.3.6.3.2}}
\newlabel{Ly_SFR}{{3.16}{179}{Star formation rate from the Ly$\alpha $ line}{equation.3.6.16}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.6.4}Direct measurement of the gas metallicity ($T_\mathrm  {e}$ method)}{179}{subsection.3.6.4}}
\newlabel{C3_EmissionDiagnostics_directMetals}{{3.6.4}{179}{Direct measurement of the gas metallicity ($T_\mathrm {e}$ method)}{subsection.3.6.4}{}}
\newlabel{Eq:total_abundance}{{3.17}{180}{Direct measurement of the gas metallicity ($T_\mathrm {e}$ method)}{equation.3.6.17}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.8}\hspace  {2.5em}Metallicities from effective temperature}{181}{example.3.8}}
%\zref@newlabel{mdf@pagelabel-52}{\default{3.8}\page{181}\abspage{202}\mdf@pagevalue{181}}
%\pgfsyspdfmark {pgfid52}{8922493}{12502515}
%\zref@newlabel{mdf@pagelabel-53}{\default{3.8}\page{182}\abspage{203}\mdf@pagevalue{182}}
\newlabel{Eq:metal_OIII}{{3.19}{182}{Direct measurement of the gas metallicity ($T_\mathrm {e}$ method)}{equation.3.6.19}{}}
%\pgfsyspdfmark {pgfid53}{8922493}{12231853}
%\zref@newlabel{mdf@pagelabel-54}{\default{3.8}\page{183}\abspage{204}\mdf@pagevalue{183}}
%\pgfsyspdfmark {pgfid54}{8922493}{41025238}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.6.4.1}Limitations of the $T_\mathrm  {e}$ method for distant galaxies}{183}{subsubsection.3.6.4.1}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.6.5}Indirect metallicity estimates from strong line ratios}{183}{subsection.3.6.5}}
\newlabel{C3_EmissionDiagnostics_StrongRatioMetals}{{3.6.5}{183}{Indirect metallicity estimates from strong line ratios}{subsection.3.6.5}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.21}{\ignorespaces R23 calibration}}{184}{figure.caption.95}}
\newlabel{C3_Fig_R23_Z}{{3.21}{184}{R23 calibration}{figure.caption.95}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.9}\hspace  {2.5em}Estimating metallicities using $\mathrm  {R_{23}}$}{184}{example.3.9}}
%\zref@newlabel{mdf@pagelabel-55}{\default{3.9}\page{185}\abspage{206}\mdf@pagevalue{185}}
%\pgfsyspdfmark {pgfid55}{8922493}{27088650}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.10}\hspace  {2.5em}Limitations of the ${N_2}$ parameter}{185}{example.3.10}}
%\zref@newlabel{mdf@pagelabel-56}{\default{3.10}\page{185}\abspage{206}\mdf@pagevalue{185}}
%\pgfsyspdfmark {pgfid56}{8922493}{11877300}
%\zref@newlabel{mdf@pagelabel-57}{\default{3.10}\page{186}\abspage{207}\mdf@pagevalue{186}}
%\pgfsyspdfmark {pgfid57}{8922493}{35097871}
\@writefile{lof}{\contentsline {figure}{\numberline {3.22}{\ignorespaces Abundance derived from Te vs strong line calibrations}}{187}{figure.caption.98}}
\newlabel{C3_Fig_correlation_method}{{3.22}{187}{Abundance derived from Te vs strong line calibrations}{figure.caption.98}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3.7}Absorption line diagnostics of ISM \& IGM}{187}{section.3.7}}
\newlabel{C3_AbsorptionDiagnostics}{{3.7}{187}{Absorption line diagnostics of ISM \& IGM}{section.3.7}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.23}{\ignorespaces The ISM from the UV lines. }}{188}{figure.caption.99}}
\newlabel{C3_Fig_UV_ISM}{{3.23}{188}{The ISM from the UV lines}{figure.caption.99}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.7.1}Measuring absorption lines}{189}{subsection.3.7.1}}
\newlabel{C3_AbsorptionDiagnostics_Measure}{{3.7.1}{189}{Measuring absorption lines}{subsection.3.7.1}{}}
\newlabel{eq:tau}{{3.24}{189}{Measuring absorption lines}{equation.3.7.24}{}}
\newlabel{eq:EW}{{3.25}{190}{Equivalent width}{equation.3.7.25}{}}
\newlabel{eq:EW}{{3.26}{190}{Equivalent width}{equation.3.7.26}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.11}\hspace  {2.5em}Measuring an equivalent width}{190}{example.3.11}}
%\zref@newlabel{mdf@pagelabel-58}{\default{3.11}\page{190}\abspage{211}\mdf@pagevalue{190}}
%\pgfsyspdfmark {pgfid58}{8922493}{23185328}
\@writefile{lof}{\contentsline {figure}{\numberline {3.24}{\ignorespaces Curve of growth for HI $\lambda $1215\nobreakspace  {}\r A,(Lyman-$\alpha $). }}{191}{figure.caption.102}}
\newlabel{C3_Fig_HI_growth}{{3.24}{191}{Curve of growth for HI $\lambda $1215~\AA ,(Lyman-$\alpha $)}{figure.caption.102}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.7.2} Back-illuminated neutral Hydrogen gas }{192}{subsection.3.7.2}}
\newlabel{C3_AbsorptionDiagnostics_NeutralGas}{{3.7.2}{192}{Back-illuminated neutral Hydrogen gas}{subsection.3.7.2}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.12}\hspace  {2.5em}The Ly$\alpha $ forest and the Gunn-Peterson trough}{192}{example.3.12}}
%\zref@newlabel{mdf@pagelabel-59}{\default{3.12}\page{192}\abspage{213}\mdf@pagevalue{192}}
%\pgfsyspdfmark {pgfid59}{8922493}{23938727}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.7.2.1}Damped Lyman Absorbers }{192}{subsubsection.3.7.2.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.25}{\ignorespaces Gunn-Peterson : Spectra of high-z Quasar }}{193}{figure.caption.103}}
\newlabel{C3_Fig_Gunn_Peterson}{{3.25}{193}{Gunn-Peterson : Spectra of high-z Quasar}{figure.caption.103}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.7.2.2}The H$\tmspace  +\thickmuskip {.2777em}$\textsc  {\rmfamily  i}\relax  column density in DLAs}{193}{subsubsection.3.7.2.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.26}{\ignorespaces Lyman Alpha line of a distant lensed galaxy }}{194}{figure.caption.104}}
\newlabel{C3_Lyman_alpha_line_fit}{{3.26}{194}{Lyman Alpha line of a distant lensed galaxy}{figure.caption.104}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.7.2.3}Abundances and metallicities in H$\tmspace  +\thickmuskip {.2777em}$\textsc  {\rmfamily  i}\relax  clouds }{194}{subsubsection.3.7.2.3}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.27}{\ignorespaces Column density of metals from Voigt profile fitting }}{195}{figure.caption.105}}
\newlabel{C3_Fig_Voigt_fit}{{3.27}{195}{Column density of metals from Voigt profile fitting}{figure.caption.105}{}}
\newlabel{eq:tau_nu}{{3.30}{195}{Abundances and metallicities in \ion {H}{1} clouds}{equation.3.7.30}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.28}{\ignorespaces Curves of growth for the ions}}{196}{figure.caption.106}}
\newlabel{C3_Fig_COG_metal}{{3.28}{196}{Curves of growth for the ions}{figure.caption.106}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.29}{\ignorespaces The effect of spectral resolution on the profile of absorption lines. }}{197}{figure.caption.107}}
\newlabel{C3_Fig_Resolution_absorption_lines}{{3.29}{197}{The effect of spectral resolution on the profile of absorption lines}{figure.caption.107}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.13}\hspace  {2.5em}How to check the saturation of a line}{197}{example.3.13}}
%\zref@newlabel{mdf@pagelabel-60}{\default{3.13}\page{198}\abspage{219}\mdf@pagevalue{198}}
%\pgfsyspdfmark {pgfid60}{8922493}{36187231}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.7.3}Absorption lines from the ISM of distant starbursts}{199}{subsection.3.7.3}}
\newlabel{C3_AbsorptionDiagnostics_AbsISM}{{3.7.3}{199}{Absorption lines from the ISM of distant starbursts}{subsection.3.7.3}{}}
\newlabel{C3_lyalpha}{{3.7.3.1}{200}{Ly$\alpha $ properties of distant starbursts}{subsubsection.3.7.3.1}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.7.3.1}Ly$\alpha $ properties of distant starbursts}{200}{subsubsection.3.7.3.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.30}{\ignorespaces Lyman alpha profile }}{201}{figure.caption.110}}
\newlabel{C3_Fig_LyaLines_profile}{{3.30}{201}{Lyman alpha profile}{figure.caption.110}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {3.7.3.2}Gas motions}{201}{subsubsection.3.7.3.2}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.14}\hspace  {2.5em}Large scale outflows in Lyman Break Galaxies}{202}{example.3.14}}
%\zref@newlabel{mdf@pagelabel-61}{\default{3.14}\page{202}\abspage{223}\mdf@pagevalue{202}}
%\pgfsyspdfmark {pgfid61}{8922493}{11197615}
\@writefile{lof}{\contentsline {figure}{\numberline {3.31}{\ignorespaces Outflow from UV inter-stellar lines }}{203}{figure.caption.111}}
\newlabel{C3_Fig_UV_outlow}{{3.31}{203}{Outflow from UV inter-stellar lines}{figure.caption.111}{}}
%\zref@newlabel{mdf@pagelabel-62}{\default{3.14}\page{203}\abspage{224}\mdf@pagevalue{203}}
%\pgfsyspdfmark {pgfid62}{8922493}{11768977}
%\zref@newlabel{mdf@pagelabel-63}{\default{3.14}\page{204}\abspage{225}\mdf@pagevalue{204}}
%\pgfsyspdfmark {pgfid63}{8922493}{36929238}
\@writefile{lof}{\contentsline {figure}{\numberline {3.32}{\ignorespaces Large-scale outflows in star-forming galaxies }}{204}{figure.caption.112}}
\newlabel{C3_Fig_outflows_Ly}{{3.32}{204}{Large-scale outflows in star-forming galaxies}{figure.caption.112}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3.8}Properties of stellar populations}{205}{section.3.8}}
\newlabel{C3_PropertiesStellarPopulations}{{3.8}{205}{Properties of stellar populations}{section.3.8}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.33}{\ignorespaces Breaking the age-metallicity degeneracy with the spectral information}}{206}{figure.caption.113}}
\newlabel{C3_Fig_ageZdege}{{3.33}{206}{Breaking the age-metallicity degeneracy with the spectral information}{figure.caption.113}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.8.1}Spectral Evolution of single stellar populations}{206}{subsection.3.8.1}}
\newlabel{C3_PropertiesStellarPopulations_SpectralEvolution}{{3.8.1}{206}{Spectral Evolution of single stellar populations}{subsection.3.8.1}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.15}\hspace  {2.5em}Identifying WR features}{207}{example.3.15}}
%\zref@newlabel{mdf@pagelabel-64}{\default{3.15}\page{207}\abspage{228}\mdf@pagevalue{207}}
%\pgfsyspdfmark {pgfid64}{8922493}{11493989}
\@writefile{lof}{\contentsline {figure}{\numberline {3.34}{\ignorespaces Spectra of SSP as a function of age and metallicity}}{208}{figure.caption.114}}
\newlabel{C3_Fig_SSP_age_Z_Vadzeli}{{3.34}{208}{Spectra of SSP as a function of age and metallicity}{figure.caption.114}{}}
%\zref@newlabel{mdf@pagelabel-65}{\default{3.15}\page{208}\abspage{229}\mdf@pagevalue{208}}
%\pgfsyspdfmark {pgfid65}{8922493}{11498742}
%\zref@newlabel{mdf@pagelabel-66}{\default{3.15}\page{209}\abspage{230}\mdf@pagevalue{209}}
%\pgfsyspdfmark {pgfid66}{8922493}{38505743}
\@writefile{lof}{\contentsline {figure}{\numberline {3.35}{\ignorespaces Blue bump in combined spectrum of the 5 GRB host }}{209}{figure.caption.115}}
\newlabel{WR_bump}{{3.35}{209}{Blue bump in combined spectrum of the 5 GRB host}{figure.caption.115}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.8.2}Lick indices}{209}{subsection.3.8.2}}
\newlabel{C3_PropertiesStellarPopulations_LickIndices}{{3.8.2}{209}{Lick indices}{subsection.3.8.2}{}}
\newlabel{RF5}{210}
\@writefile{lot}{\contentsline {table}{\numberline {3.5}{\ignorespaces Definition of Lick indices\relax }}{210}{table.caption.116}}
\newlabel{C3_Tab_lick_def}{{3.5}{210}{Definition of Lick indices\relax }{table.caption.116}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3.36}{\ignorespaces Definition of spectral index}}{211}{figure.caption.117}}
\newlabel{C3_Fig_Spectral_Indice_def}{{3.36}{211}{Definition of spectral index}{figure.caption.117}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.16}\hspace  {2.5em}Measure a Lick index}{212}{example.3.16}}
%\zref@newlabel{mdf@pagelabel-67}{\default{3.16}\page{212}\abspage{233}\mdf@pagevalue{212}}
%\pgfsyspdfmark {pgfid67}{8922493}{11490320}
%\zref@newlabel{mdf@pagelabel-68}{\default{3.16}\page{213}\abspage{234}\mdf@pagevalue{213}}
%\pgfsyspdfmark {pgfid68}{8922493}{39321302}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.8.3}Full spectra fitting}{213}{subsection.3.8.3}}
\newlabel{C3_PropertiesStellarPopulations_FullSpectraFitting}{{3.8.3}{213}{Full spectra fitting}{subsection.3.8.3}{}}
\newlabel{eq:full spectra fitting}{{3.34}{213}{Full spectra fitting}{equation.3.8.34}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}3.17}\hspace  {2.5em}Estimating a coarse SFH of a distant galaxy}{215}{example.3.17}}
%\zref@newlabel{mdf@pagelabel-69}{\default{3.17}\page{215}\abspage{236}\mdf@pagevalue{215}}
%\pgfsyspdfmark {pgfid69}{8922493}{11102482}
\@writefile{lof}{\contentsline {figure}{\numberline {3.37}{\ignorespaces  Full-spectra fitting of a distant galaxy}}{216}{figure.caption.119}}
\newlabel{C3_Full_spectra_fitting_45.11}{{3.37}{216}{Full-spectra fitting of a distant galaxy}{figure.caption.119}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.8.4}Velocity dispersion }{217}{subsection.3.8.4}}
\newlabel{C3_PropertiesStellarPopulations_VelocityDispersion}{{3.8.4}{217}{Velocity dispersion}{subsection.3.8.4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3.9}Conclusion}{217}{section.3.9}}
\newlabel{C3_Conclusion}{{3.9}{217}{Conclusion}{section.3.9}{}}
\@writefile{lot}{\contentsline {table}{\numberline {3.6}{\ignorespaces Robust determination of physical quantities of distant galaxies\relax }}{218}{table.caption.122}}
\newlabel{C3_Tab_Robust_deter}{{3.6}{218}{Robust determination of physical quantities of distant galaxies\relax }{table.caption.122}{}}
\gdef\bu@bibdata{C4_3Dspectro}
\@writefile{lof}{\addvspace {10\p@ }}
\@writefile{lot}{\addvspace {10\p@ }}
\@writefile{toc}{\contentsline {chapter}{\hbox to\@tempdima {4.\hfil }Integral Field Spectroscopy}{226}{chapter.4}}
\@writefile{toc}{\contentsline {section}{\numberline {4.1}Introduction}{226}{section.4.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.1}{\ignorespaces 3D data-cube}}{227}{figure.caption.124}}
\newlabel{C4_data-cube}{{4.1}{227}{3D data-cube}{figure.caption.124}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.2}{\ignorespaces Main techniques of IFU instruments}}{228}{figure.caption.125}}
\newlabel{C4_IFU_principle}{{4.2}{228}{Main techniques of IFU instruments}{figure.caption.125}{}}
\@writefile{toc}{\contentsline {section}{\numberline {4.2}Basics of IFU instruments}{229}{section.4.2}}
\newlabel{C4_selecting_IFU}{{4.2}{229}{Basics of IFU instruments}{section.4.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2.1}Fiber instruments}{229}{subsection.4.2.1}}
\newlabel{C4_fiber_IFU}{{4.2.1}{229}{Fiber instruments}{subsection.4.2.1}{}}
\newlabel{RF6}{230}
\@writefile{lot}{\contentsline {table}{\numberline {4.1}{\ignorespaces Main characteristics of the integral field units installed on 8m class telescopes.\relax }}{230}{table.caption.126}}
\newlabel{C4_3DtablelistIFU}{{4.1}{230}{Main characteristics of the integral field units installed on 8m class telescopes.\relax }{table.caption.126}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.3}{\ignorespaces Example of fiber array.}}{231}{figure.caption.127}}
\newlabel{C4_figarrayexample}{{4.3}{231}{Example of fiber array}{figure.caption.127}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2.2}Image slicer instruments}{231}{subsection.4.2.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.4}{\ignorespaces Image slicer technique.}}{232}{figure.caption.128}}
\newlabel{C4_slicearratimage}{{4.4}{232}{Image slicer technique}{figure.caption.128}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2.3}Compromise between resolutions and S/N}{232}{subsection.4.2.3}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.5}{\ignorespaces Impact of spatial resolution.}}{233}{figure.caption.129}}
\newlabel{C4_3Dexamplespaxels}{{4.5}{233}{Impact of spatial resolution}{figure.caption.129}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2.4}Spatial resolution}{234}{subsection.4.2.4}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.6}{\ignorespaces Spatial cross-talk}}{234}{figure.caption.130}}
\newlabel{C4_seeingsurrpave}{{4.6}{234}{Spatial cross-talk}{figure.caption.130}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.1}\hspace  {2.5em}High spatial resolution kinematics of high-z galaxies}{234}{example.4.1}}
%\zref@newlabel{mdf@pagelabel-70}{\default{4.1}\page{235}\abspage{256}\mdf@pagevalue{235}}
%\pgfsyspdfmark {pgfid70}{8922493}{31774474}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2.5}Spectral resolution and cross-talk}{235}{subsection.4.2.5}}
\newlabel{C4_spec_cross_talk}{{4.2.5}{235}{Spectral resolution and cross-talk}{subsection.4.2.5}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.2}\hspace  {2.5em}Small cross-talk or large field of view?}{235}{example.4.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.7}{\ignorespaces Example of AO observations}}{236}{figure.caption.131}}
\newlabel{C4_3DAGN}{{4.7}{236}{Example of AO observations}{figure.caption.131}{}}
%\zref@newlabel{mdf@pagelabel-71}{\default{4.2}\page{236}\abspage{257}\mdf@pagevalue{236}}
%\pgfsyspdfmark {pgfid71}{8922493}{11260939}
\@writefile{lof}{\contentsline {figure}{\numberline {4.8}{\ignorespaces Impact of spectral resolution on sky line removal}}{237}{figure.caption.132}}
\newlabel{C4_3Dfigfitandres}{{4.8}{237}{Impact of spectral resolution on sky line removal}{figure.caption.132}{}}
%\zref@newlabel{mdf@pagelabel-72}{\default{4.2}\page{237}\abspage{258}\mdf@pagevalue{237}}
%\pgfsyspdfmark {pgfid72}{8922493}{12536155}
\@writefile{lof}{\contentsline {figure}{\numberline {4.9}{\ignorespaces Fiber-to-fiber spectral cross-talk.}}{238}{figure.caption.133}}
\newlabel{C4_3DGIRAFFEcrosstalk}{{4.9}{238}{Fiber-to-fiber spectral cross-talk}{figure.caption.133}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2.6}Observing with IFU instruments}{238}{subsection.4.2.6}}
\newlabel{C4_IFU_observing}{{4.2.6}{238}{Observing with IFU instruments}{subsection.4.2.6}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.2.6.1}Astrometry}{238}{subsubsection.4.2.6.1}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.2.6.2}Observational strategy}{238}{subsubsection.4.2.6.2}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.3}\hspace  {2.5em}Strategy for reducing the sky signal with IFUs}{239}{example.4.3}}
%\zref@newlabel{mdf@pagelabel-73}{\default{4.3}\page{239}\abspage{260}\mdf@pagevalue{239}}
%\pgfsyspdfmark {pgfid73}{8922493}{31816341}
\@writefile{toc}{\contentsline {section}{\numberline {4.3}Data reduction of IFU observations}{239}{section.4.3}}
\newlabel{C4_datared_3D}{{4.3}{239}{Data reduction of IFU observations}{section.4.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3.1}Reduction of fiber data}{239}{subsection.4.3.1}}
\newlabel{C4_reduc_fiber}{{4.3.1}{239}{Reduction of fiber data}{subsection.4.3.1}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.10}{\ignorespaces Raw data images from image slicers and fibers}}{240}{figure.caption.134}}
\newlabel{C4_3Dfmtdata}{{4.10}{240}{Raw data images from image slicers and fibers}{figure.caption.134}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.3.1.1}Fiber to fiber response and sky subtraction}{240}{subsubsection.4.3.1.1}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.3.1.2}Correction of cross-talk}{241}{subsubsection.4.3.1.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3.2}Reduction of image slicer data}{241}{subsection.4.3.2}}
\newlabel{C4_reduc_slicer}{{4.3.2}{241}{Reduction of image slicer data}{subsection.4.3.2}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.3.2.1}Alignment of slices and PSF}{241}{subsubsection.4.3.2.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.11}{\ignorespaces Profile of 3 slices with different responses}}{242}{figure.caption.135}}
\newlabel{C4_3Dfigslicerreponse}{{4.11}{242}{Profile of 3 slices with different responses}{figure.caption.135}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.3.2.2}Possible problems with image slicers}{242}{subsubsection.4.3.2.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3.3}Correcting for atmospheric dispersion}{242}{subsection.4.3.3}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.12}{\ignorespaces Cross talk on adjacent slits of SINFONI}}{243}{figure.caption.136}}
\newlabel{C4_3DSINFONIcrosstalkCCD}{{4.12}{243}{Cross talk on adjacent slits of SINFONI}{figure.caption.136}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3.4}Spatial, spectral smoothing and binning}{243}{subsection.4.3.4}}
\newlabel{C4_sec:spectralsmooth}{{4.3.4}{243}{Spatial, spectral smoothing and binning}{subsection.4.3.4}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.3.4.1}Spatial smoothing}{243}{subsubsection.4.3.4.1}}
\newlabel{C4_spatialsmooth}{{4.3.4.1}{243}{Spatial smoothing}{subsubsection.4.3.4.1}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.13}{\ignorespaces An example of correction for atmospheric dispersion}}{244}{figure.caption.137}}
\newlabel{C4_3Dfigaligncorr}{{4.13}{244}{An example of correction for atmospheric dispersion}{figure.caption.137}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.3.4.2}Spectral smoothing}{244}{subsubsection.4.3.4.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.14}{\ignorespaces Effect of smoothing algorithms}}{245}{figure.caption.138}}
\newlabel{C4_3Deffectsmooth}{{4.14}{245}{Effect of smoothing algorithms}{figure.caption.138}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3.5}Optimizing sky subtraction with NIR IFUs}{245}{subsection.4.3.5}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.15}{\ignorespaces Variation of OH sky lines within a KMOS data cube}}{246}{figure.caption.139}}
\newlabel{C4_figSkyKMOS}{{4.15}{246}{Variation of OH sky lines within a KMOS data cube}{figure.caption.139}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.4}\hspace  {2.5em}Optimizing emission line S/N in the near-IR at moderate resolution (KMOS)}{246}{example.4.4}}
%\zref@newlabel{mdf@pagelabel-74}{\default{4.4}\page{246}\abspage{267}\mdf@pagevalue{246}}
%\pgfsyspdfmark {pgfid74}{8922493}{11501439}
%\zref@newlabel{mdf@pagelabel-75}{\default{4.4}\page{247}\abspage{268}\mdf@pagevalue{247}}
%\pgfsyspdfmark {pgfid75}{8922493}{18910479}
\@writefile{toc}{\contentsline {section}{\numberline {4.4}Mapping galaxy properties from a data-cube}{247}{section.4.4}}
\newlabel{C4_3D_cube}{{4.4}{247}{Mapping galaxy properties from a data-cube}{section.4.4}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.16}{\ignorespaces Optimization of the S/N for KMOS observations}}{248}{figure.caption.140}}
\newlabel{C4_3DfigKMOS}{{4.16}{248}{Optimization of the S/N for KMOS observations}{figure.caption.140}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.4.1}Measuring emission lines: methods and error budget}{248}{subsection.4.4.1}}
\newlabel{C4_sec:emmlines}{{4.4.1}{248}{Measuring emission lines: methods and error budget}{subsection.4.4.1}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.5}\hspace  {2.5em}Fitting 3 lines together}{249}{example.4.5}}
%\zref@newlabel{mdf@pagelabel-76}{\default{4.5}\page{249}\abspage{270}\mdf@pagevalue{249}}
%\pgfsyspdfmark {pgfid76}{8922493}{25474125}
\@writefile{lof}{\contentsline {figure}{\numberline {4.17}{\ignorespaces Example of a multiple line fit}}{250}{figure.caption.141}}
\newlabel{C4_HaNII}{{4.17}{250}{Example of a multiple line fit}{figure.caption.141}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.4.2}Mapping physical properties}{251}{subsection.4.4.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.4.3}Mapping the kinematics}{251}{subsection.4.4.3}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.18}{\ignorespaces Star formation map of a distant GRB host galaxy}}{252}{figure.caption.142}}
\newlabel{C4_XS_SFR}{{4.18}{252}{Star formation map of a distant GRB host galaxy}{figure.caption.142}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.6}\hspace  {2.5em}Simulations to set the S/N threshold of the velocity dispersion}{252}{example.4.6}}
%\zref@newlabel{mdf@pagelabel-77}{\default{4.6}\page{252}\abspage{273}\mdf@pagevalue{252}}
%\pgfsyspdfmark {pgfid77}{8922493}{11678410}
\@writefile{lof}{\contentsline {figure}{\numberline {4.19}{\ignorespaces Electron density maps of distant galaxies}}{253}{figure.caption.143}}
\newlabel{C4_figelecdens}{{4.19}{253}{Electron density maps of distant galaxies}{figure.caption.143}{}}
%\zref@newlabel{mdf@pagelabel-78}{\default{4.6}\page{253}\abspage{274}\mdf@pagevalue{253}}
%\pgfsyspdfmark {pgfid78}{8922493}{19961633}
\@writefile{toc}{\contentsline {section}{\numberline {4.5}Kinematics of distant galaxies}{253}{section.4.5}}
\newlabel{C4_kinematics}{{4.5}{253}{Kinematics of distant galaxies}{section.4.5}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.5.1}A fundamental reference: kinematics of nearby galaxies}{253}{subsection.4.5.1}}
\newlabel{C4_fundref}{{4.5.1}{253}{A fundamental reference: kinematics of nearby galaxies}{subsection.4.5.1}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.20}{\ignorespaces Dependence of the $\sigma $ error on S/N}}{254}{figure.caption.144}}
\newlabel{C4_simspecmc}{{4.20}{254}{Dependence of the $\sigma $ error on S/N}{figure.caption.144}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.5.1.1}Modeling the velocity fields of rotating disks}{255}{subsubsection.4.5.1.1}}
\newlabel{C4_rqrc}{{4.3}{255}{Modeling the velocity fields of rotating disks}{equation.4.5.3}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.21}{\ignorespaces Kinemetric parameters for rotating disks and mergers}}{256}{figure.caption.145}}
\newlabel{C4_kinemetry}{{4.21}{256}{Kinemetric parameters for rotating disks and mergers}{figure.caption.145}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.5.1.2}Kinematic analysis of galaxies: "kinemetry"}{256}{subsubsection.4.5.1.2}}
\newlabel{C4_kinemetrydecomp}{{4.5.1.2}{256}{Kinematic analysis of galaxies: "kinemetry"}{subsubsection.4.5.1.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.22}{\ignorespaces Interpreting the residuals of a velocity field}}{257}{figure.caption.146}}
\newlabel{C4_3Dvfrc}{{4.22}{257}{Interpreting the residuals of a velocity field}{figure.caption.146}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.5.2}Kinematics of distant galaxies and beam smearing}{258}{subsection.4.5.2}}
\newlabel{C4_kine_highz}{{4.5.2}{258}{Kinematics of distant galaxies and beam smearing}{subsection.4.5.2}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.5.2.1}Conditions to establish a rotation curve}{258}{subsubsection.4.5.2.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.23}{\ignorespaces VLT/KMOS observation of distant galaxy and sampling}}{259}{figure.caption.147}}
\newlabel{C4_beamsmearing}{{4.23}{259}{VLT/KMOS observation of distant galaxy and sampling}{figure.caption.147}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.5.2.2}Impact of beam smearing on the rotation curve of distant galaxies}{259}{subsubsection.4.5.2.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.24}{\ignorespaces Beam smearing effects on velocity estimates}}{260}{figure.caption.148}}
\newlabel{C4_beamsmearing_effect}{{4.24}{260}{Beam smearing effects on velocity estimates}{figure.caption.148}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.7}\hspace  {2.5em}How to estimate $V_{max}$ and $V_{flat}$ for distant galaxies?}{260}{example.4.7}}
%\zref@newlabel{mdf@pagelabel-79}{\default{4.7}\page{260}\abspage{281}\mdf@pagevalue{260}}
%\pgfsyspdfmark {pgfid79}{8922493}{11691842}
%\zref@newlabel{mdf@pagelabel-80}{\default{4.7}\page{261}\abspage{282}\mdf@pagevalue{261}}
%\pgfsyspdfmark {pgfid80}{8922493}{19762447}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.5.2.3}Impact of beam smearing on the $\sigma $ maps of distant galaxies}{261}{subsubsection.4.5.2.3}}
\newlabel{C4_beamsig}{{4.5.2.3}{261}{Impact of beam smearing on the $\sigma $ maps of distant galaxies}{subsubsection.4.5.2.3}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.8}\hspace  {2.5em}Size of galaxies versus sampling}{262}{example.4.8}}
%\zref@newlabel{mdf@pagelabel-81}{\default{4.8}\page{262}\abspage{283}\mdf@pagevalue{262}}
%\pgfsyspdfmark {pgfid81}{8922493}{32699454}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}4.9}\hspace  {2.5em}Precision on the $\sigma $ peak location}{262}{example.4.9}}
%\zref@newlabel{mdf@pagelabel-82}{\default{4.9}\page{262}\abspage{283}\mdf@pagevalue{262}}
%\pgfsyspdfmark {pgfid82}{8922493}{14944695}
\@writefile{lof}{\contentsline {figure}{\numberline {4.25}{\ignorespaces Beam smearing effects on the dispersion map}}{263}{figure.caption.149}}
\newlabel{C4_3DLarScale}{{4.25}{263}{Beam smearing effects on the dispersion map}{figure.caption.149}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.5.3}Classifications based on pure kinematics}{263}{subsection.4.5.3}}
\newlabel{C4_classification}{{4.5.3}{263}{Classifications based on pure kinematics}{subsection.4.5.3}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.26}{\ignorespaces Precision on the dispersion peak position}}{264}{figure.caption.150}}
\newlabel{C4_3Dsimulpeak}{{4.26}{264}{Precision on the dispersion peak position}{figure.caption.150}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.5.3.1}Classification based on kinemetry}{264}{subsubsection.4.5.3.1}}
\newlabel{C4_kavg}{{4.4}{264}{Classification based on kinemetry}{equation.4.5.4}{}}
\newlabel{C4_vasym}{{4.5}{264}{Classification based on kinemetry}{equation.4.5.5}{}}
\newlabel{C4_sigasym}{{4.6}{264}{Classification based on kinemetry}{equation.4.5.6}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.27}{\ignorespaces V$_{asym}$ versus $\sigma _{asym}$ diagnostic diagram from kinemetry}}{265}{figure.caption.151}}
\newlabel{C4_3Dclasskin3}{{4.27}{265}{V$_{asym}$ versus $\sigma _{asym}$ diagnostic diagram from kinemetry}{figure.caption.151}{}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.5.3.2}Classification based on "$\sigma $ centering"}{266}{subsubsection.4.5.3.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.28}{\ignorespaces Classification of velocity fields of distant galaxies}}{267}{figure.caption.152}}
\newlabel{C4_figexamplegir}{{4.28}{267}{Classification of velocity fields of distant galaxies}{figure.caption.152}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.29}{\ignorespaces Diagnostic diagram of the "sigma centering" method}}{268}{figure.caption.153}}
\newlabel{C4_3Dclasskin}{{4.29}{268}{Diagnostic diagram of the "sigma centering" method}{figure.caption.153}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.5.4}The kinematic classification}{268}{subsection.4.5.4}}
\newlabel{C4_morphokin}{{4.5.4}{268}{The kinematic classification}{subsection.4.5.4}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.30}{\ignorespaces Full kinematics decision tree }}{270}{figure.caption.154}}
\newlabel{C4_decisiontree}{{4.30}{270}{Full kinematics decision tree}{figure.caption.154}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4.31}{\ignorespaces Morpho-kinematics properties of two distant galaxies}}{271}{figure.caption.155}}
\newlabel{C4_IMAGES}{{4.31}{271}{Morpho-kinematics properties of two distant galaxies}{figure.caption.155}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.5.5}The morpho-kinematic classification}{272}{subsection.4.5.5}}
\newlabel{C4_morphokin2}{{4.5.5}{272}{The morpho-kinematic classification}{subsection.4.5.5}{}}
\@writefile{toc}{\contentsline {section}{\numberline {4.6}Conclusion}{272}{section.4.6}}
\gdef\bu@bibdata{C5_ws}
\@writefile{lof}{\addvspace {10\p@ }}
\@writefile{lot}{\addvspace {10\p@ }}
\@writefile{toc}{\contentsline {chapter}{\hbox to\@tempdima {5.\hfil }Applications \& Scaling Relations}{276}{chapter.5}}
\@writefile{toc}{\contentsline {section}{\numberline {5.1}Applications to different distant galaxy studies}{276}{section.5.1}}
\@writefile{toc}{\contentsline {section}{\numberline {5.2}Dissecting the properties of distant galaxies}{277}{section.5.2}}
\newlabel{C5_dissect}{{5.2}{277}{Dissecting the properties of distant galaxies}{section.5.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2.1}An example of a multi-instrument and multi wavelength survey}{277}{subsection.5.2.1}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2.2}Description of a few individual distant galaxies}{278}{subsection.5.2.2}}
\@writefile{toc}{\contentsline {paragraph}{J033237.54-274838.9}{278}{section*.157}}
\@writefile{toc}{\contentsline {paragraph}{ J033238.60-274631.4}{279}{section*.158}}
\@writefile{lof}{\contentsline {figure}{\numberline {5.1}{\ignorespaces Properties of J033237.54-274838.9, a giant, star forming spiral}}{279}{figure.caption.159}}
\newlabel{C5_37p54}{{5.1}{279}{Properties of J033237.54-274838.9, a giant, star forming spiral}{figure.caption.159}{}}
\@writefile{toc}{\contentsline {paragraph}{J033245.11-274724.0}{279}{section*.161}}
\@writefile{lof}{\contentsline {figure}{\numberline {5.2}{\ignorespaces Properties of J033238.60-274631.4, a spiral encountering an elliptical}}{280}{figure.caption.160}}
\newlabel{C5_38p60}{{5.2}{280}{Properties of J033238.60-274631.4, a spiral encountering an elliptical}{figure.caption.160}{}}
\@writefile{toc}{\contentsline {paragraph}{J033244.20-274733.5}{280}{section*.162}}
\@writefile{lof}{\contentsline {figure}{\numberline {5.3}{\ignorespaces Properties of J033245.11-274724.0, a disk rebuilding galaxy}}{281}{figure.caption.163}}
\newlabel{C5_45p11}{{5.3}{281}{Properties of J033245.11-274724.0, a disk rebuilding galaxy}{figure.caption.163}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {5.4}{\ignorespaces Properties of J033244.20-274733.5, a complex merger with $M_{stellar}$= $4.2\times 10^{10}$ $M_{\odot }$ at z=0.73605.}}{282}{figure.caption.164}}
\newlabel{C5_44p20}{{5.4}{282}{Properties of J033244.20-274733.5, a complex merger with $M_{stellar}$= $4.2\times 10^{10}$ $M_{\odot }$ at z=0.73605}{figure.caption.164}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2.3}Spiral disk building and merger rate}{282}{subsection.5.2.3}}
\@writefile{toc}{\contentsline {section}{\numberline {5.3}Evolution of scaling relations}{283}{section.5.3}}
\newlabel{C5_scale}{{5.3}{283}{Evolution of scaling relations}{section.5.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.3.1}Tully-Fisher Relation}{283}{subsection.5.3.1}}
\newlabel{C5_tf}{{5.3.1}{283}{Tully-Fisher Relation}{subsection.5.3.1}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}5.1}\hspace  {2.5em}How to construct a stellar-mass Tully-Fisher relation at high $z$?}{284}{example.5.1}}
%\zref@newlabel{mdf@pagelabel-83}{\default{5.1}\page{284}\abspage{305}\mdf@pagevalue{284}}
\newlabel{C5_doTFR}{{5.1}{284}{Tully-Fisher Relation}{example.5.1}{}}
%\pgfsyspdfmark {pgfid83}{8922493}{11719724}
%\zref@newlabel{mdf@pagelabel-84}{\default{5.1}\page{285}\abspage{306}\mdf@pagevalue{285}}
%\pgfsyspdfmark {pgfid84}{8922493}{23985878}
\@writefile{lof}{\contentsline {figure}{\numberline {5.5}{\ignorespaces Evolution of the stellar-mass TFR at z$\sim $0.6}}{286}{figure.caption.165}}
\newlabel{C5_tfr}{{5.5}{286}{Evolution of the stellar-mass TFR at z$\sim $0.6}{figure.caption.165}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.3.2}The evolution of the M-Z relation}{288}{subsection.5.3.2}}
\newlabel{C5_MZ}{{5.3.2}{288}{The evolution of the M-Z relation}{subsection.5.3.2}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}5.2}\hspace  {2.5em}How to construct a stellar-mass metallicity relation at high z?}{289}{example.5.2}}
%\zref@newlabel{mdf@pagelabel-85}{\default{5.2}\page{289}\abspage{310}\mdf@pagevalue{289}}
%\pgfsyspdfmark {pgfid85}{8922493}{13554732}
%\zref@newlabel{mdf@pagelabel-86}{\default{5.2}\page{290}\abspage{311}\mdf@pagevalue{290}}
%\pgfsyspdfmark {pgfid86}{8922493}{15502607}
\newlabel{C5_SFRM}{{5.3.3}{291}{SFR-$M_{stellar}$ diagram}{subsection.5.3.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.3.3}SFR-$M_{stellar}$ diagram}{291}{subsection.5.3.3}}
\@writefile{lof}{\contentsline {figure}{\numberline {5.6}{\ignorespaces Evolution of the M-Z relation}}{292}{figure.caption.166}}
\newlabel{C5_Fig_MZ_evolution}{{5.6}{292}{Evolution of the M-Z relation}{figure.caption.166}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {5.7}{\ignorespaces SFR-$M_{stellar}$ relation}}{292}{figure.caption.167}}
\newlabel{C5_FigSFRM}{{5.7}{292}{SFR-$M_{stellar}$ relation}{figure.caption.167}{}}
\@writefile{loe}{\contentsline {example}{\numberline {\hspace  {1.5em}5.3}\hspace  {2.5em}How to establish the SFR-$M_{stellar}$ diagram at z$\sim $ 0.9?}{293}{example.5.3}}
%\zref@newlabel{mdf@pagelabel-87}{\default{5.3}\page{293}\abspage{314}\mdf@pagevalue{293}}
%\pgfsyspdfmark {pgfid87}{8922493}{11457580}
%\zref@newlabel{mdf@pagelabel-88}{\default{5.3}\page{294}\abspage{315}\mdf@pagevalue{294}}
%\pgfsyspdfmark {pgfid88}{8922493}{34209494}
\@writefile{toc}{\contentsline {section}{\numberline {5.4}An important challenge: baryonic mass estimate}{295}{section.5.4}}
\newlabel{C5_Mass_estimates}{{5.4}{295}{An important challenge: baryonic mass estimate}{section.5.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.4.1}Stellar mass estimates}{295}{subsection.5.4.1}}
\@writefile{lof}{\contentsline {figure}{\numberline {5.8}{\ignorespaces Constraints from IMF}}{296}{figure.caption.168}}
\newlabel{C5_IMF}{{5.8}{296}{Constraints from IMF}{figure.caption.168}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.4.2}Gas mass estimates}{297}{subsection.5.4.2}}
\@writefile{lof}{\contentsline {figure}{\numberline {5.9}{\ignorespaces Inventory of baryons in galaxies}}{298}{figure.caption.169}}
\newlabel{C5_baryon_inventory}{{5.9}{298}{Inventory of baryons in galaxies}{figure.caption.169}{}}
\@writefile{lof}{\addvspace {10\p@ }}
\@writefile{lot}{\addvspace {10\p@ }}
\@writefile{toc}{\contentsline {chapter}{Appendix\nobreakspace  {}A\unskip \hspace  *{1em}Most intense emission and absorption lines}{302}{appendix.1}}
\@writefile{lot}{\contentsline {table}{\numberline {A.1}{\ignorespaces Most intense emission lines found in AGNs, H$\tmspace  +\thickmuskip {.2777em}$\textsc  {\rmfamily  ii}\relax  regions, and planetary nebulae.\relax }}{303}{table.caption.171}}
\newlabel{App_tabEL}{{A.1}{303}{Most intense emission lines found in AGNs, \ion {H}{2} regions, and planetary nebulae.\relax }{table.caption.171}{}}
\@writefile{lot}{\contentsline {table}{\numberline {A.2}{\ignorespaces Most intense absorption lines found in QSOs and galaxies.\relax }}{304}{table.caption.172}}
\newlabel{App_tabAL}{{A.2}{304}{Most intense absorption lines found in QSOs and galaxies.\relax }{table.caption.172}{}}
\bibstyle{ws-book-har_custMP}
\citation{sterken92} \citation{oke74} \citation{1995PASP..107..945F}
\citation{bessel05} \citation{2007AJ....133..734B}
\citation{kron80,petrosian76,blanton01} \citation{bertin96,graham05,graham05b}
\citation{sterken92} \citation{binney87} \citation{gilli03,vanzella05,ravikumar07}
\citation{lilly95} \citation{lilly95} \citation{lilly96}
\citation{20015AARodrigues} \citation{20015AARodrigues} \citation{flores99}
\citation{flores99b} \citation{flores99b} \citation{hogg02} \citation{hogg02}
\citation{hammer01} \citation{lilly95} \citation{lilly95} \citation{lefevre95}
\citation{rodrigues12} \citation{hammer95} \citation{liang04} \citation{garilli10}
\citation{drinkwater10} \citation{crampton95} \citation{hammer01}
\citation{lefevre95} \citation{johnston11} \citation{peebles1993}
\citation{felten76} \citation{johnston11} \citation{lilly96}
\citation{ravikumar07} \citation{wirth04} \citation{lefevre05}
\citation{crampton95} \citation{ravikumar07} \citation{wirth04}
\citation{lefevre05} \citation{crampton95} \citation{johnston07}
\citation{cowie96} \citation{lilly95} \citation{lefevre95} \citation{hammer95}
\citation{crampton95} \citation{coil04} \citation{willmer06} \citation{faber07}
\citation{lefevre05} \citation{ilbert05} \citation{lilly07} \citation{lilly09}
\citation{pozzetti10} \citation{drinkwater10} \citation{blake10}
\citation{2015arXiv150202659M} \citation{dahlen10} \citation{hildebrandt10}
\citation{margoniner08} \citation{dahlen10} \citation{abrahamse11}
\citation{kotulla11} \citation{macdonald10} \citation{hildebrandt10}
\citation{steidel96} \citation{steidel03,steidel04} \citation{steidel03,steidel04}
\citation{steidel03,steidel04} \citation{papovich04} \citation{giavalisco04}
\citation{dickinson04} \citation{hayes12} \citation{steidel03}
\citation{marchesini10} \citation{vandokkum03} \citation{daddi04}
\citation{reddy05,grazian07} \citation{forsterschreiber09,onodera10}
\citation{ouchi08} \citation{shapley03} \citation{verhamme08}
\citation{dijkstra10} \citation{prochaska03} \citation{tanvir09} \citation{han10}
\citation{lefloch05} \citation{caputi07} \citation{cimatti08}
\citation{prochaska09} \citation{prochaska09} \citation{delgadoserrano10}
\citation{delgadoserrano10} \citation{hammer05} \citation{prochaska09}
\citation{delgadoserrano10} \citation{neichel08}
\bibdata{C1_sample}
\bibcite{abrahamse11}{{1}{2011}{{{Abrahamse} \emph  {et~al.},}}{{{Abrahamse}, {Knox}, {Schmidt}, {Thorman}, {Tyson} and {Zhan}}}}
\bibcite{bertin96}{{2}{1996}{{{Bertin} and {Arnouts}}}{{}}}
\bibcite{bessel05}{{3}{2005}{{Bessell}}{{}}}
\bibcite{binney87}{{4}{1987}{{{Binney} and {Tremaine}}}{{}}}
\bibcite{blake10}{{5}{2010}{{{Blake} \emph  {et~al.},}}{{{Blake}, {Brough}, {Colless}, {Couch}, {Croom}, {Davis}, {Drinkwater}, {Forster}, {Glazebrook}, {Jelliffe} and {Jurek}}}}
\bibcite{blanton01}{{6}{2001}{{{Blanton} \emph  {et~al.},}}{{{Blanton}, {Dalcanton}, {Eisenstein}, {Loveday}, {Strauss}, {SubbaRao}, {Weinberg}, {Anderson}, {Annis}, {Bahcall}, {Bernardi}, {Brinkmann}, {Brunner}, {Burles}, {Carey} and {Castander}}}}
\bibcite{2007AJ....133..734B}{{7}{2007}{{{Blanton} and {Roweis}}}{{}}}
\bibcite{caputi07}{{8}{2007}{{{Caputi} \emph  {et~al.},}}{{{Caputi}, {Lagache}, {Yan}, {Dole}, {Bavouzet}, {Le Floc'h}, {Choi}, {Helou} and {Reddy}}}}
\bibcite{cimatti08}{{9}{2008}{{{Cimatti} \emph  {et~al.},}}{{{Cimatti}, {Cassata}, {Pozzetti}, {Kurk}, {Mignoli}, {Renzini}, {Daddi}, {Bolzonella}, {Brusa}, {Rodighiero}, {Dickinson}, {Franceschini}, {Zamorani}, {Berta}, {Rosati} and {Halliday}}}}
\bibcite{coil04}{{10}{2004}{{{Coil} \emph  {et~al.},}}{{{Coil}, {Davis}, {Madgwick}, {Newman}, {Conselice}, {Cooper}, {Ellis}, {Faber} and {Finkbeiner}}}}
\bibcite{cowie96}{{11}{1996}{{{Cowie} \emph  {et~al.},}}{{{Cowie}, {Songaila}, {Hu} and {Cohen}}}}
\bibcite{crampton95}{{12}{1995}{{{Crampton} \emph  {et~al.},}}{{{Crampton}, {Le Fevre}, {Lilly} and {Hammer}}}}
\bibcite{daddi04}{{13}{2004}{{{Daddi} \emph  {et~al.},}}{{{Daddi}, {Cimatti}, {Renzini}, {Fontana}, {Mignoli}, {Pozzetti}, {Tozzi} and {Zamorani}}}}
\bibcite{dahlen10}{{14}{2010}{{{Dahlen} \emph  {et~al.},}}{{{Dahlen}, {Mobasher}, {Dickinson}, {Ferguson}, {Giavalisco}, {Grogin}, {Guo}, {Koekemoer}, {Lee}, {Lee}, {Nonino}, {Riess} and {Salimbeni}}}}
\bibcite{delgadoserrano10}{{15}{2010}{{{Delgado-Serrano} \emph  {et~al.},}}{{{Delgado-Serrano}, {Hammer}, {Yang}, {Puech}, {Flores} and {Rodrigues}}}}
\bibcite{dickinson04}{{16}{2004}{{{Dickinson} \emph  {et~al.},}}{{{Dickinson}, {Stern}, {Giavalisco}, {Ferguson}, {Tsvetanov}, {Chornock}, {Cristiani}, {Dawson}, {Dey}, {Filippenko}, {Moustakas}, {Nonino}, {Papovich}, {Ravindranath}, {Riess}, {Rosati}, {Spinrad} and {Vanzella}}}}
\bibcite{dijkstra10}{{17}{2010}{{{Dijkstra} and {Wyithe}}}{{}}}
\bibcite{drinkwater10}{{18}{2010}{{{Drinkwater} \emph  {et~al.},}}{{{Drinkwater}, {Jurek}, {Blake}, {Woods}, {Pimbblet}, {Glazebrook}, {Sharp}, {Pracy} and {Brough}}}}
\bibcite{faber07}{{19}{2007}{{{Faber} \emph  {et~al.},}}{{{Faber}, {Willmer}, {Wolf}, {Koo}, {Weiner}, {Newman}, {Im}, {Coil}, {Conroy}, {Cooper}, {Davis}, {Finkbeiner}, {Gerke}, {Gebhardt} and {Groth}}}}
\bibcite{felten76}{{20}{1976}{{Felten}}{{}}}
\bibcite{flores99b}{{21}{1999}{{Flores}}{{}}}
\bibcite{flores99}{{22}{1999}{{{Flores} \emph  {et~al.},}}{{{Flores}, {Hammer}, {Thuan}, {C{\'e}sarsky}, {Desert}, {Omont}, {Lilly}, {Eales}, {Crampton} and {Le F{\`e}vre}}}}
\bibcite{forsterschreiber09}{{23}{2009}{{{F{\"o}rster Schreiber} \emph  {et~al.},}}{{{F{\"o}rster Schreiber}, {Genzel}, {Bouch{\'e}}, {Cresci}, {Davies}, {Buschkamp}, {Shapiro}, {Tacconi}, {Hicks}, {Genel} and {Shapley}}}}
\bibcite{1995PASP..107..945F}{{24}{1995}{{{Fukugita} \emph  {et~al.},}}{{{Fukugita}, {Shimasaku} and {Ichikawa}}}}
\bibcite{garilli10}{{25}{2010}{{{Garilli} \emph  {et~al.},}}{{{Garilli}, {Fumana}, {Franzetti}, {Paioro}, {Scodeggio}, {Le F{\`e}vre}, {Paltani} and {Scaramella}}}}
\bibcite{giavalisco04}{{26}{2004}{{{Giavalisco} \emph  {et~al.},}}{{{Giavalisco}, {Dickinson}, {Ferguson}, {Ravindranath}, {Kretchmer}, {Moustakas}, {Madau}, {Fall}, {Gardner}, {Livio}, {Papovich}, {Renzini}, {Spinrad}, {Stern} and {Riess}}}}
\bibcite{gilli03}{{27}{2003}{{{Gilli} \emph  {et~al.},}}{{{Gilli}, {Cimatti}, {Daddi}, {Hasinger}, {Rosati}, {Szokoly}, {Tozzi}, {Bergeron}, {Borgani}, {Giacconi}, {Kewley}, {Mainieri}, {Mignoli}, {Nonino}, {Norman}, {Wang}, {Zamorani}, {Zheng} and {Zirm}}}}
\bibcite{graham05b}{{28}{2005}{{{Graham} and {Driver}}}{{}}}
\bibcite{graham05}{{29}{2005}{{{Graham} \emph  {et~al.},}}{{{Graham}, {Driver}, {Petrosian}, {Conselice}, {Bershady}, {Crawford} and {Goto}}}}
\bibcite{grazian07}{{30}{2007}{{{Grazian} \emph  {et~al.},}}{{{Grazian}, {Salimbeni}, {Pentericci}, {Fontana}, {Nonino}, {Vanzella}, {Cristiani}, {de Santis}, {Gallozzi}, {Giallongo} and {Santini}}}}
\bibcite{hammer95}{{31}{1995}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Crampton}, {Le Fevre} and {Lilly}}}}
\bibcite{hammer05}{{32}{2005}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Elbaz}, {Zheng}, {Liang} and {Cesarsky}}}}
\bibcite{hammer01}{{33}{2001}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Gruel}, {Thuan}, {Flores} and {Infante}}}}
\bibcite{han10}{{34}{2010}{{{Han} \emph  {et~al.},}}{{{Han}, {Hammer}, {Liang}, {Flores}, {Rodrigues}, {Hou} and {Wei}}}}
\bibcite{hayes12}{{35}{2012}{{{Hayes} \emph  {et~al.},}}{{{Hayes}, {Laporte}, {Pell{\'o}}, {Schaerer} and {Le Borgne}}}}
\bibcite{hildebrandt10}{{36}{2010}{{{Hildebrandt} \emph  {et~al.},}}{{{Hildebrandt}, {Arnouts}, {Capak}, {Moustakas}, {Wolf}, {Abdalla}, {Assef}, {Banerji}, {Ben{\'{\i }}tez}, {Brammer} and {Budav{\'a}ri}}}}
\bibcite{hogg02}{{37}{2002}{{{Hogg} \emph  {et~al.},}}{{{Hogg}, {Baldry}, {Blanton} and {Eisenstein}}}}
\bibcite{ilbert05}{{38}{2005}{{{Ilbert} \emph  {et~al.},}}{{{Ilbert}, {Tresse}, {Zucca}, {Bardelli}, {Arnouts}, {Zamorani}, {Pozzetti}, {Bottini}, {Garilli}, {Le Brun}, {Le F{\`e}vre} and {Maccagni}}}}
\bibcite{johnston11}{{39}{2011}{{Johnston}}{{}}}
\bibcite{johnston07}{{40}{2007}{{{Johnston} \emph  {et~al.},}}{{{Johnston}, {Teodoro} and {Hendry}}}}
\bibcite{kotulla11}{{41}{2011}{{Kotulla}}{{}}}
\bibcite{kron80}{{42}{1980}{{Kron}}{{}}}
\bibcite{lefevre95}{{43}{1995}{{{Le Fevre} \emph  {et~al.},}}{{{Le Fevre}, {Crampton}, {Lilly}, {Hammer} and {Tresse}}}}
\bibcite{lefevre05}{{44}{2005}{{{Le F{\`e}vre} \emph  {et~al.},}}{{{Le F{\`e}vre}, {Vettolani}, {Garilli}, {Tresse}, {Bottini}, {Le Brun}, {Maccagni}, {Picat} and {Scaramella}}}}
\bibcite{lefloch05}{{45}{2005}{{{Le Floc'h} \emph  {et~al.},}}{{{Le Floc'h}, {Papovich}, {Dole}, {Bell}, {Lagache}, {Rieke}, {Egami}, {P{\'e}rez-Gonz{\'a}lez}, {Alonso-Herrero}, {Rieke}, {Blaylock}, {Engelbracht}, {Gordon}, {Hines}, {Misselt}, {Morrison} and {Mould}}}}
\bibcite{liang04}{{46}{2004}{{{Liang} \emph  {et~al.},}}{{{Liang}, {Hammer}, {Flores}, {Gruel} and {Ass{\'e}mat}}}}
\bibcite{lilly09}{{47}{2009}{{{Lilly} \emph  {et~al.},}}{{{Lilly}, {Le Brun}, {Maier}, {Mainieri}, {Mignoli}, {Scodeggio}, {Zamorani}, {Carollo}, {Contini}, {Kneib}, {Le F{\`e}vre} and {Renzini}}}}
\bibcite{lilly95}{{48}{1995}{{{Lilly} \emph  {et~al.},}}{{{Lilly}, {Le Fevre}, {Crampton}, {Hammer} and {Tresse}}}}
\bibcite{lilly96}{{49}{1996}{{{Lilly} \emph  {et~al.},}}{{{Lilly}, {Le Fevre}, {Hammer} and {Crampton}}}}
\bibcite{lilly07}{{50}{2007}{{{Lilly} \emph  {et~al.},}}{{{Lilly}, {Le F{\`e}vre}, {Renzini}, {Zamorani}, {Scodeggio}, {Contini}, {Carollo}, {Hasinger}, {Kneib}, {Iovino}, {Le Brun}, {Maier}, {Mainieri} and {Mignoli}}}}
\bibcite{macdonald10}{{51}{2010}{{{MacDonald} and {Bernstein}}}{{}}}
\bibcite{marchesini10}{{52}{2010}{{{Marchesini} \emph  {et~al.},}}{{{Marchesini}, {Whitaker}, {Brammer}, {van Dokkum}, {Labb{\'e}}, {Muzzin}, {Quadri}, {Kriek}, {Lee}, {Rudnick}, {Franx}, {Illingworth} and {Wake}}}}
\bibcite{margoniner08}{{53}{2008}{{{Margoniner} and {Wittman}}}{{}}}
\bibcite{2015arXiv150202659M}{{54}{2015}{{{Morris} \emph  {et~al.},}}{{{Morris}, {Kocevski}, {Trump}, {Weiner}, {Hathi}, {Barro}, {Dahlen}, {Faber}, {Finkelstein}, {Fontana}, {Ferguson}, {Grogin}, {Gr{\"u}tzbauch}, {Guo}, {Hsu}, {Koekemoer}, {Koo}, {Mobasher}, {Pforr}, {Salvato}, {Wiklind} and {Wuyts}}}}
\bibcite{neichel08}{{55}{2008}{{{Neichel} \emph  {et~al.},}}{{{Neichel}, {Hammer}, {Puech}, {Flores}, {Lehnert}, {Rawat}, {Yang}, {Delgado}, {Amram}, {Balkowski} and {Dannerbauer}}}}
\bibcite{oke74}{{56}{1974}{{Oke}}{{}}}
\bibcite{onodera10}{{57}{2010}{{{Onodera} \emph  {et~al.},}}{{{Onodera}, {Arimoto}, {Daddi}, {Renzini}, {Kong}, {Cimatti}, {Broadhurst} and {Alexander}}}}
\bibcite{ouchi08}{{58}{2008}{{{Ouchi} \emph  {et~al.},}}{{{Ouchi}, {Shimasaku}, {Akiyama}, {Simpson}, {Saito}, {Ueda}, {Furusawa}, {Sekiguchi}, {Yamada}, {Kodama}, {Kashikawa}, {Okamura}, {Iye}, {Takata}, {Yoshida} and {Yoshida}}}}
\bibcite{papovich04}{{59}{2004}{{{Papovich} \emph  {et~al.},}}{{{Papovich}, {Dickinson}, {Ferguson}, {Giavalisco}, {Lotz}, {Madau}, {Idzi}, {Kretchmer}, {Moustakas}, {de Mello}, {Gardner}, {Rieke}, {Somerville} and {Stern}}}}
\bibcite{peebles1993}{{60}{1993}{{Peebles}}{{}}}
\bibcite{petrosian76}{{61}{1976}{{Petrosian}}{{}}}
\bibcite{pozzetti10}{{62}{2010}{{{Pozzetti} \emph  {et~al.},}}{{{Pozzetti}, {Bolzonella}, {Zucca}, {Zamorani}, {Lilly}, {Renzini}, {Moresco}, {Mignoli}, {Cassata}, {Tasca}, {Lamareille}, {Maier} and {Meneux}}}}
\bibcite{prochaska03}{{63}{2003}{{{Prochaska} \emph  {et~al.},}}{{{Prochaska}, {Gawiser}, {Wolfe}, {Castro} and {Djorgovski}}}}
\bibcite{prochaska09}{{64}{2009}{{{Prochaska} and {Wolfe}}}{{}}}
\bibcite{ravikumar07}{{65}{2007}{{{Ravikumar} \emph  {et~al.},}}{{{Ravikumar}, {Puech}, {Flores}, {Proust}, {Hammer}, {Lehnert}, {Rawat}, {Amram}, {Balkowski} and {Burgarella}}}}
\bibcite{reddy05}{{66}{2005}{{{Reddy} \emph  {et~al.},}}{{{Reddy}, {Erb}, {Steidel}, {Shapley}, {Adelberger} and {Pettini}}}}
\bibcite{20015AARodrigues}{{67}{2015}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Foster}, {Taylor}, {Wright}, {Hopkins}, {Baldry}, {Brough}, {Bland-Hawthorn}, {Cluver}, {Lara-Lopez}, {Liske}, {Lopez-Sanchez} and {Pimbblet}}}}
\bibcite{rodrigues12}{{68}{2012}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Puech}, {Hammer}, {Rothberg} and {Flores}}}}
\bibcite{shapley03}{{69}{2003}{{{Shapley} \emph  {et~al.},}}{{{Shapley}, {Steidel}, {Pettini} and {Adelberger}}}}
\bibcite{steidel03}{{70}{2003}{{{Steidel} \emph  {et~al.},}}{{{Steidel}, {Adelberger}, {Shapley}, {Pettini}, {Dickinson} and {Giavalisco}}}}
\bibcite{steidel96}{{71}{1996}{{{Steidel} \emph  {et~al.},}}{{{Steidel}, {Giavalisco}, {Pettini}, {Dickinson} and {Adelberger}}}}
\bibcite{steidel04}{{72}{2004}{{{Steidel} \emph  {et~al.},}}{{{Steidel}, {Shapley}, {Pettini}, {Adelberger}, {Erb}, {Reddy} and {Hunt}}}}
\bibcite{sterken92}{{73}{1992}{{{Sterken} and {Manfroid}}}{{}}}
\bibcite{tanvir09}{{74}{2009}{{{Tanvir} \emph  {et~al.},}}{{{Tanvir}, {Fox}, {Levan}, {Berger}, {Wiersema}, {Fynbo}, {Cucchiara}, {Kr{\"u}hler}, {Gehrels}, {Bloom}, {Greiner}, {Evans}, {Rol}, {Olivares}, {Hjorth} and {Jakobsson}}}}
\bibcite{vandokkum03}{{75}{2003}{{{van Dokkum} \emph  {et~al.},}}{{{van Dokkum}, {F{\"o}rster Schreiber}, {Franx}, {Daddi}, {Illingworth}, {Labb{\'e}}, {Moorwood}, {Rix}, {R{\"o}ttgering}, {Rudnick}, {van der Wel}, {van der Werf} and {van Starkenburg}}}}
\bibcite{vanzella05}{{76}{2005}{{{Vanzella} \emph  {et~al.},}}{{{Vanzella}, {Cristiani}, {Dickinson}, {Kuntschner}, {Moustakas}, {Nonino}, {Rosati}, {Stern}, {Cesarsky}, {Ettori}, {Ferguson}, {Fosbury}, {Giavalisco}, {Haase}, {Renzini}, {Rettura}, {Serra} and {GOODS Team}}}}
\bibcite{verhamme08}{{77}{2008}{{{Verhamme} \emph  {et~al.},}}{{{Verhamme}, {Schaerer}, {Atek} and {Tapken}}}}
\bibcite{willmer06}{{78}{2006}{{{Willmer} \emph  {et~al.},}}{{{Willmer}, {Faber}, {Koo}, {Weiner}, {Newman}, {Coil}, {Connolly}, {Conroy}, {Cooper}, {Davis} and {Finkbeiner}}}}
\bibcite{wirth04}{{79}{2004}{{{Wirth} \emph  {et~al.},}}{{{Wirth}, {Willmer}, {Amico}, {Chaffee}, {Goodrich}, {Kwok}, {Lyke}, {Mader} and {Tran}}}}
\bibstyle{ws-book-har_custMP}
\citation{mackay86} \citation{rieke07} \citation{vandenbergh02,delgadoserrano10}
\citation{neichel08} \citation{tokovinin02} \citation{martinez10}
\citation{king71} \citation{moffat69,trujillo01} \citation{neichel08}
\citation{neichel08} \citation{roddier81} \citation{fried66} \citation{holtzman90}
\citation{howell96} \citation{harris90} \citation{puech08} \citation{lauer99}
\citation{fruchter02,fruchter11} \citation{marsh04} \citation{starck02,puetter05}
\citation{disseau15} \citation{barden08} \citation{barden08} \citation{beckwith06}
\citation{koekemoer13} \citation{grazian12} \citation{sullivan12}
\citation{grazian12} \citation{szalay99} \citation{bouwens15}
\citation{cappellari03,diehl06} \citation{starck06} \citation{zackrisson08}
\citation{waller90} \citation{tilvi13} \citation{mostardi13} \citation{tilvi13}
\citation{mostardi13} \citation{bessell05} \citation{fukugita96}
\citation{smith02} \citation{carpenter01} \citation{bessell05} \citation{bilir08}
\citation{charlot96} \citation{charlot96} \citation{kuchinski00}
\citation{bunker00} \citation{bunker00} \citation{delgadoserrano10}
\citation{leinert98,noll12} \citation{vaduvescu04} \citation{davies12}
\citation{gilliland92} \citation{newberry91} \citation{tyson93}
\citation{chromey96} \citation{tyson88,tyson90} \citation{newberry91}
\citation{tyson90} \citation{sterken92} \citation{chromey96} \citation{andersen95}
\citation{grundahl96} \citation{moehler10} \citation{howell12} \citation{tyson88}
\citation{kornilov12} \citation{howell06,merline95} \citation{howell06}
\citation{rieke07} \citation{leinert98} \citation{hubble26} \citation{sandage05}
\citation{jeans19} \citation{reynolds20} \citation{buta11} \citation{comeron12}
\citation{hubble36} \citation{sandage61} \citation{sandage05}
\citation{devaucouleurs59} \citation{vandenbergh60} \citation{vandenbergh02}
\citation{kormendy13}
\citation{devaucouleurs59,morgan58,morgan59,morgan57,vandenbergh60,vandenbergh60b}
\citation{sandage05} \citation{delgadoserrano10} \citation{vandenbergh07}
\citation{delgadoserrano12} \citation{roberts94} \citation{hammer05,zheng05}
\citation{vandenbergh02} \citation{kormendy13}
\citation{vandenbergh02,elmegreen05,elmegreen07} \citation{zheng05,sheth08}
\citation{rawat09} \citation{cameron11} \citation{hubble26,heidmann72,unterborn08}
\citation{brinchmann98,vandenbergh02} \citation{naim95} \citation{zheng05}
\citation{kartaltepe15} \citation{nair10} \citation{sersic68} \citation{peng10}
\citation{freeman70} \citation{graham05} \citation{peng10} \citation{haussler07}
\citation{barden12} \citation{vikram10} \citation{kelvin12} \citation{ryan11}
\citation{simard98,simard02} \citation{peng02,peng10} \citation{wadadekar99}
\citation{desouza04} \citation{pignatelli06} \citation{yoon11}
\citation{casertano00} \citation{kormendy04} \citation{disseau15}
\citation{disseau15} \citation{hammer09} \citation{schade95,abraham96,conselice00}
\citation{conselice03} \citation{abraham03,lotz04} \citation{lotz11}
\citation{conselice00,lotz04,lauger05,lisker08,chen10}
\citation{burgarella01,conselice03,lauger05,taylormager07}
\citation{conselice03,conselice08} \citation{neichel08} \citation{franceschini06}
\citation{neichel08} \citation{neichel08} \citation{neichel08}
\citation{neichel08} \citation{scarlata07} \citation{huertascompany08}
\citation{roberts94} \citation{oh13} \citation{schade99}
\citation{strateva01,baldry04,bell04} \citation{cassata08} \citation{kannappan09}
\citation{delgadoserrano10} \citation{delgadoserrano10}
\citation{delgadoserrano10} \citation{delgadoserrano10}
\citation{neichel08,hammer09} \citation{delgadoserrano10}
\citation{zheng04,zheng05,neichel08} \citation{delgadoserrano10}
\citation{delapparent11} \citation{vandenbergh02} \citation{neichel08}
\citation{hammer09} \citation{abraham99,menanteau01,zheng04} \citation{zheng04}
\citation{zheng04} \citation{abraham99,menanteau01,zibetti11} \citation{zheng04}
\citation{delgadoserrano10} \citation{neichel08} \citation{neichel08}
\citation{neichel08} \citation{neichel08} \citation{zheng04} \citation{zheng04}
\citation{yan13} \citation{yan13} \citation{flores99} \citation{flores99}
\citation{flores99} \citation{howell89} \citation{phillipps84}
\citation{morrissey07} \citation{jarvis81} \citation{bertin96} \citation{elbaz11}
\citation{elbaz11} \citation{laidler07} \citation{laidler07} \citation{laidler07}
\citation{laidler07} \citation{stetson87} \citation{schechter93}
\citation{annunziatella13} \citation{laidler07} \citation{mancone13}
\citation{annibali08} \citation{annibali08} \citation{neichel08}
\citation{leger89} \citation{polletta07} \citation{silva98} \citation{polletta07}
\citation{polletta07} \citation{silva98} \citation{polletta07}
\citation{tinsley67,tinsley72} \citation{schaerer13} \citation{rodrigues14}
\citation{worthey94} \citation{gordon97} \citation{charlot96}
\citation{schlegel98} \citation{peek10} \citation{schlegel98} \citation{nonino09}
\citation{takeuchi12}
\citation{cardelli89,odonnell94,calzetti00,fitzpatrick99,fitzpatrick07}
\citation{charlot00} \citation{tully98,masters03,wild11} \citation{unterborn08}
\citation{masters03} \citation{tully98} \citation{giavalisco02} \citation{madau95}
\citation{meiksin06,inoue08} \citation{harrison11} \citation{gunn65}
\citation{becker01} \citation{bouwens10} \citation{bouwens10}
\citation{osterbrock06} \citation{leitherer99} \citation{schaerer09}
\citation{krueger95} \citation{raiter10} \citation{schaerer09,debarros14}
\citation{zackrisson08} \citation{leitherer99,fioc99,schaerer09}
\citation{reines10} \citation{reines10} \citation{conroy13}
\citation{maraston10,pforr12} \citation{conroy13} \citation{walcher11}
\citation{conroy09,conroy10a,conroy10b,kriek10,pirzkal12,pforr12,conroy13}
\citation{papovich01} \citation{puech09} \citation{puech09} \citation{puech09}
\citation{puech09} \citation{taylor11} \citation{milone11} \citation{pforr12}
\citation{pforr12} \citation{pforr12} \citation{avni76} \citation{walcher11}
\citation{taylor11} \citation{kauffmann03,walcher11} \citation{pirzkal13}
\citation{bruzual03} \citation{walcher11} \citation{maraston10,pirzkal12}
\citation{maraston05,kriek10,melbourne12,zibetti13} \citation{conroy09}
\citation{pforr12} \citation{papovich01} \citation{papovich01} \citation{puech09}
\citation{puech09} \citation{papovich01} \citation{puech09} \citation{puech09}
\citation{bell01} \citation{bell03} \citation{zibetti09} \citation{gallazzi09}
\citation{bell01} \citation{kauffmann98,bell01} \citation{mcgaugh14}
\citation{bell03} \citation{mcgaugh14} \citation{bell03} \citation{bell03}
\citation{puech08} \citation{bell03} \citation{bell03} \citation{bell03}
\citation{stark09} \citation{kannappan07} \citation{kennicutt12}
\citation{kennicutt98,lefloch05,rieke08} \citation{condon92}
\citation{smolcic08,ivison10} \citation{kennicutt98} \citation{kennicutt12}
\citation{flores99,lefloch05} \citation{kennicutt12} \citation{bell05}
\citation{kennicutt12} \citation{kennicutt98,kennicutt12} \citation{chary01}
\citation{kennicutt98} \citation{chary01,dale02,lagache03,rieke08}
\citation{kennicutt98} \citation{bell05} \citation{bell05}
\citation{shapley11,elbaz11} \citation{nordon10,elbaz10} \citation{galametz13}
\citation{nguyen10,berta10,elbaz10,elbaz11} \citation{flores04,dominguezsanchez12}
\citation{dominguezsanchez12} \citation{flores04} \citation{dominguezsanchez12}
\citation{flores04}
\bibdata{C2_imaging}
\bibcite{abraham99}{{80}{1999}{{{Abraham} \emph  {et~al.},}}{{{Abraham}, {Ellis}, {Fabian}, {Tanvir} and {Glazebrook}}}}
\bibcite{abraham96}{{81}{1996}{{{Abraham} \emph  {et~al.},}}{{{Abraham}, {Tanvir}, {Santiago}, {Ellis}, {Glazebrook} and {van den Bergh}}}}
\bibcite{abraham03}{{82}{2003}{{{Abraham} \emph  {et~al.},}}{{{Abraham}, {van den Bergh} and {Nair}}}}
\bibcite{andersen95}{{83}{1995}{{{Andersen} \emph  {et~al.},}}{{{Andersen}, {Freyhammer} and {Storm}}}}
\bibcite{annibali08}{{84}{2008}{{{Annibali} \emph  {et~al.},}}{{{Annibali}, {Aloisi}, {Mack}, {Tosi}, {van der Marel}, {Angeretti}, {Leitherer} and {Sirianni}}}}
\bibcite{annunziatella13}{{85}{2013}{{{Annunziatella} \emph  {et~al.},}}{{{Annunziatella}, {Mercurio}, {Brescia}, {Cavuoti} and {Longo}}}}
\bibcite{avni76}{{86}{1976}{{Avni}}{{}}}
\bibcite{baldry04}{{87}{2004}{{{Baldry} \emph  {et~al.},}}{{{Baldry}, {Glazebrook}, {Brinkmann}, {Ivezi{\'c}}, {Lupton}, {Nichol} and {Szalay}}}}
\bibcite{barden12}{{88}{2012}{{{Barden} \emph  {et~al.},}}{{{Barden}, {H{\"a}u{\ss }ler}, {Peng}, {McIntosh} and {Guo}}}}
\bibcite{barden08}{{89}{2008}{{{Barden} \emph  {et~al.},}}{{{Barden}, {Jahnke} and {H{\"a}u{\ss }ler}}}}
\bibcite{becker01}{{90}{2001}{{{Becker} \emph  {et~al.},}}{{{Becker}, {Fan}, {White}, {Strauss}, {Narayanan}, {Lupton}, {Gunn}, {Annis}, {Bahcall}, {Brinkmann}, {Connolly}, {Csabai} and {Czarapata}}}}
\bibcite{beckwith06}{{91}{2006}{{{Beckwith} \emph  {et~al.},}}{{{Beckwith}, {Stiavelli}, {Koekemoer}, {Caldwell}, {Ferguson}, {Hook}, {Lucas}, {Bergeron}, {Corbin}, {Jogee}, {Panagia}, {Robberto}, {Royle}, {Somerville} and {Sosey}}}}
\bibcite{bell01}{{92}{2001}{{{Bell} and {de Jong}}}{{}}}
\bibcite{bell03}{{93}{2003}{{{Bell} \emph  {et~al.},}}{{{Bell}, {McIntosh}, {Katz} and {Weinberg}}}}
\bibcite{bell05}{{94}{2005}{{{Bell} \emph  {et~al.},}}{{{Bell}, {Papovich}, {Wolf}, {Le Floc'h}, {Caldwell}, {Barden}, {Egami}, {McIntosh}, {Meisenheimer}, {P{\'e}rez-Gonz{\'a}lez}, {Rieke}, {Rieke}, {Rigby} and {Rix}}}}
\bibcite{bell04}{{95}{2004}{{{Bell} \emph  {et~al.},}}{{{Bell}, {Wolf}, {Meisenheimer}, {Rix}, {Borch}, {Dye}, {Kleinheinrich}, {Wisotzki} and {McIntosh}}}}
\bibcite{berta10}{{96}{2010}{{{Berta} \emph  {et~al.},}}{{{Berta}, {Magnelli}, {Lutz}, {Altieri}, {Aussel}, {Andreani}, {Bauer}, {Bongiovanni}, {Cava}, {Cepa}, {Cimatti}, {Daddi}, {Dominguez}, {Elbaz}, {Feuchtgruber}, {F{\"o}rster Schreiber}, {Genzel}, {Gruppioni} and {Katterloher}}}}
\bibcite{bertin96}{{97}{1996}{{{Bertin} and {Arnouts}}}{{}}}
\bibcite{bessell05}{{98}{2005}{{Bessell}}{{}}}
\bibcite{bilir08}{{99}{2008}{{{Bilir} \emph  {et~al.},}}{{{Bilir}, {Ak}, {Karaali}, {Cabrera-Lavers}, {Chonis} and {Gaskell}}}}
\bibcite{bouwens10}{{100}{2010}{{{Bouwens} \emph  {et~al.},}}{{{Bouwens}, {Illingworth}, {Oesch}, {Stiavelli}, {van Dokkum}, {Trenti}, {Magee}, {Labb{\'e}}, {Franx}, {Carollo} and {Gonzalez}}}}
\bibcite{bouwens15}{{101}{2015}{{{Bouwens} \emph  {et~al.},}}{{{Bouwens}, {Illingworth}, {Oesch}, {Trenti}, {Labb{\'e}}, {Bradley}, {Carollo}, {van Dokkum}, {Gonzalez}, {Holwerda}, {Franx}, {Spitler}, {Smit} and {Magee}}}}
\bibcite{brinchmann98}{{102}{1998}{{{Brinchmann} \emph  {et~al.},}}{{{Brinchmann}, {Abraham}, {Schade}, {Tresse}, {Ellis}, {Lilly}, {Le Fevre}, {Glazebrook}, {Hammer}, {Colless}, {Crampton} and {Broadhurst}}}}
\bibcite{bruzual03}{{103}{2003}{{{Bruzual} and {Charlot}}}{{}}}
\bibcite{bunker00}{{104}{2000}{{{Bunker} \emph  {et~al.},}}{{{Bunker}, {Spinrad}, {Stern}, {Thompson}, {Moustakas}, {Davis} and {Dey}}}}
\bibcite{burgarella01}{{105}{2001}{{{Burgarella} \emph  {et~al.},}}{{{Burgarella}, {Buat}, {Donas}, {Milliard} and {Chapelon}}}}
\bibcite{buta11}{{106}{2011}{{Buta}}{{}}}
\bibcite{calzetti00}{{107}{2000}{{{Calzetti} \emph  {et~al.},}}{{{Calzetti}, {Armus}, {Bohlin}, {Kinney}, {Koornneef} and {Storchi-Bergmann}}}}
\bibcite{cameron11}{{108}{2011}{{{Cameron} \emph  {et~al.},}}{{{Cameron}, {Carollo}, {Oesch}, {Bouwens}, {Illingworth}, {Trenti}, {Labb{\'e}} and {Magee}}}}
\bibcite{cappellari03}{{109}{2003}{{{Cappellari} and {Copin}}}{{}}}
\bibcite{cardelli89}{{110}{1989}{{{Cardelli} \emph  {et~al.},}}{{{Cardelli}, {Clayton} and {Mathis}}}}
\bibcite{carpenter01}{{111}{2001}{{Carpenter}}{{}}}
\bibcite{casertano00}{{112}{2000}{{{Casertano} \emph  {et~al.},}}{{{Casertano}, {de Mello}, {Dickinson}, {Ferguson}, {Fruchter}, {Gonzalez-Lopezlira}, {Heyer}, {Hook}, {Levay}, {Lucas} and {Mack}}}}
\bibcite{cassata08}{{113}{2008}{{{Cassata} \emph  {et~al.},}}{{{Cassata}, {Cimatti}, {Kurk}, {Rodighiero}, {Pozzetti}, {Bolzonella}, {Daddi}, {Mignoli}, {Berta}, {Dickinson} and {Franceschini}}}}
\bibcite{charlot96}{{114}{1996}{{Charlot}}{{}}}
\bibcite{charlot00}{{115}{2000}{{{Charlot} and {Fall}}}{{}}}
\bibcite{chary01}{{116}{2001}{{{Chary} and {Elbaz}}}{{}}}
\bibcite{chen10}{{117}{2010}{{{Chen} \emph  {et~al.},}}{{{Chen}, {C{\^o}t{\'e}}, {West}, {Peng} and {Ferrarese}}}}
\bibcite{chromey96}{{118}{1996}{{{Chromey} and {Hasselbacher}}}{{}}}
\bibcite{comeron12}{{119}{2012}{{{Comer{\'o}n} \emph  {et~al.},}}{{{Comer{\'o}n}, {Elmegreen}, {Salo}, {Laurikainen}, {Athanassoula}, {Bosma}, {Knapen}, {Gadotti} and {Sheth}}}}
\bibcite{condon92}{{120}{1992}{{Condon}}{{}}}
\bibcite{conroy13}{{121}{2013}{{Conroy}}{{}}}
\bibcite{conroy10a}{{122}{2010}{{{Conroy} and {Gunn}}}{{}}}
\bibcite{conroy09}{{123}{2009}{{{Conroy} \emph  {et~al.},}}{{{Conroy}, {Gunn} and {White}}}}
\bibcite{conroy10b}{{124}{2010}{{{Conroy} \emph  {et~al.},}}{{{Conroy}, {White} and {Gunn}}}}
\bibcite{conselice03}{{125}{2003}{{{Conselice} \emph  {et~al.},}}{{{Conselice}, {Bershady}, {Dickinson} and {Papovich}}}}
\bibcite{conselice00}{{126}{2000}{{{Conselice} \emph  {et~al.},}}{{{Conselice}, {Bershady} and {Jangren}}}}
\bibcite{conselice08}{{127}{2008}{{{Conselice} \emph  {et~al.},}}{{{Conselice}, {Rajgor} and {Myers}}}}
\bibcite{dale02}{{128}{2002}{{{Dale} and {Helou}}}{{}}}
\bibcite{davies12}{{129}{2012}{{{Davies} and {Kasper}}}{{}}}
\bibcite{debarros14}{{130}{2014}{{{de Barros} \emph  {et~al.},}}{{{de Barros}, {Schaerer} and {Stark}}}}
\bibcite{delapparent11}{{131}{2011}{{{de Lapparent} \emph  {et~al.},}}{{{de Lapparent}, {Baillard} and {Bertin}}}}
\bibcite{desouza04}{{132}{2004}{{{de Souza} \emph  {et~al.},}}{{{de Souza}, {Gadotti} and {dos Anjos}}}}
\bibcite{devaucouleurs59}{{133}{1959}{{de Vaucouleurs}}{{}}}
\bibcite{delgadoserrano12}{{134}{2012}{{Delgado-Serrano}}{{}}}
\bibcite{delgadoserrano10}{{135}{2010}{{{Delgado-Serrano} \emph  {et~al.},}}{{{Delgado-Serrano}, {Hammer}, {Yang}, {Puech}, {Flores} and {Rodrigues}}}}
\bibcite{diehl06}{{136}{2006}{{{Diehl} and {Statler}}}{{}}}
\bibcite{disseau15}{{137}{2015}{{{Disseau} \emph  {et~al.},}}{{{Disseau}, {Hammer}, {Puech}, {Flores} and Y.}}}
\bibcite{dominguezsanchez12}{{138}{2012}{{{Dom{\'{\i }}nguez S{\'a}nchez} \emph  {et~al.},}}{{{Dom{\'{\i }}nguez S{\'a}nchez}, {Mignoli}, {Pozzi}, {Calura}, {Cimatti}, {Gruppioni}, {Cepa} and {S{\'a}nchez Portal}}}}
\bibcite{elbaz11}{{139}{2011}{{{Elbaz} \emph  {et~al.},}}{{{Elbaz}, {Dickinson}, {Hwang}, {D{\'{\i }}az-Santos}, {Magdis}, {Magnelli}, {Le Borgne}, {Galliano}, {Pannella}, {Chanial} and {Armus}}}}
\bibcite{elbaz10}{{140}{2010}{{{Elbaz} \emph  {et~al.},}}{{{Elbaz}, {Hwang}, {Magnelli}, {Daddi}, {Aussel}, {Altieri}, {Amblard}, {Andreani}, {Arumugam}, {Auld}, {Babbedge}, {Berta} and {Blain}}}}
\bibcite{elmegreen07}{{141}{2007}{{{Elmegreen} \emph  {et~al.},}}{{{Elmegreen}, {Elmegreen}, {Ravindranath} and {Coe}}}}
\bibcite{elmegreen05}{{142}{2005}{{{Elmegreen} \emph  {et~al.},}}{{{Elmegreen}, {Elmegreen}, {Rubin} and {Schaffer}}}}
\bibcite{fioc99}{{143}{1999}{{{Fioc} and {Rocca-Volmerange}}}{{}}}
\bibcite{fitzpatrick99}{{144}{1999}{{Fitzpatrick}}{{}}}
\bibcite{fitzpatrick07}{{145}{2007}{{{Fitzpatrick} and {Massa}}}{{}}}
\bibcite{flores99}{{146}{1999}{{{Flores} \emph  {et~al.},}}{{{Flores}, {Hammer}, {D{\'e}sert}, {C{\'e}sarsky}, {Thuan}, {Crampton}, {Eales}, {Le F{\`e}vre}, {Lilly}, {Omont} and {Elbaz}}}}
\bibcite{flores04}{{147}{2004}{{{Flores} \emph  {et~al.},}}{{{Flores}, {Hammer}, {Elbaz}, {Cesarsky}, {Liang}, {Fadda} and {Gruel}}}}
\bibcite{franceschini06}{{148}{2006}{{{Franceschini} \emph  {et~al.},}}{{{Franceschini}, {Rodighiero}, {Cassata}, {Berta}, {Vaccari}, {Nonino}, {Vanzella}, {Hatziminaoglou}, {Antichi} and {Cristiani}}}}
\bibcite{freeman70}{{149}{1970}{{Freeman}}{{}}}
\bibcite{fried66}{{150}{1966}{{Fried}}{{}}}
\bibcite{fruchter11}{{151}{2011}{{Fruchter}}{{}}}
\bibcite{fruchter02}{{152}{2002}{{{Fruchter} and {Hook}}}{{}}}
\bibcite{fukugita96}{{153}{1996}{{{Fukugita} \emph  {et~al.},}}{{{Fukugita}, {Ichikawa}, {Gunn}, {Doi}, {Shimasaku} and {Schneider}}}}
\bibcite{galametz13}{{154}{2013}{{{Galametz} \emph  {et~al.},}}{{{Galametz}, {Kennicutt}, {Calzetti}, {Aniano}, {Draine}, {Boquien}, {Brandl}, {Croxall}, {Dale}, {Engelbracht}, {Gordon}, {Groves}, {Hao}, {Helou}, {Hinz}, {Hunt}, {Johnson}, {Li}, {Murphy}, {Roussel}, {Sandstrom}, {Skibba} and {Tabatabaei}}}}
\bibcite{gallazzi09}{{155}{2009}{{{Gallazzi} and {Bell}}}{{}}}
\bibcite{giavalisco02}{{156}{2002}{{Giavalisco}}{{}}}
\bibcite{gilliland92}{{157}{1992}{{Gilliland}}{{}}}
\bibcite{gordon97}{{158}{1997}{{{Gordon} \emph  {et~al.},}}{{{Gordon}, {Calzetti} and {Witt}}}}
\bibcite{graham05}{{159}{2005}{{{Graham} and {Driver}}}{{}}}
\bibcite{grazian12}{{160}{2012}{{{Grazian} \emph  {et~al.},}}{{{Grazian}, {Castellano}, {Fontana}, {Pentericci}, {Dunlop}, {McLure}, {Koekemoer}, {Dickinson}, {Faber}, {Ferguson} and {Galametz}}}}
\bibcite{grundahl96}{{161}{1996}{{{Grundahl} and {Sorensen}}}{{}}}
\bibcite{gunn65}{{162}{1965}{{{Gunn} and {Peterson}}}{{}}}
\bibcite{hammer05}{{163}{2005}{{Hammer}}{{}}}
\bibcite{hammer09}{{164}{2009}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Puech}, {Yang}, {Athanassoula}, {Rodrigues} and {Delgado}}}}
\bibcite{harris90}{{165}{1990}{{Harris}}{{}}}
\bibcite{harrison11}{{166}{2011}{{{Harrison} \emph  {et~al.},}}{{{Harrison}, {Meiksin} and {Stock}}}}
\bibcite{haussler07}{{167}{2007}{{{H{\"a}ussler} \emph  {et~al.},}}{{{H{\"a}ussler}, {McIntosh}, {Barden}, {Bell}, {Rix}, {Borch}, {Beckwith}, {Caldwell}, {Heymans}, {Jahnke}, {Jogee}, {Koposov}, {Meisenheimer}, {S{\'a}nchez}, {Somerville}, {Wisotzki} and {Wolf}}}}
\bibcite{heidmann72}{{168}{1972}{{{Heidmann} \emph  {et~al.},}}{{{Heidmann}, {Heidmann} and {de Vaucouleurs}}}}
\bibcite{holtzman90}{{169}{1990}{{Holtzman}}{{}}}
\bibcite{howell89}{{170}{1989}{{Howell}}{{}}}
\bibcite{howell06}{{171}{2006}{{Howell}}{{}}}
\bibcite{howell12}{{172}{2012}{{Howell}}{{}}}
\bibcite{howell96}{{173}{1996}{{{Howell} \emph  {et~al.},}}{{{Howell}, {Koehn}, {Bowell} and {Hoffman}}}}
\bibcite{hubble26}{{174}{1926}{{Hubble}}{{}}}
\bibcite{hubble36}{{175}{1936}{{Hubble}}{{}}}
\bibcite{huertascompany08}{{176}{2008}{{{Huertas-Company} \emph  {et~al.},}}{{{Huertas-Company}, {Rouan}, {Tasca}, {Soucail} and {Le F{\`e}vre}}}}
\bibcite{inoue08}{{177}{2008}{{{Inoue} and {Kamaya}}}{{}}}
\bibcite{ivison10}{{178}{2010}{{{Ivison} \emph  {et~al.},}}{{{Ivison}, {Magnelli}, {Ibar}, {Andreani}, {Elbaz}, {Altieri}, {Amblard}, {Arumugam}, {Auld}, {Aussel}, {Babbedge}, {Berta}, {Blain}, {Bock}, {Bongiovanni} and {Boselli}}}}
\bibcite{jarvis81}{{179}{1981}{{{Jarvis} and {Tyson}}}{{}}}
\bibcite{jeans19}{{180}{1919}{{Jeans}}{{}}}
\bibcite{kannappan07}{{181}{2007}{{{Kannappan} and {Gawiser}}}{{}}}
\bibcite{kannappan09}{{182}{2009}{{{Kannappan} \emph  {et~al.},}}{{{Kannappan}, {Guie} and {Baker}}}}
\bibcite{kartaltepe15}{{183}{2015}{{{Kartaltepe} \emph  {et~al.},}}{{{Kartaltepe}, {Mozena}, {Kocevski}, {McIntosh}, {Lotz}, {Bell}, {Faber}, {Ferguson}, {Koo}, {Bassett}, {Bernyk}, {Blancato}, {Bournaud}, {Cassata}, {Castellano}, {Cheung}, {Conselice}, {Croton}, {Dahlen}, {de Mello}, {DeGroot}, {Donley}, {Guedes}, {Grogin}, {Hathi}, {Hilton}, {Hollon}, {Koekemoer}, {Liu}, {Lucas}, {Martig}, {McGrath}, {McPartland}, {Mobasher}, {Morlock}, {O'Leary}, {Peth}, {Pforr}, {Pillepich}, {Rosario}, {Soto}, {Straughn}, {Telford}, {Sunnquist}, {Trump}, {Weiner} and {Wuyts}}}}
\bibcite{kauffmann98}{{184}{1998}{{{Kauffmann} and {Charlot}}}{{}}}
\bibcite{kauffmann03}{{185}{2003}{{{Kauffmann} \emph  {et~al.},}}{{{Kauffmann}, {Heckman}, {White}, {Charlot}, {Tremonti}, {Brinchmann}, {Bruzual}, {Peng} and {Seibert}}}}
\bibcite{kelvin12}{{186}{2012}{{{Kelvin} \emph  {et~al.},}}{{{Kelvin}, {Driver}, {Robotham}, {Hill}, {Alpaslan}, {Baldry}, {Bamford} and {Bland-Hawthorn}}}}
\bibcite{kennicutt12}{{187}{2012}{{{Kennicutt} and {Evans}}}{{}}}
\bibcite{kennicutt98}{{188}{1998}{{Kennicutt}}{{}}}
\bibcite{king71}{{189}{1971}{{King}}{{}}}
\bibcite{koekemoer13}{{190}{2013}{{{Koekemoer} \emph  {et~al.},}}{{{Koekemoer}, {Ellis}, {McLure}, {Dunlop}, {Robertson}, {Ono}, {Schenker}, {Ouchi}, {Bowler}, {Rogers} and {Curtis-Lake}}}}
\bibcite{kormendy13}{{191}{2013}{{Kormendy}}{{}}}
\bibcite{kormendy04}{{192}{2004}{{{Kormendy} and {Kennicutt}}}{{}}}
\bibcite{kornilov12}{{193}{2012}{{Kornilov}}{{}}}
\bibcite{kriek10}{{194}{2010}{{{Kriek} \emph  {et~al.},}}{{{Kriek}, {Labb{\'e}}, {Conroy}, {Whitaker}, {van Dokkum}, {Brammer}, {Franx}, {Illingworth}, {Marchesini}, {Muzzin}, {Quadri} and {Rudnick}}}}
\bibcite{krueger95}{{195}{1995}{{{Krueger} \emph  {et~al.},}}{{{Krueger}, {Fritze-v.~Alvensleben} and {Loose}}}}
\bibcite{kuchinski00}{{196}{2000}{{{Kuchinski} \emph  {et~al.},}}{{{Kuchinski}, {Freedman}, {Madore}, {Trewhella}, {Bohlin}, {Cornett}, {Fanelli}, {Marcum}, {Neff}, {O'Connell}, {Roberts}, {Smith}, {Stecher} and {Waller}}}}
\bibcite{lagache03}{{197}{2003}{{{Lagache} \emph  {et~al.},}}{{{Lagache}, {Dole} and {Puget}}}}
\bibcite{laidler07}{{198}{2007}{{{Laidler} \emph  {et~al.},}}{{{Laidler}, {Papovich}, {Grogin}, {Idzi}, {Dickinson}, {Ferguson}, {Hilbert}, {Clubb} and {Ravindranath}}}}
\bibcite{lauer99}{{199}{1999}{{Lauer}}{{}}}
\bibcite{lauger05}{{200}{2005}{{{Lauger} \emph  {et~al.},}}{{{Lauger}, {Burgarella} and {Buat}}}}
\bibcite{lefloch05}{{201}{2005}{{{Le Floc'h} \emph  {et~al.},}}{{{Le Floc'h}, {Papovich}, {Dole}, {Bell}, {Lagache}, {Rieke}, {Egami}, {P{\'e}rez-Gonz{\'a}lez}, {Alonso-Herrero}, {Rieke}, {Blaylock}, {Engelbracht}, {Gordon}, {Hines}, {Misselt}, {Morrison} and {Mould}}}}
\bibcite{leger89}{{202}{1989}{{{Leger} \emph  {et~al.},}}{{{Leger}, {D'Hendecourt} and {Defourneau}}}}
\bibcite{leinert98}{{203}{1998}{{{Leinert} \emph  {et~al.},}}{{{Leinert}, {Bowyer}, {Haikala}, {Hanner}, {Hauser}, {Levasseur-Regourd}, {Mann}, {Mattila}, {Reach}, {Schlosser}, {Staude}, {Toller}, {Weiland}, {Weinberg} and {Witt}}}}
\bibcite{leitherer99}{{204}{1999}{{{Leitherer} \emph  {et~al.},}}{{{Leitherer}, {Schaerer}, {Goldader}, {Gonz{\'a}lez Delgado}, {Robert}, {Kune}, {de Mello}, {Devost} and {Heckman}}}}
\bibcite{lisker08}{{205}{2008}{{Lisker}}{{}}}
\bibcite{lotz11}{{206}{2011}{{{Lotz} \emph  {et~al.},}}{{{Lotz}, {Jonsson}, {Cox}, {Croton}, {Primack}, {Somerville} and {Stewart}}}}
\bibcite{lotz04}{{207}{2004}{{{Lotz} \emph  {et~al.},}}{{{Lotz}, {Primack} and {Madau}}}}
\bibcite{mackay86}{{208}{1986}{{Mackay}}{{}}}
\bibcite{madau95}{{209}{1995}{{Madau}}{{}}}
\bibcite{mancone13}{{210}{2013}{{{Mancone} \emph  {et~al.},}}{{{Mancone}, {Gonzalez}, {Moustakas} and {Price}}}}
\bibcite{maraston05}{{211}{2005}{{Maraston}}{{}}}
\bibcite{maraston10}{{212}{2010}{{{Maraston} \emph  {et~al.},}}{{{Maraston}, {Pforr}, {Renzini}, {Daddi}, {Dickinson}, {Cimatti} and {Tonini}}}}
\bibcite{marsh04}{{213}{2004}{{{Marsh} \emph  {et~al.},}}{{{Marsh}, {Young}, {Johnson} and {Smith}}}}
\bibcite{martinez10}{{214}{2010}{{{Martinez} \emph  {et~al.},}}{{{Martinez}, {Kolb}, {Tokovinin} and {Sarazin}}}}
\bibcite{masters03}{{215}{2003}{{{Masters} \emph  {et~al.},}}{{{Masters}, {Giovanelli} and {Haynes}}}}
\bibcite{mcgaugh14}{{216}{2014}{{{McGaugh} and {Schombert}}}{{}}}
\bibcite{meiksin06}{{217}{2006}{{Meiksin}}{{}}}
\bibcite{melbourne12}{{218}{2012}{{{Melbourne} \emph  {et~al.},}}{{{Melbourne}, {Williams}, {Dalcanton}, {Rosenfield}, {Girardi}, {Marigo}, {Weisz}, {Dolphin}, {Boyer}, {Olsen}, {Skillman} and {Seth}}}}
\bibcite{menanteau01}{{219}{2001}{{{Menanteau} \emph  {et~al.},}}{{{Menanteau}, {Jimenez} and {Matteucci}}}}
\bibcite{merline95}{{220}{1995}{{{Merline} and {Howell}}}{{}}}
\bibcite{milone11}{{221}{2011}{{{Milone} and {Young}}}{{}}}
\bibcite{moehler10}{{222}{2010}{{{Moehler} \emph  {et~al.},}}{{{Moehler}, {Freudling}, {M{\o }ller}, {Patat}, {Rupprecht} and {O'Brien}}}}
\bibcite{moffat69}{{223}{1969}{{Moffat}}{{}}}
\bibcite{morgan58}{{224}{1958}{{Morgan}}{{}}}
\bibcite{morgan59}{{225}{1959}{{Morgan}}{{}}}
\bibcite{morgan57}{{226}{1957}{{{Morgan} and {Mayall}}}{{}}}
\bibcite{morrissey07}{{227}{2007}{{{Morrissey} \emph  {et~al.},}}{{{Morrissey}, {Conrow}, {Barlow}, {Small}, {Seibert}, {Wyder}, {Budav{\'a}ri}, {Arnouts}, {Friedman}, {Forster}, {Martin}, {Neff}, {Schiminovich}, {Bianchi}, {Donas}, {Heckman}, {Lee}, {Madore}, {Milliard}, {Rich}, {Szalay}, {Welsh} and {Yi}}}}
\bibcite{mostardi13}{{228}{2013}{{{Mostardi} \emph  {et~al.},}}{{{Mostardi}, {Shapley}, {Nestor}, {Steidel}, {Reddy} and {Trainor}}}}
\bibcite{naim95}{{229}{1995}{{{Naim} \emph  {et~al.},}}{{{Naim}, {Lahav}, {Buta}, {Corwin}, {de Vaucouleurs}, {Dressler}, {Huchra}, {van den Bergh}, {Raychaudhury}, {Sodre} and {Storrie-Lombardi}}}}
\bibcite{nair10}{{230}{2010}{{{Nair} and {Abraham}}}{{}}}
\bibcite{neichel08}{{231}{2008}{{{Neichel} \emph  {et~al.},}}{{{Neichel}, {Fusco} and {Conan}}}}
\bibcite{newberry91}{{232}{1991}{{Newberry}}{{}}}
\bibcite{nguyen10}{{233}{2010}{{{Nguyen} \emph  {et~al.},}}{{{Nguyen}, {Schulz}, {Levenson}, {Amblard}, {Arumugam}, {Aussel}, {Babbedge}, {Blain}, {Bock}, {Boselli}, {Buat} and {Castro-Rodriguez}}}}
\bibcite{noll12}{{234}{2012}{{{Noll} \emph  {et~al.},}}{{{Noll}, {Kausch}, {Barden}, {Jones}, {Szyszka}, {Kimeswenger} and {Vinther}}}}
\bibcite{nonino09}{{235}{2009}{{{Nonino} \emph  {et~al.},}}{{{Nonino}, {Dickinson}, {Rosati}, {Grazian}, {Reddy}, {Cristiani}, {Giavalisco}, {Kuntschner}, {Vanzella}, {Daddi}, {Fosbury} and {Cesarsky}}}}
\bibcite{nordon10}{{236}{2010}{{{Nordon} \emph  {et~al.},}}{{{Nordon}, {Lutz}, {Shao}, {Magnelli}, {Berta}, {Altieri}, {Andreani}, {Aussel}, {Bongiovanni}, {Cava}, {Cepa}, {Cimatti} and {Daddi}}}}
\bibcite{odonnell94}{{237}{1994}{{O'Donnell}}{{}}}
\bibcite{oh13}{{238}{2013}{{{Oh} \emph  {et~al.},}}{{{Oh}, {Choi}, {Kim}, {Moon} and {Yi}}}}
\bibcite{osterbrock06}{{239}{2006}{{{Osterbrock} and {Ferland}}}{{}}}
\bibcite{papovich01}{{240}{2001}{{{Papovich} \emph  {et~al.},}}{{{Papovich}, {Dickinson} and {Ferguson}}}}
\bibcite{peek10}{{241}{2010}{{{Peek} and {Graves}}}{{}}}
\bibcite{peng02}{{242}{2002}{{{Peng} \emph  {et~al.},}}{{{Peng}, {Ho}, {Impey} and {Rix}}}}
\bibcite{peng10}{{243}{2010}{{{Peng} \emph  {et~al.},}}{{{Peng}, {Ho}, {Impey} and {Rix}}}}
\bibcite{pforr12}{{244}{2012}{{{Pforr} \emph  {et~al.},}}{{{Pforr}, {Maraston} and {Tonini}}}}
\bibcite{phillipps84}{{245}{1984}{{Phillipps}}{{}}}
\bibcite{pignatelli06}{{246}{2006}{{{Pignatelli} \emph  {et~al.},}}{{{Pignatelli}, {Fasano} and {Cassata}}}}
\bibcite{pirzkal12}{{247}{2012}{{{Pirzkal} \emph  {et~al.},}}{{{Pirzkal}, {Rothberg}, {Nilsson}, {Finkelstein}, {Koekemoer}, {Malhotra} and {Rhoads}}}}
\bibcite{pirzkal13}{{248}{2013}{{{Pirzkal} \emph  {et~al.},}}{{{Pirzkal}, {Rothberg}, {Ryan}, {Coe}, {Malhotra}, {Rhoads} and {Noeske}}}}
\bibcite{polletta07}{{249}{2007}{{{Polletta} \emph  {et~al.},}}{{{Polletta}, {Tajer}, {Maraschi}, {Trinchieri}, {Lonsdale}, {Chiappetti}, {Andreon}, {Pierre}, {Le F{\`e}vre}, {Zamorani} and {Maccagni}}}}
\bibcite{puech08}{{250}{2008}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Flores}, {Hammer}, {Yang}, {Neichel}, {Lehnert}, {Chemin}, {Nesvadba}, {Epinat}, {Amram}, {Balkowski}, {Cesarsky} and {Dannerbauer}}}}
\bibcite{puech09}{{251}{2009}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Hammer}, {Flores}, {Neichel} and {Yang}}}}
\bibcite{puetter05}{{252}{2005}{{{Puetter} \emph  {et~al.},}}{{{Puetter}, {Gosnell} and {Yahil}}}}
\bibcite{raiter10}{{253}{2010}{{{Raiter} \emph  {et~al.},}}{{{Raiter}, {Schaerer} and {Fosbury}}}}
\bibcite{rawat09}{{254}{2009}{{{Rawat} \emph  {et~al.},}}{{{Rawat}, {Wadadekar} and {De Mello}}}}
\bibcite{reines10}{{255}{2010}{{{Reines} \emph  {et~al.},}}{{{Reines}, {Nidever}, {Whelan} and {Johnson}}}}
\bibcite{reynolds20}{{256}{1920}{{Reynolds}}{{}}}
\bibcite{rieke07}{{257}{2007}{{Rieke}}{{}}}
\bibcite{rieke08}{{258}{2008}{{{Rieke} \emph  {et~al.},}}{{{Rieke}, {Blaylock}, {Decin}, {Engelbracht}, {Ogle}, {Avrett}, {Carpenter}, {Cutri}, {Armus}, {Gordon}, {Gray}, {Hinz}, {Su} and {Willmer}}}}
\bibcite{roberts94}{{259}{1994}{{{Roberts} and {Haynes}}}{{}}}
\bibcite{roddier81}{{260}{1981}{{Roddier}}{{}}}
\bibcite{rodrigues14}{{261}{2014}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Patricio}, {Rothberg}, {Sanchez-Janssen} and {Vale Asari}}}}
\bibcite{ryan11}{{262}{2011}{{Ryan}}{{}}}
\bibcite{sandage61}{{263}{1961}{{Sandage}}{{}}}
\bibcite{sandage05}{{264}{2005}{{Sandage}}{{}}}
\bibcite{scarlata07}{{265}{2007}{{{Scarlata} \emph  {et~al.},}}{{{Scarlata}, {Carollo}, {Lilly}, {Sargent}, {Feldmann}, {Kampczyk}, {Porciani}, {Koekemoer}, {Scoville}, {Kneib}, {Leauthaud} and {Massey}}}}
\bibcite{schade99}{{266}{1999}{{{Schade} \emph  {et~al.},}}{{{Schade}, {Lilly}, {Crampton}, {Ellis}, {Le F{\`e}vre}, {Hammer}, {Brinchmann}, {Abraham}, {Colless}, {Glazebrook}, {Tresse} and {Broadhurst}}}}
\bibcite{schade95}{{267}{1995}{{{Schade} \emph  {et~al.},}}{{{Schade}, {Lilly}, {Crampton}, {Hammer}, {Le Fevre} and {Tresse}}}}
\bibcite{schaerer13}{{268}{2013}{{Schaerer}}{{}}}
\bibcite{schaerer09}{{269}{2009}{{{Schaerer} and {de Barros}}}{{}}}
\bibcite{schechter93}{{270}{1993}{{{Schechter} \emph  {et~al.},}}{{{Schechter}, {Mateo} and {Saha}}}}
\bibcite{schlegel98}{{271}{1998}{{{Schlegel} \emph  {et~al.},}}{{{Schlegel}, {Finkbeiner} and {Davis}}}}
\bibcite{sersic68}{{272}{1968}{{Sersic}}{{}}}
\bibcite{shapley11}{{273}{2011}{{Shapley}}{{}}}
\bibcite{sheth08}{{274}{2008}{{{Sheth} \emph  {et~al.},}}{{{Sheth}, {Elmegreen}, {Elmegreen}, {Capak}, {Abraham}, {Athanassoula}, {Ellis} and {Mobasher}}}}
\bibcite{silva98}{{275}{1998}{{{Silva} \emph  {et~al.},}}{{{Silva}, {Granato}, {Bressan} and {Danese}}}}
\bibcite{simard98}{{276}{1998}{{Simard}}{{}}}
\bibcite{simard02}{{277}{2002}{{{Simard} \emph  {et~al.},}}{{{Simard}, {Willmer}, {Vogt}, {Sarajedini}, {Phillips}, {Weiner}, {Koo}, {Im}, {Illingworth} and {Faber}}}}
\bibcite{smith02}{{278}{2002}{{{Smith} \emph  {et~al.},}}{{{Smith}, {Tucker}, {Kent}, {Richmond}, {Fukugita}, {Ichikawa}, {Ichikawa}, {Jorgensen}, {Uomoto}, {Gunn}, {Hamabe} and {Watanabe}}}}
\bibcite{smolcic08}{{279}{2008}{{{Smol{\v c}i{\'c}} \emph  {et~al.},}}{{{Smol{\v c}i{\'c}}, {Schinnerer}, {Scodeggio}, {Franzetti}, {Aussel}, {Bondi}, {Brusa}, {Carilli} and {Capak}}}}
\bibcite{starck06}{{280}{2006}{{{Starck} and {Murtagh}}}{{}}}
\bibcite{starck02}{{281}{2002}{{{Starck} \emph  {et~al.},}}{{{Starck}, {Pantin} and {Murtagh}}}}
\bibcite{stark09}{{282}{2009}{{{Stark} \emph  {et~al.},}}{{{Stark}, {McGaugh} and {Swaters}}}}
\bibcite{sterken92}{{283}{1992}{{{Sterken} and {Manfroid}}}{{}}}
\bibcite{stetson87}{{284}{1987}{{Stetson}}{{}}}
\bibcite{strateva01}{{285}{2001}{{{Strateva} \emph  {et~al.},}}{{{Strateva}, {Ivezi{\'c}}, {Knapp}, {Narayanan}, {Strauss}, {Gunn}, {Lupton}, {Schlegel}, {Bahcall}, {Brinkmann}, {Brunner}, {Budav{\'a}ri} and {Csabai}}}}
\bibcite{sullivan12}{{286}{2012}{{{Sullivan} and {Simcoe}}}{{}}}
\bibcite{szalay99}{{287}{1999}{{{Szalay} \emph  {et~al.},}}{{{Szalay}, {Connolly} and {Szokoly}}}}
\bibcite{takeuchi12}{{288}{2012}{{{Takeuchi} \emph  {et~al.},}}{{{Takeuchi}, {Yuan}, {Ikeyama}, {Murata} and {Inoue}}}}
\bibcite{taylor11}{{289}{2011}{{{Taylor} \emph  {et~al.},}}{{{Taylor}, {Hopkins}, {Baldry}, {Brown}, {Driver}, {Kelvin}, {Hill}, {Robotham}, {Bland-Hawthorn}, {Jones} and {Sharp}}}}
\bibcite{taylormager07}{{290}{2007}{{{Taylor-Mager} \emph  {et~al.},}}{{{Taylor-Mager}, {Conselice}, {Windhorst} and {Jansen}}}}
\bibcite{tilvi13}{{291}{2013}{{{Tilvi} \emph  {et~al.},}}{{{Tilvi}, {Papovich}, {Tran}, {Labb{\'e}}, {Spitler}, {Straatman}, {Persson}, {Monson}, {Glazebrook}, {Quadri}, {van Dokkum}, {Ashby} and {Faber}}}}
\bibcite{tinsley72}{{292}{1972}{{Tinsley}}{{}}}
\bibcite{tinsley67}{{293}{1967}{{Tinsley}}{{}}}
\bibcite{tokovinin02}{{294}{2002}{{Tokovinin}}{{}}}
\bibcite{trujillo01}{{295}{2001}{{{Trujillo} \emph  {et~al.},}}{{{Trujillo}, {Aguerri}, {Cepa} and {Guti{\'e}rrez}}}}
\bibcite{tully98}{{296}{1998}{{{Tully} \emph  {et~al.},}}{{{Tully}, {Pierce}, {Huang}, {Saunders}, {Verheijen} and {Witchalls}}}}
\bibcite{tyson90}{{297}{1990}{{Tyson}}{{}}}
\bibcite{tyson88}{{298}{1988}{{{Tyson} and {Seitzer}}}{{}}}
\bibcite{tyson93}{{299}{1993}{{{Tyson} and {Gal}}}{{}}}
\bibcite{unterborn08}{{300}{2008}{{{Unterborn} and {Ryden}}}{{}}}
\bibcite{vaduvescu04}{{301}{2004}{{{Vaduvescu} and {McCall}}}{{}}}
\bibcite{vandenbergh60b}{{302}{1960{a}}{{van den Bergh}}{{}}}
\bibcite{vandenbergh60}{{303}{1960{b}}{{van den Bergh}}{{}}}
\bibcite{vandenbergh02}{{304}{2002}{{van den Bergh}}{{}}}
\bibcite{vandenbergh07}{{305}{2007}{{van den Bergh}}{{}}}
\bibcite{vikram10}{{306}{2010}{{{Vikram} \emph  {et~al.},}}{{{Vikram}, {Wadadekar}, {Kembhavi} and {Vijayagovindan}}}}
\bibcite{wadadekar99}{{307}{1999}{{{Wadadekar} \emph  {et~al.},}}{{{Wadadekar}, {Robbason} and {Kembhavi}}}}
\bibcite{walcher11}{{308}{2011}{{{Walcher} \emph  {et~al.},}}{{{Walcher}, {Groves}, {Budav{\'a}ri} and {Dale}}}}
\bibcite{waller90}{{309}{1990}{{Waller}}{{}}}
\bibcite{wild11}{{310}{2011}{{{Wild} \emph  {et~al.},}}{{{Wild}, {Charlot}, {Brinchmann}, {Heckman}, {Vince}, {Pacifici} and {Chevallard}}}}
\bibcite{worthey94}{{311}{1994}{{Worthey}}{{}}}
\bibcite{yan13}{{312}{2014}{{{Yan} \emph  {et~al.},}}{{{Yan}, {Stefanon}, {Ma}, {Willner}, {Somerville}, {Ashby}, {Dave}, {Perez-Gonzalez}, {Cava}, {Wiklind}, {Kocevski}, {Rafelski}, {Kartaltepe} and {Cooray}}}}
\bibcite{yoon11}{{313}{2011}{{{Yoon} \emph  {et~al.},}}{{{Yoon}, {Weinberg} and {Katz}}}}
\bibcite{zackrisson08}{{314}{2008}{{{Zackrisson} \emph  {et~al.},}}{{{Zackrisson}, {Bergvall} and {Leitet}}}}
\bibcite{zheng04}{{315}{2004}{{{Zheng} \emph  {et~al.},}}{{{Zheng}, {Hammer}, {Flores}, {Ass{\'e}mat} and {Pelat}}}}
\bibcite{zheng05}{{316}{2005}{{{Zheng} \emph  {et~al.},}}{{{Zheng}, {Hammer}, {Flores}, {Ass{\'e}mat} and {Rawat}}}}
\bibcite{zibetti09}{{317}{2009}{{{Zibetti} \emph  {et~al.},}}{{{Zibetti}, {Charlot} and {Rix}}}}
\bibcite{zibetti13}{{318}{2013}{{{Zibetti} \emph  {et~al.},}}{{{Zibetti}, {Gallazzi}, {Charlot}, {Pierini} and {Pasquali}}}}
\bibcite{zibetti11}{{319}{2011}{{{Zibetti} and {Groves}}}{{}}}
\bibstyle{ws-book-har_custMP}
\citation{Lilly1995} \citation{Hammer1997} \citation{Osterbrock1989}
\citation{2007pcim.book.....K} \citation{2012A&A...539A..61T}
\citation{2012MNRAS.421.2888R} \citation{2012A&A...539A..61T}
\citation{2012MNRAS.421.2888R} \citation{2007pcim.book.....K}
\citation{Moustakas2006} \citation{Moustakas2006} \citation{Massey2010}
\citation{2006PASP..118..270P} \citation{Liang2004a} \citation{Liang2004a}
\citation{Liang2004a} \citation{Liang2004a}
\citation{Liang2004a,Hammer2005a,Hammer2005b} \citation{Rola1994}
\citation{Fox2005} \citation{CidFerandes2005} \citation{1982PASP...94..715F}
\citation{1998SPIE.3355...36C} \citation{2012A&A...543A..92N}
\citation{2012A&A...543A..92N} \citation{1998NewAR..42..503B}
\citation{1998NewAR..42..503B} \citation{2008A&A...481..575P}
\citation{Puech2012b} \citation{Hanuschik2003} \citation{Rousselot2000}
\citation{Rodrigues2010,Rodrigues2012b} \citation{2013Msngr.151...10Y}
\citation{Glazebrook2001} \citation{Cuillandre2003} \citation{Liang2004a}
\citation{Kobulnicky2004} \citation{Liang2006a} \citation{Kobulnicky2004}
\citation{Liang2006a} \citation{Kenworthy2004} \citation{Vacca2003}
\citation{2015A&A...576A..77S} \citation{2002ApJ...569..742P}
\citation{2002ApJ...569..742P} \citation{Liang2004a} \citation{CidFerandes2005}
\citation{2008A&A...477..789Y} \citation{Rola1994} \citation{2004A&A...421..847Z}
\citation{Osterbrock1989} \citation{Stasinska2007} \citation{1999ApJ...517..148F}
\citation{Fitzpatrick1999} \citation{2000ApJ...533..682C} \citation{Cardelli1989}
\citation{Osterbrock1989} \citation{Cardelli1989} \citation{2003ApJ...594..279G}
\citation{2000ApJ...533..682C} \citation{Cardelli1989} \citation{Fitzpatrick1999}
\citation{2000ApJ...533..682C} \citation{Osterbrock1989} \citation{Cardelli1989}
\citation{2003ApJ...594..279G} \citation{2000ApJ...533..682C}
\citation{Osterbrock1989} \citation{Cardelli1989} \citation{2003ApJ...594..279G}
\citation{2000ApJ...533..682C} \citation{Osterbrock1989} \citation{Osterbrock1989}
\citation{Osterbrock1989} \citation{Kennicutt1998} \citation{2000ApJ...539..718C}
\citation{2011MNRAS.417.1760W} \citation{2009A&A...507.1793N,2011A&A...533A..93B}
\citation{2012ApJ...753...82Z} \citation{Calzetti1994}
\citation{2011MNRAS.417.1760W} \citation{Hammer2009} \citation{Stasinska2008}
\citation{Osterbrock1989} \citation{BPT1981}
\citation{2003MNRAS.346.1055K,2006MNRAS.372..961K} \citation{2013ApJ...774L..10K}
\citation{2013ApJ...774L..10K} \citation{20015A&ARodrigues} \citation{Kewley2001}
\citation{Kauffmann2003} \citation{Kauffmann2003} \citation{20015A&ARodrigues}
\citation{Kewley2001} \citation{Kauffmann2003} \citation{Kauffmann2003}
\citation{1996MNRAS.281..847T,1997ApJ...481...49H} \citation{Steidel2002}
\citation{1986ApJ...300..658F} \citation{2011ApJ...736..104J}
\citation{2011ApJ...728...38Y} \citation{McCall1985} \citation{Osterbrock1989}
\citation{2008A&A...492..371R} \citation{McCall1985} \citation{Osterbrock1989}
\citation{2008A&A...492..371R} \citation{2012ARA&A..50..531K}
\citation{2012ARA&A..50..531K} \citation{Kroupa2013} \citation{Kennicutt1992}
\citation{Kennicutt1992} \citation{Hammer1997} \citation{Jansen2001}
\citation{Ajiki2003,Atek2008} \citation{Kunth1998,Atek2008,Hayes2011}
\citation{Kornei2010,Atek2009} \citation{Kennicutt1998} \citation{salpeter55}
\citation{Atek2009} \citation{Atek2009} \citation{2004MNRAS.350..351C}
\citation{2012EAS....54.....S} \citation{2006A&A...454..103H}
\citation{Osterbrock1989} \citation{Garnett1992} \citation{2006A&A...454..103H}
\citation{1994ApJ...435..647I} \citation{Garnett1992}
\citation{2006A&A...448..955I} \citation{2007A&A...473..411L}
\citation{2004MNRAS.355.1132V} \citation{Kewley2002} \citation{Pagel1992}
\citation{Tremonti2004} \citation{Kobulnicky2004} \citation{1991ApJ...380..140M}
\citation{1986ApJ...307..431D} \citation{2011arXiv1112.3300M}
\citation{Tremonti2004} \citation{Kobulnicky2004} \citation{1991ApJ...380..140M}
\citation{1986ApJ...307..431D} \citation{2011arXiv1112.3300M}
\citation{Kobulnicky2004} \citation{Pilyugin2000,Pilyugin2005}
\citation{Alloin1979} \citation{Storchi1994} \citation{Dopita2000}
\citation{Yin2007} \citation{Kewley2008} \citation{Liang2006b,Stasinska2008}
\citation{Yin2007} \citation{Yin2007} \citation{Yin2007}
\citation{2014arXiv1405.5473S} \citation{Yin2007} \citation{2014arXiv1405.5473S}
\citation{Angel2012,2014arXiv1409.7071S} \citation{Kewley2008}
\citation{Liang2006b} \citation{Kewley2008} \citation{2012A&A...539A..61T}
\citation{2012A&A...539A..61T} \citation{Starck1997} \citation{2008Noterdaeme}
\citation{2008Noterdaeme} \citation{1998ARA&A..36..267R}
\citation{2003MNRAS.345..480P} \citation{2001AJ....122.2850B}
\citation{2001AJ....122.2850B} \citation{2005ARA&A..43..861W}
\citation{2005ARA&A..43..861W} \citation{2007A&A...474..393N}
\citation{2007A&A...474..393N} \citation{2009ARA&A..47..481A}
\citation{2014MNRAS.440..307D} \citation{2014MNRAS.440..307D}
\citation{2014MNRAS.440..307D} \citation{2014MNRAS.440..307D}
\citation{2006ApJ...650..272P} \citation{2006ApJ...650..272P}
\citation{2003Natur.423...57P,2003A&A...403...55C,2006A&A...454..151V,2007A&A...470..431D}
\citation{2006A&A...454..151V}
\citation{2001ApJ...557.1007V,2003MNRAS.345..447D,2010MNRAS.408.2071M}
\citation{2006fdg..conf..319P} \citation{Partridge1967,Schaerer2003}
\citation{2006A&A...460..397V} \citation{2006A&A...460..397V,2008A&A...480..369S}
\citation{2008A&A...480..369S} \citation{2008A&A...491...89V}
\citation{2008A&A...480..369S} \citation{2008A&A...491...89V}
\citation{Steidel1996} \citation{Pettini2001} \citation{Prochaska2010}
\citation{Prochaska2010} \citation{2010ApJ...717..289S}
\citation{2010ApJ...717..289S} \citation{2010ApJ...717..289S}
\citation{2010ApJ...717..289S} \citation{2006A&A...460..397V}
\citation{Pettini2007} \citation{Pettini2007} \citation{1899ApJ.....9..149S}
\citation{1968ApJ...151..547T} \citation{1969AJ.....74..515M}
\citation{1971ApJS...22..445S} \citation{2003MNRAS.344.1000B}
\citation{2003MNRAS.344.1000B} \citation{1976MNRAS.177...91A,1985A&A...142..411K}
\citation{1986A&A...169...71K,1986ApJ...311...45D}
\citation{2000ApJ...531..776G,1998ApJ...497..227I}
\citation{1986A&A...169...71K,1986ApJ...311...45D} \citation{1998ApJ...497..618S}
\citation{2012ApJ...759...26E,2003ApJ...588...65S,2010A&A...510A..26D}
\citation{2010A&A...514A..24H} \citation{2010A&A...514A..24H}
\citation{1973ApJ...179..731F,1984ApJ...287..586B}
\citation{1994ApJS...95..107W,2010MNRAS.404.1639V}
\citation{2004ApJ...615...98R,2006AJ....131.2755K,2009A&A...493..425M,2013A&A...549A.129C}
\citation{2003MNRAS.341...33K,2005MNRAS.362...41G,2004ApJ...613..898T}
\citation{1988A&A...195...76B,1997MNRAS.284..365P,2000A&A...357..850B,2008MNRAS.386..715T,2008ApJS..177..446G}
\citation{1994ApJS...95..107W} \citation{2010MNRAS.404.1639V}
\citation{1998ApJS..116....1T} \citation{1993PhDT.......172G,2003A&A...409..511C}
\citation{1983ApJ...273..105B} \citation{2000MNRAS.317..965H}
\citation{2004PASP..116..138C} \citation{2004ApJ...613..898T,2006A&A...448..893L}
\citation{CidFerandes2005} \citation{2006MNRAS.365...46O}
\citation{2009A&A...501.1269K} \citation{2007MNRAS.381.1252T}
\citation{2008MNRAS.385.1998K} \citation{2009MNRAS.399.1044R}
\citation{2007MNRAS.381.1252T} \citation{Hammer2009} \citation{Hammer2009}
\citation{Hammer2009}
\citation{1986A&AS...66..171B,1995A&A...303..753S,2002MNRAS.335..233P,2005ApJS..160..163S}
\citation{1993ApJ...405..538B}
\citation{2003MNRAS.344.1000B,2005MNRAS.362..799M,2009MNRAS.396..462K,2010MNRAS.404.1639V}
\citation{2009ApJ...699..486C,2010ApJ...712..833C} \citation{1999ApJS..123....3L}
\citation{2003ApJS..144...21R} \citation{2012A&A...538A.143K}
\citation{2004PASP..116..138C} \citation{2005astro.ph..9907H}
\bibdata{C3_spectro}
\bibcite{Ajiki2003}{{320}{2003}{{{Ajiki} \emph  {et~al.},}}{{{Ajiki}, {Taniguchi}, {Fujita}, {Shioya}, {Nagao}, {Murayama}, {Yamada}, {Umeda} and {Komiyama}}}}
\bibcite{1976MNRAS.177...91A}{{321}{1976}{{{Allen} \emph  {et~al.},}}{{{Allen}, {Wright} and {Goss}}}}
\bibcite{Alloin1979}{{322}{1979}{{{Alloin} \emph  {et~al.},}}{{{Alloin}, {Collin-Souffrin} and {Joly}}}}
\bibcite{2009ARA&A..47..481A}{{323}{2009}{{{Asplund} \emph  {et~al.},}}{{{Asplund}, {Grevesse}, {Sauval} and {Scott}}}}
\bibcite{Atek2008}{{324}{2008}{{{Atek} \emph  {et~al.},}}{{{Atek}, {Kunth}, {Hayes}, {{\"O}stlin} and {Mas-Hesse}}}}
\bibcite{Atek2009}{{325}{2009}{{{Atek} \emph  {et~al.},}}{{{Atek}, {Kunth}, {Schaerer}, {Hayes}, {Deharveng}, {{\"O}stlin} and {Mas-Hesse}}}}
\bibcite{BPT1981}{{326}{1981}{{{Baldwin} \emph  {et~al.},}}{{{Baldwin}, {Phillips} and {Terlevich}}}}
\bibcite{2001AJ....122.2850B}{{327}{2001}{{{Becker} \emph  {et~al.},}}{{{Becker}, {Fan}, {White}, {Strauss}, {Narayanan}, {Lupton}, {Gunn}, {Annis}, {Bahcall}, {Brinkmann}, {Connolly}, {Csabai}, {Czarapata}, {Doi}, {Heckman}, {Hennessy}, {Ivezi{\'c}}, {Knapp}, {Lamb}, {McKay}, {Munn}, {Nash}, {Nichol}, {Pier}, {Richards}, {Schneider}, {Stoughton}, {Szalay}, {Thakar} and {York}}}}
\bibcite{1998NewAR..42..503B}{{328}{1998}{{{Benn} and {Ellison}}}{{}}}
\bibcite{1988A&A...195...76B}{{329}{1988}{{Bica}}{{}}}
\bibcite{1986A&AS...66..171B}{{330}{1986}{{{Bica} and {Alloin}}}{{}}}
\bibcite{2000A&A...357..850B}{{331}{2000}{{{Boisson} \emph  {et~al.},}}{{{Boisson}, {Joly}, {Moultaka}, {Pelat} and {Serote Roos}}}}
\bibcite{2003MNRAS.344.1000B}{{332}{2003}{{{Bruzual} and {Charlot}}}{{}}}
\bibcite{1983ApJ...273..105B}{{333}{1983}{{Bruzual A.}}{{}}}
\bibcite{1993ApJ...405..538B}{{334}{1993}{{{Bruzual A.} and {Charlot}}}{{}}}
\bibcite{2011A&A...533A..93B}{{335}{2011}{{{Buat} \emph  {et~al.},}}{{{Buat}, {Giovannoli}, {Heinis}, {Charmandaris}, {Coia}, {Daddi}, {Dickinson}, {Elbaz}, {Hwang}, {Morrison}, {Dasyra}, {Aussel}, {Altieri}, {Dannerbauer}, {Kartaltepe}, {Leiton}, {Magdis}, {Magnelli} and {Popesso}}}}
\bibcite{1984ApJ...287..586B}{{336}{1984}{{{Burstein} \emph  {et~al.},}}{{{Burstein}, {Faber}, {Gaskell} and {Krumm}}}}
\bibcite{2004MNRAS.350..351C}{{337}{2004}{{{Calura} and {Matteucci}}}{{}}}
\bibcite{2000ApJ...533..682C}{{338}{2000}{{{Calzetti} \emph  {et~al.},}}{{{Calzetti}, {Armus}, {Bohlin}, {Kinney}, {Koornneef} and {Storchi-Bergmann}}}}
\bibcite{Calzetti1994}{{339}{1994}{{{Calzetti} \emph  {et~al.},}}{{{Calzetti}, {Kinney} and {Storchi-Bergmann}}}}
\bibcite{2004PASP..116..138C}{{340}{2004}{{{Cappellari} and {Emsellem}}}{{}}}
\bibcite{Cardelli1989}{{341}{1989}{{{Cardelli} \emph  {et~al.},}}{{{Cardelli}, {Clayton} and {Mathis}}}}
\bibcite{2003A&A...409..511C}{{342}{2003}{{{Cardiel} \emph  {et~al.},}}{{{Cardiel}, {Gorgas}, {S{\'a}nchez-Bl{\'a}zquez}, {Cenarro}, {Pedraz}, {Bruzual} and {Klement}}}}
\bibcite{2003A&A...403...55C}{{343}{2003}{{{Centuri{\'o}n} \emph  {et~al.},}}{{{Centuri{\'o}n}, {Molaro}, {Vladilo}, {P{\'e}roux}, {Levshakov} and {D'Odorico}}}}
\bibcite{2013A&A...549A.129C}{{344}{2013}{{{Cesetti} \emph  {et~al.},}}{{{Cesetti}, {Pizzella}, {Ivanov}, {Morelli}, {Corsini} and {Dalla Bont{\`a}}}}}
\bibcite{2000ApJ...539..718C}{{345}{2000}{{{Charlot} and {Fall}}}{{}}}
\bibcite{CidFerandes2005}{{346}{2005}{{{Cid Fernandes} \emph  {et~al.},}}{{{Cid Fernandes}, {Mateus}, {Sodr{\'e}}, {Stasi{\'n}ska} and {Gomes}}}}
\bibcite{2010ApJ...712..833C}{{347}{2010}{{{Conroy} and {Gunn}}}{{}}}
\bibcite{2009ApJ...699..486C}{{348}{2009}{{{Conroy} \emph  {et~al.},}}{{{Conroy}, {Gunn} and {White}}}}
\bibcite{1998SPIE.3355...36C}{{349}{1998}{{{Cuby} \emph  {et~al.},}}{{{Cuby}, {Bottini} and {Picat}}}}
\bibcite{Cuillandre2003}{{350}{2003}{{{Cuillandre} \emph  {et~al.},}}{{{Cuillandre}, {Fort}, {Picat} and {Soucail}}}}
\bibcite{2007A&A...470..431D}{{351}{2007}{{{Dessauges-Zavadsky} \emph  {et~al.},}}{{{Dessauges-Zavadsky}, {Calura}, {Prochaska}, {D'Odorico} and {Matteucci}}}}
\bibcite{2010A&A...510A..26D}{{352}{2010}{{{Dessauges-Zavadsky} \emph  {et~al.},}}{{{Dessauges-Zavadsky}, {D'Odorico}, {Schaerer}, {Modigliani}, {Tapken} and {Vernet}}}}
\bibcite{2003MNRAS.345..447D}{{353}{2003}{{{Dessauges-Zavadsky} \emph  {et~al.},}}{{{Dessauges-Zavadsky}, {P{\'e}roux}, {Kim}, {D'Odorico} and {McMahon}}}}
\bibcite{1986ApJ...311...45D}{{354}{1986}{{{Dinerstein} and {Shields}}}{{}}}
\bibcite{1986ApJ...307..431D}{{355}{1986}{{{Dopita} and {Evans}}}{{}}}
\bibcite{Dopita2000}{{356}{2000}{{{Dopita} \emph  {et~al.},}}{{{Dopita}, {Kewley}, {Heisler} and {Sutherland}}}}
\bibcite{2014MNRAS.440..307D}{{357}{2014}{{{Dutta} \emph  {et~al.},}}{{{Dutta}, {Srianand}, {Rahmani}, {Petitjean}, {Noterdaeme} and {Ledoux}}}}
\bibcite{2012ApJ...759...26E}{{358}{2012}{{{Erb} \emph  {et~al.},}}{{{Erb}, {Quider}, {Henry} and {Martin}}}}
\bibcite{1973ApJ...179..731F}{{359}{1973}{{Faber}}{{}}}
\bibcite{1986ApJ...300..658F}{{360}{1986}{{{Ferland} and {Osterbrock}}}{{}}}
\bibcite{1982PASP...94..715F}{{361}{1982}{{Filippenko}}{{}}}
\bibcite{Fitzpatrick1999}{{362}{1999}{{Fitzpatrick}}{{}}}
\bibcite{1999ApJ...517..148F}{{363}{1999}{{{Flores} \emph  {et~al.},}}{{{Flores}, {Hammer}, {Thuan}, {C{\'e}sarsky}, {Desert}, {Omont}, {Lilly}, {Eales}, {Crampton} and {Le F{\`e}vre}}}}
\bibcite{Fox2005}{{364}{2005}{{{Fox} \emph  {et~al.},}}{{{Fox}, {Savage} and {Wakker}}}}
\bibcite{2005MNRAS.362...41G}{{365}{2005}{{{Gallazzi} \emph  {et~al.},}}{{{Gallazzi}, {Charlot}, {Brinchmann}, {White} and {Tremonti}}}}
\bibcite{Garnett1992}{{366}{1992}{{Garnett}}{{}}}
\bibcite{Glazebrook2001}{{367}{2001}{{{Glazebrook} and {Bland-Hawthorn}}}{{}}}
\bibcite{1993PhDT.......172G}{{368}{1993}{{Gonz{\'a}lez}}{{}}}
\bibcite{2003ApJ...594..279G}{{369}{2003}{{{Gordon} \emph  {et~al.},}}{{{Gordon}, {Clayton}, {Misselt}, {Landolt} and {Wolff}}}}
\bibcite{2008ApJS..177..446G}{{370}{2008}{{{Graves} and {Schiavon}}}{{}}}
\bibcite{2000ApJ...531..776G}{{371}{2000}{{{Guseva} \emph  {et~al.},}}{{{Guseva}, {Izotov} and {Thuan}}}}
\bibcite{Hammer2005b}{{372}{2005{a}}{{Hammer}}{{}}}
\bibcite{2005astro.ph..9907H}{{373}{2005{b}}{{Hammer}}{{}}}
\bibcite{Hammer2005a}{{374}{2005}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Elbaz}, {Zheng}, {Liang} and {Cesarsky}}}}
\bibcite{1997ApJ...481...49H}{{375}{1997{a}}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Lilly}, {Crampton}, {Le F{\`e}vre}, {Rola}, {Mallen-Ornelas}, {Schade} and {Tresse}}}}
\bibcite{Hammer1997}{{376}{1997{b}}{{{Hammer} \emph  {et~al.}}}{{{Hammer}, {Flores}, {Lilly}, {Crampton}, {Le Fevre}, {Rola}, {Mallen-Ornelas}, {Schade} and {Tresse}}}}
\bibcite{2006A&A...454..103H}{{377}{2006}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Schaerer}, {Dessauges-Zavadsky}, {Le Floc'h} and {Puech}}}}
\bibcite{Hammer2009}{{378}{2009}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Yang}, {Athanassoula}, {Puech}, {Rodrigues} and {Peirani}}}}
\bibcite{2010A&A...514A..24H}{{379}{2010}{{{Han} \emph  {et~al.},}}{{{Han}, {Hammer}, {Liang}, {Flores}, {Rodrigues}, {Hou} and {Wei}}}}
\bibcite{Hanuschik2003}{{380}{2003}{{Hanuschik}}{{}}}
\bibcite{Hayes2011}{{381}{2011}{{{Hayes} \emph  {et~al.},}}{{{Hayes}, {Scarlata} and {Siana}}}}
\bibcite{2000MNRAS.317..965H}{{382}{2000}{{{Heavens} \emph  {et~al.},}}{{{Heavens}, {Jimenez} and {Lahav}}}}
\bibcite{2006A&A...448..955I}{{383}{2006}{{{Izotov} \emph  {et~al.},}}{{{Izotov}, {Stasi{\'n}ska}, {Meynet}, {Guseva} and {Thuan}}}}
\bibcite{1998ApJ...497..227I}{{384}{1998}{{{Izotov} and {Thuan}}}{{}}}
\bibcite{1994ApJ...435..647I}{{385}{1994}{{{Izotov} \emph  {et~al.},}}{{{Izotov}, {Thuan} and {Lipovetsky}}}}
\bibcite{Jansen2001}{{386}{2001}{{{Jansen} \emph  {et~al.},}}{{{Jansen}, {Franx} and {Fabricant}}}}
\bibcite{2011ApJ...736..104J}{{387}{2011}{{{Juneau} \emph  {et~al.},}}{{{Juneau}, {Dickinson}, {Alexander} and {Salim}}}}
\bibcite{2003MNRAS.346.1055K}{{388}{2003{a}}{{{Kauffmann} \emph  {et~al.},}}{{{Kauffmann}, {Heckman}, {Tremonti}, {Brinchmann}, {Charlot}, {White}, {Ridgway}, {Brinkmann}, {Fukugita}, {Hall}, {Ivezi{\'c}}, {Richards} and {Schneider}}}}
\bibcite{Kauffmann2003}{{389}{2003{b}}{{{Kauffmann} \emph  {et~al.}}}{{{Kauffmann}, {Heckman}, {Tremonti}, {Brinchmann}, {Charlot}, {White}, {Ridgway}, {Brinkmann}, {Fukugita}, {Hall}, {Ivezi{\'c}}, {Richards} and {Schneider}}}}
\bibcite{2003MNRAS.341...33K}{{390}{2003{c}}{{{Kauffmann} \emph  {et~al.},}}{{{Kauffmann}, {Heckman}, {White}, {Charlot}, {Tremonti}, {Brinchmann}, {Bruzual}, {Peng}, {Seibert}, {Bernardi}, {Blanton}, {Brinkmann}, {Castander}, {Cs{\'a}bai}, {Fukugita}, {Ivezic}, {Munn}, {Nichol}, {Padmanabhan}, {Thakar}, {Weinberg} and {York}}}}
\bibcite{2006AJ....131.2755K}{{391}{2006}{{Keel}}{{}}}
\bibcite{2012ARA&A..50..531K}{{392}{2012}{{{Kennicutt} and {Evans}}}{{}}}
\bibcite{Kennicutt1992}{{393}{1992}{{Kennicutt}}{{}}}
\bibcite{Kennicutt1998}{{394}{1998}{{Kennicutt}}{{}}}
\bibcite{Kenworthy2004}{{395}{2004}{{{Kenworthy} and {Hanson}}}{{}}}
\bibcite{Kewley2002}{{396}{2002}{{{Kewley} and {Dopita}}}{{}}}
\bibcite{Kewley2008}{{397}{2008}{{{Kewley} and {Ellison}}}{{}}}
\bibcite{2006MNRAS.372..961K}{{398}{2006}{{{Kewley} \emph  {et~al.},}}{{{Kewley}, {Groves}, {Kauffmann} and {Heckman}}}}
\bibcite{Kewley2001}{{399}{2001}{{{Kewley} \emph  {et~al.},}}{{{Kewley}, {Heisler}, {Dopita} and {Lumsden}}}}
\bibcite{2013ApJ...774L..10K}{{400}{2013}{{{Kewley} \emph  {et~al.},}}{{{Kewley}, {Maier}, {Yabe}, {Ohta}, {Akiyama}, {Dopita} and {Yuan}}}}
\bibcite{Kobulnicky2004}{{401}{2004}{{{Kobulnicky} and {Kewley}}}{{}}}
\bibcite{2009A&A...501.1269K}{{402}{2009}{{{Koleva} \emph  {et~al.},}}{{{Koleva}, {Prugniel}, {Bouchard} and {Wu}}}}
\bibcite{2008MNRAS.385.1998K}{{403}{2008}{{{Koleva} \emph  {et~al.},}}{{{Koleva}, {Prugniel}, {Ocvirk}, {Le Borgne} and {Soubiran}}}}
\bibcite{2012A&A...538A.143K}{{404}{2012}{{{Koleva} and {Vazdekis}}}{{}}}
\bibcite{Kornei2010}{{405}{2010}{{{Kornei} \emph  {et~al.},}}{{{Kornei}, {Shapley}, {Erb}, {Steidel}, {Reddy}, {Pettini} and {Bogosavljevi{\'c}}}}}
\bibcite{2009MNRAS.396..462K}{{406}{2009}{{{Kotulla} \emph  {et~al.},}}{{{Kotulla}, {Fritze}, {Weilbacher} and {Anders}}}}
\bibcite{Kroupa2013}{{407}{2013}{{{Kroupa} \emph  {et~al.},}}{{{Kroupa}, {Weidner}, {Pflamm-Altenburg}, {Thies}, {Dabringhausen}, {Marks} and {Maschberger}}}}
\bibcite{1985A&A...142..411K}{{408}{1985}{{{Kunth} and {Joubert}}}{{}}}
\bibcite{Kunth1998}{{409}{1998}{{{Kunth} \emph  {et~al.},}}{{{Kunth}, {Mas-Hesse}, {Terlevich}, {Terlevich}, {Lequeux} and {Fall}}}}
\bibcite{1986A&A...169...71K}{{410}{1986}{{{Kunth} and {Schild}}}{{}}}
\bibcite{2007pcim.book.....K}{{411}{2007}{{Kwok}}{{}}}
\bibcite{2006A&A...448..893L}{{412}{2006}{{{Lamareille} \emph  {et~al.},}}{{{Lamareille}, {Contini}, {Le Borgne}, {Brinchmann}, {Charlot} and {Richard}}}}
\bibcite{1999ApJS..123....3L}{{413}{1999}{{{Leitherer} \emph  {et~al.},}}{{{Leitherer}, {Schaerer}, {Goldader}, {Gonz{\'a}lez Delgado}, {Robert}, {Kune}, {de Mello}, {Devost} and {Heckman}}}}
\bibcite{Liang2006a}{{414}{2006{a}}{{{Liang} \emph  {et~al.},}}{{{Liang}, {Hammer} and {Flores}}}}
\bibcite{Liang2004a}{{415}{2004}{{{Liang} \emph  {et~al.},}}{{{Liang}, {Hammer}, {Flores}, {Gruel} and {Ass{\'e}mat}}}}
\bibcite{2007A&A...473..411L}{{416}{2007}{{{Liang} \emph  {et~al.},}}{{{Liang}, {Hammer}, {Yin}, {Flores}, {Rodrigues} and {Yang}}}}
\bibcite{Liang2006b}{{417}{2006{b}}{{{Liang} \emph  {et~al.},}}{{{Liang}, {Yin}, {Hammer}, {Deng}, {Flores} and {Zhang}}}}
\bibcite{Lilly1995}{{418}{1995}{{{Lilly} \emph  {et~al.,}}}{{{Lilly}, {Le Fevre}, {Crampton}, {Hammer} and {Tresse}}}}
\bibcite{Angel2012}{{419}{2012}{{{L{\'o}pez-S{\'a}nchez} \emph  {et~al.},}}{{{L{\'o}pez-S{\'a}nchez}, {Dopita}, {Kewley}, {Zahid}, {Nicholls} and {Scharw{\"a}chter}}}}
\bibcite{2005MNRAS.362..799M}{{420}{2005}{{Maraston}}{{}}}
\bibcite{2009A&A...493..425M}{{421}{2009}{{{Maraston} \emph  {et~al.},}}{{{Maraston}, {Nieves Colmen{\'a}rez}, {Bender} and {Thomas}}}}
\bibcite{Massey2010}{{422}{2010}{{{Massey} and {Hanson}}}{{}}}
\bibcite{McCall1985}{{423}{1985}{{{McCall} \emph  {et~al.},}}{{{McCall}, {Rybski} and {Shields}}}}
\bibcite{1991ApJ...380..140M}{{424}{1991}{{McGaugh}}{{}}}
\bibcite{2010MNRAS.408.2071M}{{425}{2010}{{{Milutinovic} \emph  {et~al.},}}{{{Milutinovic}, {Ellison}, {Prochaska} and {Tumlinson}}}}
\bibcite{1969AJ.....74..515M}{{426}{1969}{{{Morgan} and {Osterbrock}}}{{}}}
\bibcite{Moustakas2006}{{427}{2006}{{{Moustakas} \emph  {et~al.},}}{{{Moustakas}, {Kennicutt} and {Tremonti}}}}
\bibcite{2011arXiv1112.3300M}{{428}{2011}{{{Moustakas} \emph  {et~al.},}}{{{Moustakas}, {Zaritsky}, {Brown}, {Cool}, {Dey}, {Eisenstein}, {Gonzalez}, {Jannuzi}, {Jones}, {Kochanek}, {Murray} and {Wild}}}}
\bibcite{2009A&A...507.1793N}{{429}{2009}{{{Noll} \emph  {et~al.},}}{{{Noll}, {Burgarella}, {Giovannoli}, {Buat}, {Marcillac} and {Mu{\~n}oz-Mateos}}}}
\bibcite{2012A&A...543A..92N}{{430}{2012}{{{Noll} \emph  {et~al.},}}{{{Noll}, {Kausch}, {Barden}, {Jones}, {Szyszka}, {Kimeswenger} and {Vinther}}}}
\bibcite{2008Noterdaeme}{{431}{}{{Noterdaeme}}{{}}}
\bibcite{2007A&A...474..393N}{{432}{2007}{{{Noterdaeme} \emph  {et~al.},}}{{{Noterdaeme}, {Ledoux}, {Petitjean}, {Le Petit}, {Srianand} and {Smette}}}}
\bibcite{2006MNRAS.365...46O}{{433}{2006}{{{Ocvirk} \emph  {et~al.},}}{{{Ocvirk}, {Pichon}, {Lan{\c c}on} and {Thi{\'e}baut}}}}
\bibcite{Osterbrock1989}{{434}{1989}{{Osterbrock}}{{}}}
\bibcite{Pagel1992}{{435}{1992}{{{Pagel} \emph  {et~al.},}}{{{Pagel}, {Simonson}, {Terlevich} and {Edmunds}}}}
\bibcite{Partridge1967}{{436}{1967}{{{Partridge} and {Peebles}}}{{}}}
\bibcite{2006PASP..118..270P}{{437}{2006}{{{Pasquali} \emph  {et~al.},}}{{{Pasquali}, {Pirzkal}, {Larsen}, {Walsh} and {K{\"u}mmel}}}}
\bibcite{2008A&A...481..575P}{{438}{2008}{{Patat}}{{}}}
\bibcite{1997MNRAS.284..365P}{{439}{1997}{{Pelat}}{{}}}
\bibcite{2003MNRAS.345..480P}{{440}{2003}{{{P{\'e}roux} \emph  {et~al.},}}{{{P{\'e}roux}, {Dessauges-Zavadsky}, {D'Odorico}, {Kim} and {McMahon}}}}
\bibcite{2006fdg..conf..319P}{{441}{2006}{{Pettini}}{{}}}
\bibcite{2002ApJ...569..742P}{{442}{2002}{{{Pettini} \emph  {et~al.},}}{{{Pettini}, {Rix}, {Steidel}, {Adelberger}, {Hunt} and {Shapley}}}}
\bibcite{Pettini2001}{{443}{2001}{{{Pettini} \emph  {et~al.},}}{{{Pettini}, {Shapley}, {Steidel}, {Cuby}, {Dickinson}, {Moorwood}, {Adelberger} and {Giavalisco}}}}
\bibcite{Pettini2007}{{444}{2007}{{{Pettini} \emph  {et~al.},}}{{{Pettini}, {Steidel}, {Adelberger}, {Dickinson}, {Erb}, {Giavalisco}, {Law}, {Reddy} and {Shapley}}}}
\bibcite{2002MNRAS.335..233P}{{445}{2002}{{{Piatti} \emph  {et~al.},}}{{{Piatti}, {Bica}, {Clari{\'a}}, {Santos} and {Ahumada}}}}
\bibcite{Pilyugin2000}{{446}{2000}{{Pilyugin}}{{}}}
\bibcite{Pilyugin2005}{{447}{2005}{{{Pilyugin} and {Thuan}}}{{}}}
\bibcite{2006ApJ...650..272P}{{448}{2006}{{Prochaska}}{{}}}
\bibcite{2003Natur.423...57P}{{449}{2003}{{{Prochaska} \emph  {et~al.},}}{{{Prochaska}, {Howk} and {Wolfe}}}}
\bibcite{Prochaska2010}{{450}{2010}{{{Prochaska} and {Wolfe}}}{{}}}
\bibcite{Puech2012b}{{451}{2012}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Flores}, {Yang}, {Rodrigues}, {Gon{\c c}alves}, {Hammer} and {Disseau}}}}
\bibcite{1998ARA&A..36..267R}{{452}{1998}{{Rauch}}{{}}}
\bibcite{2009MNRAS.399.1044R}{{453}{2009}{{{Richards} \emph  {et~al.},}}{{{Richards}, {Freeman}, {Lee} and {Schafer}}}}
\bibcite{2004ApJ...615...98R}{{454}{2004}{{{Rix} \emph  {et~al.},}}{{{Rix}, {Pettini}, {Leitherer}, {Bresolin}, {Kudritzki} and {Steidel}}}}
\bibcite{2003ApJS..144...21R}{{455}{2003}{{{Robert} \emph  {et~al.},}}{{{Robert}, {Pellerin}, {Aloisi}, {Leitherer}, {Hoopes} and {Heckman}}}}
\bibcite{Rodrigues2012b}{{456}{2012{a}}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Cirasuolo}, {Hammer}, {Royer}, {Evans}, {Puech}, {Flores}, {Guinouard}, {Li Causi}, {Disseau} and {Yang}}}}
\bibcite{Rodrigues2010}{{457}{2010}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Flores}, {Puech}, {Yang} and {Royer}}}}
\bibcite{20015A&ARodrigues}{{458}{2015}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Foster}, {Taylor}, {Wright}, {Hopkins}, {Baldry}, {Brough}, {Bland-Hawthorn}, {Cluver}, {Lara-Lopez}, {Liske}, {Lopez-Sanchez} and {Pimbblet}}}}
\bibcite{2008A&A...492..371R}{{459}{2008}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Hammer}, {Flores}, {Puech}, {Liang}, {Fuentes-Carrera}, {Nesvadba}, {Lehnert}, {Yang}, {Amram}, {Balkowski}, {Cesarsky}, {Dannerbauer}, {Delgado}, {Guiderdoni}, {Kembhavi}, {Neichel}, {{\"O}stlin}, {Pozzetti}, {Ravikumar}, {Rawat}, {di Serego Alighieri}, {Vergani}, {Vernet} and {Wozniak}}}}
\bibcite{2012MNRAS.421.2888R}{{460}{2012{b}}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Puech}, {Hammer}, {Rothberg} and {Flores}}}}
\bibcite{Rola1994}{{461}{1994}{{{Rola} and {Pelat}}}{{}}}
\bibcite{Rousselot2000}{{462}{2000}{{{Rousselot} \emph  {et~al.},}}{{{Rousselot}, {Lidman}, {Cuby}, {Moreels} and {Monnet}}}}
\bibcite{salpeter55}{{463}{1955}{{Salpeter}}{{}}}
\bibcite{1995A&A...303..753S}{{464}{1995}{{{Santos} \emph  {et~al.},}}{{{Santos}, {Bica}, {Dottori}, {Ortolani} and {Barbuy}}}}
\bibcite{Schaerer2003}{{465}{2003}{{Schaerer}}{{}}}
\bibcite{1998ApJ...497..618S}{{466}{1998}{{{Schaerer} and {Vacca}}}{{}}}
\bibcite{2008A&A...480..369S}{{467}{2008}{{{Schaerer} and {Verhamme}}}{{}}}
\bibcite{1899ApJ.....9..149S}{{468}{1899}{{Scheiner}}{{}}}
\bibcite{2005ApJS..160..163S}{{469}{2005}{{{Schiavon} \emph  {et~al.},}}{{{Schiavon}, {Rose}, {Courteau} and {MacArthur}}}}
\bibcite{2014arXiv1409.7071S}{{470}{2014}{{{Shapley} \emph  {et~al.},}}{{{Shapley}, {Reddy}, {Kriek}, {Freeman}, {Sanders}, {Siana}, {Coil}, {Mobasher}, {Shivaei}, {Price} and {de Groot}}}}
\bibcite{2003ApJ...588...65S}{{471}{2003}{{{Shapley} \emph  {et~al.},}}{{{Shapley}, {Steidel}, {Pettini} and {Adelberger}}}}
\bibcite{2015A&A...576A..77S}{{472}{2015}{{{Smette} \emph  {et~al.},}}{{{Smette}, {Sana}, {Noll}, {Horst}, {Kausch}, {Kimeswenger}, {Barden}, {Szyszka}, {Jones}, {Gallenne}, {Vinther}, {Ballester} and {Taylor}}}}
\bibcite{1971ApJS...22..445S}{{473}{1971}{{{Spinrad} and {Taylor}}}{{}}}
\bibcite{Starck1997}{{474}{1997}{{{Starck} \emph  {et~al.},}}{{{Starck}, {Siebenmorgen} and {Gredel}}}}
\bibcite{Stasinska2007}{{475}{2007}{{Stasi{\'n}ska}}{{}}}
\bibcite{2012EAS....54.....S}{{476}{2012}{{{Stasi{\'n}ska} \emph  {et~al.},}}{{{Stasi{\'n}ska}, {Prantzos}, {Meynet}, {Sim{\'o}n-D{\'{\i }}az}, {Chiappini}, {Dessauges-Zavadsky}, {Charbonnel}, {Ludwig}, {Mendoza}, {Grevesse}, {Arnould}, {Barbuy}, {Lebreton}, {Decourchelle}, {Hill}, {Ferrando}, {H{\'e}brard}, {Durret}, {Katsuma} and {Zeippen}}}}
\bibcite{Stasinska2008}{{477}{2008}{{{Stasi{\'n}ska} \emph  {et~al.},}}{{{Stasi{\'n}ska}, {Vale Asari}, {Cid Fernandes}, {Gomes}, {Schlickmann}, {Mateus}, {Schoenell} and {Sodr{\'e}}}}}
\bibcite{2010ApJ...717..289S}{{478}{2010}{{{Steidel} \emph  {et~al.},}}{{{Steidel}, {Erb}, {Shapley}, {Pettini}, {Reddy}, {Bogosavljevi{\'c}}, {Rudie} and {Rakic}}}}
\bibcite{Steidel1996}{{479}{1996}{{{Steidel} \emph  {et~al.},}}{{{Steidel}, {Giavalisco}, {Dickinson} and {Adelberger}}}}
\bibcite{Steidel2002}{{480}{2002}{{{Steidel} \emph  {et~al.},}}{{{Steidel}, {Hunt}, {Shapley}, {Adelberger}, {Pettini}, {Dickinson} and {Giavalisco}}}}
\bibcite{2014arXiv1405.5473S}{{481}{2014}{{{Steidel} \emph  {et~al.},}}{{{Steidel}, {Rudie}, {Strom}, {Pettini}, {Reddy}, {Shapley}, {Trainor}, {Erb}, {Turner}, {Konidaris}, {Kulas}, {Mace}, {Matthews} and {McLean}}}}
\bibcite{Storchi1994}{{482}{1994}{{{Storchi-Bergmann} \emph  {et~al.},}}{{{Storchi-Bergmann}, {Calzetti} and {Kinney}}}}
\bibcite{2012A&A...539A..61T}{{483}{2012}{{{Talia} \emph  {et~al.},}}{{{Talia}, {Mignoli}, {Cimatti}, {Kurk}, {Berta}, {Bolzonella}, {Cassata}, {Daddi}, {Dickinson}, {Franceschini}, {Halliday}, {Pozzetti}, {Renzini}, {Rodighiero}, {Rosati} and {Zamorani}}}}
\bibcite{1968ApJ...151..547T}{{484}{1968}{{Tinsley}}{{}}}
\bibcite{2007MNRAS.381.1252T}{{485}{2007}{{{Tojeiro} \emph  {et~al.},}}{{{Tojeiro}, {Heavens}, {Jimenez} and {Panter}}}}
\bibcite{2008MNRAS.386..715T}{{486}{2008}{{{Trager} \emph  {et~al.},}}{{{Trager}, {Faber} and {Dressler}}}}
\bibcite{1998ApJS..116....1T}{{487}{1998}{{{Trager} \emph  {et~al.},}}{{{Trager}, {Worthey}, {Faber}, {Burstein} and {Gonz{\'a}lez}}}}
\bibcite{Tremonti2004}{{488}{2004{a}}{{{Tremonti} \emph  {et~al.},}}{{{Tremonti}, {Heckman}, {Kauffmann}, {Brinchmann}, {Charlot}, {White}, {Seibert}, {Peng}, {Schlegel}, {Uomoto}, {Fukugita} and {Brinkmann}}}}
\bibcite{2004ApJ...613..898T}{{489}{2004{b}}{{{Tremonti} \emph  {et~al.}}}{{{Tremonti}, {Heckman}, {Kauffmann}, {Brinchmann}, {Charlot}, {White}, {Seibert}, {Peng}, {Schlegel}, {Uomoto}, {Fukugita} and {Brinkmann}}}}
\bibcite{1996MNRAS.281..847T}{{490}{1996}{{{Tresse} \emph  {et~al.},}}{{{Tresse}, {Rola}, {Hammer}, {Stasi{\'n}ska}, {Le Fevre}, {Lilly} and {Crampton}}}}
\bibcite{Vacca2003}{{491}{2003}{{{Vacca} \emph  {et~al.},}}{{{Vacca}, {Cushing} and {Rayner}}}}
\bibcite{2010MNRAS.404.1639V}{{492}{2010}{{{Vazdekis} \emph  {et~al.},}}{{{Vazdekis}, {S{\'a}nchez-Bl{\'a}zquez}, {Falc{\'o}n-Barroso}, {Cenarro}, {Beasley}, {Cardiel}, {Gorgas} and {Peletier}}}}
\bibcite{2008A&A...491...89V}{{493}{2008}{{{Verhamme} \emph  {et~al.},}}{{{Verhamme}, {Schaerer}, {Atek} and {Tapken}}}}
\bibcite{2006A&A...460..397V}{{494}{2006}{{{Verhamme} \emph  {et~al.},}}{{{Verhamme}, {Schaerer} and {Maselli}}}}
\bibcite{2004MNRAS.355.1132V}{{495}{2004}{{{Villar-Mart{\'{\i }}n} \emph  {et~al.},}}{{{Villar-Mart{\'{\i }}n}, {Cervi{\~n}o} and {Gonz{\'a}lez Delgado}}}}
\bibcite{2001ApJ...557.1007V}{{496}{2001}{{{Vladilo} \emph  {et~al.},}}{{{Vladilo}, {Centuri{\'o}n}, {Bonifacio} and {Howk}}}}
\bibcite{2006A&A...454..151V}{{497}{2006}{{{Vladilo} \emph  {et~al.},}}{{{Vladilo}, {Centuri{\'o}n}, {Levshakov}, {P{\'e}roux}, {Khare}, {Kulkarni} and {York}}}}
\bibcite{2011MNRAS.417.1760W}{{498}{2011}{{{Wild} \emph  {et~al.},}}{{{Wild}, {Charlot}, {Brinchmann}, {Heckman}, {Vince}, {Pacifici} and {Chevallard}}}}
\bibcite{2005ARA&A..43..861W}{{499}{2005}{{{Wolfe} \emph  {et~al.},}}{{{Wolfe}, {Gawiser} and {Prochaska}}}}
\bibcite{1994ApJS...95..107W}{{500}{1994}{{Worthey}}{{}}}
\bibcite{2011ApJ...728...38Y}{{501}{2011}{{{Yan} \emph  {et~al.},}}{{{Yan}, {Ho}, {Newman}, {Coil}, {Willmer}, {Laird}, {Georgakakis}, {Aird}, {Barmby}, {Bundy}, {Cooper}, {Davis}, {Faber}, {Fang}, {Griffith}, {Koekemoer}, {Koo}, {Nandra}, {Park}, {Sarajedini}, {Weiner} and {Willner}}}}
\bibcite{2008A&A...477..789Y}{{502}{2008}{{{Yang} \emph  {et~al.},}}{{{Yang}, {Flores}, {Hammer}, {Neichel}, {Puech}, {Nesvadba}, {Rawat}, {Cesarsky}, {Lehnert}, {Pozzetti}, {Fuentes-Carrera}, {Amram}, {Balkowski}, {Dannerbauer}, {di Serego Alighieri}, {Guiderdoni}, {Kembhavi}, {Liang}, {{\"O}stlin}, {Ravikumar}, {Vergani}, {Vernet} and {Wozniak}}}}
\bibcite{2013Msngr.151...10Y}{{503}{2013}{{{Yang} \emph  {et~al.},}}{{{Yang}, {Rodrigues}, {Puech}, {Flores}, {Royer}, {Disseau}, {Gon{\c c}alves}, {Hammer}, {Cirasuolo}, {Evans}, {Li Causi}, {Maiolino} and {Melo}}}}
\bibcite{Yin2007}{{504}{2007}{{{Yin} \emph  {et~al.},}}{{{Yin}, {Liang}, {Hammer}, {Brinchmann}, {Zhang}, {Deng} and {Flores}}}}
\bibcite{2012ApJ...753...82Z}{{505}{2012}{{{Zafar} \emph  {et~al.},}}{{{Zafar}, {Watson}, {El{\'{\i }}asd{\'o}ttir}, {Fynbo}, {Kr{\"u}hler}, {Schady}, {Leloudas}, {Jakobsson}, {Th{\"o}ne}, {Perley}, {Morgan}, {Bloom} and {Greiner}}}}
\bibcite{2004A&A...421..847Z}{{506}{2004}{{{Zheng} \emph  {et~al.},}}{{{Zheng}, {Hammer}, {Flores}, {Ass{\'e}mat} and {Pelat}}}}
\bibstyle{ws-book-har_custMP}
\citation{1997ApJ...489..559G,1998ApJ...499..112B,2004AetA...421..847Z}
\citation{1997ApJ...481...49H} \citation{2012MNRAS.421.2888R}
\citation{1980PASP...92..858V} \citation{courtes82} \citation{bacon95}
\citation{afanasiev90} \citation{1938ApJ....88..113B} \citation{weitzel96}
\citation{allington06} \citation{allington06} \citation{wolf14}
\citation{1914PA.....22...19S} \citation{1976AetAS...25..527V}
\citation{1988ASPC....3...26R} \citation{2008Ealet} \citation{2008Ealet}
\citation{2014ApJ...787...38F} \citation{2014ApJ...787...38F}
\citation{2014ApJ...787...38F} \citation{2014ApJ...787...38F}
\citation{2008AetA...477..789Y} \citation{1989AJ.....97..700G}
\citation{2008AetA...477..789Y} \citation{1989AJ.....97..700G}
\citation{2010MNRAS.408.2495S} \citation{2013Msngr.151...10Y}
\citation{clare1997functional} \citation{2003MNRAS.342..345C}
\citation{Vetterling:1992:NRE:573244} \citation{Vegte:2001:FDS:516614}
\citation{2011ApJ...732L..14Y} \citation{2011ApJ...732L..14Y}
\citation{2011ApJ...732L..14Y} \citation{2006AetA...455..107F}
\citation{2006AetA...455..107F} \citation{2011AetA...535A.127V}
\citation{2011AetA...535A.127V} \citation{2011AetA...535A.127V}
\citation{2011AetA...535A.127V} \citation{2006AetA...455..131P}
\citation{2006AetA...455..131P} \citation{ISBI.2007.357020}
\citation{2011ApJ...741...69D} \citation{2008AetA...477..789Y}
\citation{2008AetA...477..789Y} \citation{2008AetA...477..789Y}
\citation{2008AetA...477..789Y} \citation{rogstad74,2010MNRAS.401.2113E}
\citation{1911MNRAS..71..460P} \citation{2007MNRAS.378...41S}
\citation{1997ApJ...489..559G} \citation{1998ApJ...499..112B}
\citation{2010AetA...509A..78D} \citation{2006MNRAS.366..787K}
\citation{2008ApJ...682..231S} \citation{2008ApJ...682..231S} \citation{rogstad74}
\citation{1973MNRAS.163..163W} \citation{1973MNRAS.163..163W}
\citation{1973MNRAS.163..163W} \citation{2006MNRAS.366..787K}
\citation{2008ApJ...682..231S} \citation{2006MNRAS.366..787K}
\citation{2006MNRAS.366..787K} \citation{1997MNRAS.292..349S}
\citation{2004ApJ...605..183W} \citation{2006MNRAS.366..787K}
\citation{2008ApJ...682..231S} \citation{2007ApJ...654..172D}
\citation{1978PhDT.......195B} \citation{2010MNRAS.402..903P}
\citation{Wisnioski15} \citation{1978PhDT.......195B} \citation{Wisnioski15}
\citation{1978PhDT.......195B} \citation{2007AJ....134..945P}
\citation{2010MNRAS.401.2113E} \citation{2008A&A...484..173P}
\citation{2010MNRAS.401.2113E} \citation{2010MNRAS.402..903P}
\citation{2010MNRAS.401.2113E} \citation{2010MNRAS.402..903P}
\citation{1978PhDT.......195B} \citation{1997AJ....114.2402C}
\citation{2006AetA...455..107F} \citation{2008AetA...477..789Y}
\citation{2008A&A...484..173P} \citation{2010AetA...510A..68P}
\citation{2010MNRAS.401.2113E} \citation{2010MNRAS.401.2113E}
\citation{2002A&A...387..821G} \citation{2002A&A...387..821G}
\citation{2008ApJ...682..231S} \citation{2008ApJ...682..231S}
\citation{2006AetA...455..107F} \citation{2008ApJ...682..231S}
\citation{2008ApJ...682..231S} \citation{2008ApJ...682..231S}
\citation{2008ApJ...682..231S} \citation{perret:tel-01059736}
\citation{2007AetA...476.1179B} \citation{2008ApJ...682..231S}
\citation{2008ApJ...682..231S} \citation{perret:tel-01059736}
\citation{2007AetA...476.1179B} \citation{2006MNRAS.366..787K}
\citation{perret:tel-01059736} \citation{2009AetA...504..789E,2010MNRAS.401.2113E}
\citation{2009ApJ...706.1364F} \citation{2006AetA...455..107F}
\citation{2006AetA...455..107F} \citation{2008AetA...477..789Y} \citation{Hung15}
\citation{2011ApJ...741...69D} \citation{2008AetA...477..789Y}
\citation{2008AetA...477..789Y} \citation{2008AetA...477..789Y}
\citation{perret:tel-01059736} \citation{2010MNRAS.401.2113E}
\citation{2009ApJ...705.1395C} \citation{2008A&A...484..173P}
\citation{2009AetA...504..789E} \citation{1990AetA...229..441B}
\citation{2006MNRAS.366..787K} \citation{2008AetA...477..789Y} \citation{Hammer09}
\citation{2008AetA...477..789Y} \citation{2006ApJ...645.1062F}
\citation{2009ApJ...697.2057L} \citation{2006ApJ...645.1062F}
\citation{2009ApJ...697.2057L} \citation{2008AetA...477..789Y} \citation{Hammer09}
\citation{2008AetA...477..789Y} \citation{2006ApJ...645.1062F}
\citation{2009ApJ...697.2057L} \citation{2006ApJ...645.1062F}
\citation{2009ApJ...697.2057L} \citation{2012AetA...542A..54B}
\citation{2009AetA...504..789E} \citation{Hung15}
\citation{1963MNRAS.126..553M,1982ac...proc..233G,2009MNRAS.396..121D}
\citation{2008ApJ...689...17H} \citation{2006MNRAS.366..787K}
\citation{Hammer09,Hung15} \citation{Hung15} \citation{2010AetA...509A..78D}
\citation{2002AetA...387..821G,2009AetA...504..789E}
\citation{2014arXiv1408.5765G} \citation{2010AetA...509A..78D}
\citation{2002AetA...387..821G,2009AetA...504..789E}
\citation{2014arXiv1408.5765G} \citation{2009AetA...496...51P}
\citation{2008A&A...484..159N} \citation{2006AetA...455..107F} \citation{Hammer09}
\citation{Hammer09}
\bibdata{C4_3Dspectro}
\bibcite{afanasiev90}{{507}{1990}{{Afanasiev}}{{}}}
\bibcite{allington06}{{508}{2006}{{Allington-Smith}}{{}}}
\bibcite{bacon95}{{509}{1995}{{{Bacon} \emph  {et~al.},}}{{{Bacon}, {Adam}, {Baranne}, {Courtes}, {Dubet}, {Dubois}, {Emsellem}, {Ferruit}, {Georgelin}, {Monnet}, {Pecontal}, {Rousset} and {Say}}}}
\bibcite{2012AetA...542A..54B}{{510}{2012}{{{Bellocchi} \emph  {et~al.},}}{{{Bellocchi}, {Arribas} and {Colina}}}}
\bibcite{1990AetA...229..441B}{{511}{1990}{{Bender}}{{}}}
\bibcite{1978PhDT.......195B}{{512}{1978}{{Bosma}}{{}}}
\bibcite{2007AetA...476.1179B}{{513}{2007}{{{Bournaud} \emph  {et~al.},}}{{{Bournaud}, {Jog} and {Combes}}}}
\bibcite{1938ApJ....88..113B}{{514}{1938}{{Bowen}}{{}}}
\bibcite{1998ApJ...499..112B}{{515}{1998}{{{Brinchmann} \emph  {et~al.},}}{{{Brinchmann}, {Abraham}, {Schade}, {Tresse}, {Ellis}, {Lilly}, {Le F{\`e}vre}, {Glazebrook}, {Hammer}, {Colless}, {Crampton} and {Broadhurst}}}}
\bibcite{2003MNRAS.342..345C}{{516}{2003}{{{Cappellari} and {Copin}}}{{}}}
\bibcite{2009ApJ...705.1395C}{{517}{2009}{{{Chemin} \emph  {et~al.},}}{{{Chemin}, {Carignan} and {Foster}}}}
\bibcite{clare1997functional}{{518}{1997}{{Clare}}{{}}}
\bibcite{1997AJ....114.2402C}{{519}{1997}{{Courteau}}{{}}}
\bibcite{courtes82}{{520}{1982}{{Courtes}}{{}}}
\bibcite{2007ApJ...654..172D}{{521}{2007}{{{Dahlen} \emph  {et~al.},}}{{{Dahlen}, {Mobasher}, {Dickinson}, {Ferguson}, {Giavalisco}, {Kretchmer} and {Ravindranath}}}}
\bibcite{2011ApJ...741...69D}{{522}{2011}{{{Davies} \emph  {et~al.},}}{{{Davies}, {F{\"o}rster Schreiber}, {Cresci}, {Genzel}, {Bouch{\'e}}, {Burkert}, {Buschkamp}, {Genel}, {Hicks}, {Kurk}, {Lutz}, {Newman}, {Shapiro}, {Sternberg}, {Tacconi} and {Wuyts}}}}
\bibcite{2010AetA...509A..78D}{{523}{2010}{{{Delgado-Serrano} \emph  {et~al.},}}{{{Delgado-Serrano}, {Hammer}, {Yang}, {Puech}, {Flores} and {Rodrigues}}}}
\bibcite{2009MNRAS.396..121D}{{524}{2009}{{Dutton}}{{}}}
\bibcite{2008Ealet}{{525}{2008}{{{Ealet} \emph  {et~al.},}}{{{Ealet}, {Prieto}, {Aumeunier}, {Cerna}, {Bonissent}, {Malina} and {Smadja}}}}
\bibcite{2010MNRAS.401.2113E}{{526}{2010}{{{Epinat} \emph  {et~al.},}}{{{Epinat}, {Amram}, {Balkowski} and {Marcelin}}}}
\bibcite{2009AetA...504..789E}{{527}{2009}{{{Epinat} \emph  {et~al.},}}{{{Epinat}, {Contini}, {Le F{\`e}vre}, {Vergani}, {Garilli}, {Amram}, {Queyrel}, {Tasca} and {Tresse}}}}
\bibcite{2006AetA...455..107F}{{528}{2006}{{{Flores} \emph  {et~al.},}}{{{Flores}, {Hammer}, {Puech}, {Amram} and {Balkowski}}}}
\bibcite{2009ApJ...706.1364F}{{529}{2009}{{{F{\"o}rster Schreiber} \emph  {et~al.},}}{{{F{\"o}rster Schreiber}, {Genzel}, {Bouch{\'e}}, {Cresci}, {Davies}, {Buschkamp}, {Shapiro}, {Tacconi}, {Hicks}, {Genel}, {Shapley}, {Erb}, {Steidel}, {Lutz}, {Eisenhauer}, {Gillessen}, {Sternberg}, {Renzini}, {Cimatti}, {Daddi}, {Kurk}, {Lilly}, {Kong}, {Lehnert}, {Nesvadba}, {Verma}, {McCracken}, {Arimoto}, {Mignoli} and {Onodera}}}}
\bibcite{2006ApJ...645.1062F}{{530}{2006}{{{F{\"o}rster Schreiber} \emph  {et~al.},}}{{{F{\"o}rster Schreiber}, {Genzel}, {Lehnert}, {Bouch{\'e}}, {Verma}, {Erb}, {Shapley}, {Steidel}, {Davies}, {Lutz}, {Nesvadba}, {Tacconi}, {Eisenhauer}, {Abuter}, {Gilbert}, {Gillessen} and {Sternberg}}}}
\bibcite{2014ApJ...787...38F}{{531}{2014}{{{F{\"o}rster Schreiber} \emph  {et~al.},}}{{{F{\"o}rster Schreiber}, {Genzel}, {Newman}, {Kurk}, {Lutz}, {Tacconi}, {Wuyts}, {Bandara}, {Burkert}, {Buschkamp}, {Carollo}, {Cresci}, {Daddi}, {Davies}, {Eisenhauer}, {Hicks}, {Lang}, {Lilly}, {Mainieri}, {Mancini}, {Naab}, {Peng}, {Renzini}, {Rosario}, {Shapiro Griffin}, {Shapley}, {Sternberg}, {Tacchella}, {Vergani}, {Wisnioski}, {Wuyts} and {Zamorani}}}}
\bibcite{1989AJ.....97..700G}{{532}{1989}{{{Gallagher} \emph  {et~al.},}}{{{Gallagher}, {Hunter} and {Bushouse}}}}
\bibcite{2014arXiv1408.5765G}{{533}{2014}{{{Garcia-Lorenzo} \emph  {et~al.},}}{{{Garcia-Lorenzo}, {Marquez}, {Barrera-Ballesteros}, {Masegosa}, {Husemann}, {Falc{\'o}n-Barroso}, {Lyubenova}, {Sanchez}, {Walcher}, {Mast}, {Garcia-Benito}, {Mendez-Abreu}, {van de Ven}, {Spekkens}, {Holmes}, {Monreal-Ibero}, {del Olmo}, {Ziegler}, {Bland-Hawthorn}, {Sanchez-Blazquez}, {Iglesias-Paramo}, {Aguerri}, {Papaderos}, {Gomes}, {Marino}, {Gonzalez Delgado}, {Cortijo-Ferrero}, {Lopez-Sanchez}, {Bekeraite}, {Wisotzki}, {Bomans} and {the CALIFA team}}}}
\bibcite{2002A&A...387..821G}{{534}{2002{a}}{{{Garrido} \emph  {et~al.},}}{{{Garrido}, {Marcelin}, {Amram} and {Boulesteix}}}}
\bibcite{2002AetA...387..821G}{{535}{2002{b}}{{{Garrido} \emph  {et~al.}}}{{{Garrido}, {Marcelin}, {Amram} and {Boulesteix}}}}
\bibcite{1982ac...proc..233G}{{536}{1982}{{Gunn}}{{}}}
\bibcite{1997ApJ...489..559G}{{537}{1997}{{{Guzm{\'a}n} \emph  {et~al.},}}{{{Guzm{\'a}n}, {Gallego}, {Koo}, {Phillips}, {Lowenthal}, {Faber}, {Illingworth} and {Vogt}}}}
\bibcite{1997ApJ...481...49H}{{538}{1997}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Lilly}, {Crampton}, {Le F{\`e}vre}, {Rola}, {Mallen-Ornelas}, {Schade} and {Tresse}}}}
\bibcite{Hammer09}{{539}{2009}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Puech}, {Yang}, {Athanassoula}, {Rodrigues} and {Delgado}}}}
\bibcite{2008ApJ...689...17H}{{540}{2008}{{{Hopkins} \emph  {et~al.},}}{{{Hopkins}, {Cox} and {Hernquist}}}}
\bibcite{Hung15}{{541}{2015}{{{Hung} \emph  {et~al.},}}{{{Hung}, {Rich}, {Yuan}, {Larson}, {Casey}, {Smith}, {Sanders}, {Kewley} and {Hayward}}}}
\bibcite{2006MNRAS.366..787K}{{542}{2006}{{{Krajnovi{\'c}} \emph  {et~al.},}}{{{Krajnovi{\'c}}, {Cappellari}, {de Zeeuw} and {Copin}}}}
\bibcite{2009ApJ...697.2057L}{{543}{2009}{{{Law} \emph  {et~al.},}}{{{Law}, {Steidel}, {Erb}, {Larkin}, {Pettini}, {Shapley} and {Wright}}}}
\bibcite{ISBI.2007.357020}{{544}{2007}{{Liang}}{{}}}
\bibcite{1963MNRAS.126..553M}{{545}{1963}{{Mestel}}{{}}}
\bibcite{2008A&A...484..159N}{{546}{2008}{{{Neichel} \emph  {et~al.},}}{{{Neichel}, {Hammer}, {Puech}, {Flores}, {Lehnert}, {Rawat}, {Yang}, {Delgado}, {Amram}, {Balkowski}, {Cesarsky}, {Dannerbauer}, {Fuentes-Carrera}, {Guiderdoni}, {Kembhavi}, {Liang}, {Nesvadba}, {{\"O}stlin}, {Pozzetti}, {Ravikumar}, {di Serego Alighieri}, {Vergani}, {Vernet} and {Wozniak}}}}
\bibcite{2009AetA...496...51P}{{547}{2009}{{{Peirani} \emph  {et~al.},}}{{{Peirani}, {Hammer}, {Flores}, {Yang} and {Athanassoula}}}}
\bibcite{perret:tel-01059736}{{548}{2014}{{Perret}}{{}}}
\bibcite{2007AJ....134..945P}{{549}{2007}{{{Pizagno} \emph  {et~al.},}}{{{Pizagno}, {Prada}, {Weinberg}, {Rix}, {Pogge}, {Grebel}, {Harbeck}, {Blanton}, {Brinkmann} and {Gunn}}}}
\bibcite{1911MNRAS..71..460P}{{550}{1911}{{Plummer}}{{}}}
\bibcite{2006AetA...455..131P}{{551}{2006}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Flores}, {Hammer} and {Lehnert}}}}
\bibcite{2008A&A...484..173P}{{552}{2008}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Flores}, {Hammer}, {Yang}, {Neichel}, {Lehnert}, {Chemin}, {Nesvadba}, {Epinat}, {Amram}, {Balkowski}, {Cesarsky}, {Dannerbauer}, {di Serego Alighieri}, {Fuentes-Carrera}, {Guiderdoni}, {Kembhavi}, {Liang}, {{\"O}stlin}, {Pozzetti}, {Ravikumar}, {Rawat}, {Vergani}, {Vernet} and {Wozniak}}}}
\bibcite{2010AetA...510A..68P}{{553}{2010{a}}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Hammer}, {Flores}, {Delgado-Serrano}, {Rodrigues} and {Yang}}}}
\bibcite{2010MNRAS.402..903P}{{554}{2010{b}}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Rosati}, {Toft}, {Cimatti}, {Neichel} and {Fusco}}}}
\bibcite{1988ASPC....3...26R}{{555}{1988}{{Ramsey}}{{}}}
\bibcite{2012MNRAS.421.2888R}{{556}{2012}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Puech}, {Hammer}, {Rothberg} and {Flores}}}}
\bibcite{rogstad74}{{557}{1974}{{{Rogstad} \emph  {et~al.},}}{{{Rogstad}, {Lockhart} and {Wright}}}}
\bibcite{2007MNRAS.378...41S}{{558}{2007}{{{Salucci} \emph  {et~al.},}}{{{Salucci}, {Lapi}, {Tonini}, {Gentile}, {Yegorova} and {Klein}}}}
\bibcite{1997MNRAS.292..349S}{{559}{1997}{{{Schoenmakers} \emph  {et~al.},}}{{{Schoenmakers}, {Franx} and {de Zeeuw}}}}
\bibcite{2008ApJ...682..231S}{{560}{2008}{{{Shapiro} \emph  {et~al.},}}{{{Shapiro}, {Genzel}, {F{\"o}rster Schreiber}, {Tacconi}, {Bouch{\'e}}, {Cresci}, {Davies}, {Eisenhauer}, {Johansson}, {Krajnovi{\'c}}, {Lutz}, {Naab}, {Arimoto}, {Arribas}, {Cimatti}, {Colina}, {Daddi}, {Daigle}, {Erb}, {Hernandez}, {Kong}, {Mignoli}, {Onodera}, {Renzini}, {Shapley} and {Steidel}}}}
\bibcite{2010MNRAS.408.2495S}{{561}{2010}{{{Sharp} and {Parkinson}}}{{}}}
\bibcite{1914PA.....22...19S}{{562}{1914}{{Slipher}}{{}}}
\bibcite{1976AetAS...25..527V}{{563}{1976}{{van der Kruit}}{{}}}
\bibcite{1980PASP...92..858V}{{564}{1980}{{Vanderriest}}{{}}}
\bibcite{Vegte:2001:FDS:516614}{{565}{2001}{{Vegte}}{{}}}
\bibcite{2011AetA...535A.127V}{{566}{2011}{{{Vergani} \emph  {et~al.},}}{{{Vergani}, {Flores}, {Covino}, {Fugazza}, {Gorosabel}, {Levan}, {Puech}, {Salvaterra}, {Tello}, {de Ugarte Postigo}, {D'Avanzo}, {D'Elia}, {Fern{\'a}ndez}, {Fynbo}, {Ghirlanda}, {Jel{\'{\i }}nek}, {Lundgren}, {Malesani}, {Palazzi}, {Piranomonte}, {Rodrigues}, {S{\'a}nchez-Ram{\'{\i }}rez}, {Terr{\'o}n}, {Th{\"o}ne}, {Antonelli}, {Campana}, {Castro-Tirado}, {Goldoni}, {Hammer}, {Hjorth}, {Jakobsson}, {Kaper}, {Melandri}, {Milvang-Jensen}, {Sollerman}, {Tagliaferri}, {Tanvir}, {Wiersema} and {Wijers}}}}
\bibcite{Vetterling:1992:NRE:573244}{{567}{1992}{{Vetterling \emph  {et~al.},}}{{Vetterling, Teukolsky and Press}}}
\bibcite{1973MNRAS.163..163W}{{568}{1973}{{{Warner} \emph  {et~al.},}}{{{Warner}, {Wright} and {Baldwin}}}}
\bibcite{weitzel96}{{569}{1996}{{{Weitzel} \emph  {et~al.},}}{{{Weitzel}, {Krabbe}, {Kroker}, {Thatte}, {Tacconi-Garman}, {Cameron} and {Genzel}}}}
\bibcite{Wisnioski15}{{570}{2015}{{{Wisnioski} \emph  {et~al.},}}{{{Wisnioski}, {F{\"o}rster Schreiber}, {Wuyts}, {Wuyts}, {Bandara}, {Wilman}, {Genzel}, {Bender}, {Davies}, {Fossati}, {Lang}, {Mendel}, {Beifiori}, {Brammer}, {Chan}, {Fabricius}, {Fudamoto}, {Kulkarni}, {Kurk}, {Lutz}, {Nelson}, {Momcheva}, {Rosario}, {Saglia}, {Seitz}, {Tacconi} and {van Dokkum}}}}
\bibcite{wolf14}{{571}{1914}{{Wolf}}{{}}}
\bibcite{2004ApJ...605..183W}{{572}{2004}{{{Wong} \emph  {et~al.},}}{{{Wong}, {Blitz} and {Bosma}}}}
\bibcite{2008AetA...477..789Y}{{573}{2008}{{{Yang} \emph  {et~al.},}}{{{Yang}, {Flores}, {Hammer}, {Neichel}, {Puech}, {Nesvadba}, {Rawat}, {Cesarsky}, {Lehnert}, {Pozzetti}, {Fuentes-Carrera}, {Amram}, {Balkowski}, {Dannerbauer}, {di Serego Alighieri}, {Guiderdoni}, {Kembhavi}, {Liang}, {{\"O}stlin}, {Ravikumar}, {Vergani}, {Vernet} and {Wozniak}}}}
\bibcite{2013Msngr.151...10Y}{{574}{2013}{{{Yang} \emph  {et~al.},}}{{{Yang}, {Rodrigues}, {Puech}, {Flores}, {Royer}, {Disseau}, {Gon{\c c}alves}, {Hammer}, {Cirasuolo}, {Evans}, {Li Causi}, {Maiolino} and {Melo}}}}
\bibcite{2011ApJ...732L..14Y}{{575}{2011}{{{Yuan} \emph  {et~al.},}}{{{Yuan}, {Kewley}, {Swinbank}, {Richard} and {Livermore}}}}
\bibcite{2004AetA...421..847Z}{{576}{2004}{{{Zheng} \emph  {et~al.},}}{{{Zheng}, {Hammer}, {Flores}, {Ass{\'e}mat} and {Pelat}}}}
\bibstyle{ws-book-har_custMP}
\citation{hammer12} \citation{delgadoserrano10} \citation{neichel08}
\citation{hammer12} \citation{hammer09,delgadoserrano10} \citation{Hammer97}
\citation{delgadoserrano10} \citation{hammer05} \citation{neichel08}
\citation{hammer09b} \citation{barnes02} \citation{barnes02} \citation{hammer09}
\citation{peirani09} \citation{puech09} \citation{kennicutt98}
\citation{fuentes10} \citation{yang09} \citation{lefevre00} \citation{rawat08}
\citation{lotz10,lotz10b} \citation{hammer09} \citation{puech12}
\citation{hopkins10a} \citation{tully77} \citation{courteau07}
\citation{eisenstein96,silk97,navarro00,portinari07,mcgaugh10,mcgaugh12}
\citation{dutton11} \citation{vogt96,vogt97,ziegler02,bohm04}
\citation{conselice05,flores06,kassin07,miller11}
\citation{flores06,puech08,cresci09,vergani12} \citation{kannappan02,hammer07}
\citation{epinat09} \citation{puech08} \citation{puech10} \citation{puech10}
\citation{pizagno07} \citation{miller11,miller12} \citation{glazebrook13}
\citation{fuentes10} \citation{conselice05,flores06}
\citation{flores06,kassin07,puech08} \citation{kannappan04} \citation{covington10}
\citation{weiner06,kassin07,puech10,vergani12} \citation{pizagno07}
\citation{puech10} \citation{puech08,cresci09,puech10,miller12,vergani12}
\citation{hammer07} \citation{verheijen01} \citation{bell01}
\citation{verheijen01} \citation{pizagno07} \citation{puech10}
\citation{gnerucci11} \citation{puech08} \citation{mcgaugh00} \citation{puech10}
\citation{vergani12} \citation{rodrigues12} \citation{dutton11}
\citation{mcgaugh05} \citation{white97} \citation{desmond12} \citation{zaritsky14}
\citation{weidner13} \citation{mcgaugh10} \citation{tremonti04}
\citation{2015MNRASRodrigues} \citation{liang06b,yin07,kewley08}
\citation{kewley08} \citation{liang06a,rodrigues08,zahid11} \citation{erb06}
\citation{maiolino08} \citation{rodrigues08} \citation{zahid11}
\citation{moustakas11} \citation{zahid13} \citation{zahid13}
\citation{tremonti04,moustakas11} \citation{moustakas11} \citation{rodrigues12}
\citation{2015MNRASRodrigues} \citation{rodrigues08} \citation{tremonti04}
\citation{bell03} \citation{zahid11} \citation{kobulnicky04} \citation{erb06}
\citation{2015MNRASRodrigues} \citation{rodrigues08} \citation{tremonti04}
\citation{bell03} \citation{zahid11} \citation{kobulnicky04} \citation{erb06}
\citation{noeske07} \citation{noeske07} \citation{noeske07} \citation{elbaz07}
\citation{elbaz07} \citation{ravikumar07} \citation{brinchmann04}
\citation{brinchmann04} \citation{renzini15} \citation{drory08} \citation{puech14}
\citation{abramson14} \citation{noeske07} \citation{rodrigues12}
\citation{puech14} \citation{drory08} \citation{scoville15} \citation{bell03}
\citation{kroupa13} \citation{bell03} \citation{kauffmann03} \citation{kroupa13}
\citation{bell03} \citation{kauffmann03} \citation{kroupa13} \citation{kroupa13}
\citation{bell03} \citation{kauffmann03} \citation{fukugita98}
\citation{fukugita04} \citation{werk14} \citation{werk14} \citation{werk14}
\citation{werk14} \citation{werk14} \citation{werk14} \citation{fukugita04}
\citation{rauch97,weinberg97,kim01} \citation{erb06}
\bibdata{C5_ws}
\bibcite{abramson14}{{577}{2014}{{{Abramson} \emph  {et~al.},}}{{{Abramson}, {Kelson}, {Dressler}, {Poggianti}, {Gladders}, {Oemler} and {Vulcani}}}}
\bibcite{barnes02}{{578}{2002}{{Barnes}}{{}}}
\bibcite{bell01}{{579}{2001}{{{Bell} and {de Jong}}}{{}}}
\bibcite{bell03}{{580}{2003}{{{Bell} \emph  {et~al.},}}{{{Bell}, {McIntosh}, {Katz} and {Weinberg}}}}
\bibcite{bohm04}{{581}{2004}{{{B{\"o}hm} \emph  {et~al.},}}{{{B{\"o}hm}, {Ziegler}, {Saglia}, {Bender}, {Fricke}, {Gabasch}, {Heidt}, {Mehlert}, {Noll} and {Seitz}}}}
\bibcite{brinchmann04}{{582}{2004}{{{Brinchmann} \emph  {et~al.},}}{{{Brinchmann}, {Charlot}, {White}, {Tremonti}, {Kauffmann}, {Heckman} and {Brinkmann}}}}
\bibcite{conselice05}{{583}{2005}{{{Conselice} \emph  {et~al.},}}{{{Conselice}, {Bundy}, {Ellis}, {Brichmann}, {Vogt} and {Phillips}}}}
\bibcite{courteau07}{{584}{2007}{{{Courteau} \emph  {et~al.},}}{{{Courteau}, {Dutton}, {van den Bosch}, {MacArthur}, {Dekel}, {McIntosh} and {Dale}}}}
\bibcite{covington10}{{585}{2010}{{{Covington} \emph  {et~al.},}}{{{Covington}, {Kassin}, {Dutton}, {Weiner}, {Cox}, {Jonsson}, {Primack}, {Faber} and {Koo}}}}
\bibcite{cresci09}{{586}{2009}{{{Cresci} \emph  {et~al.},}}{{{Cresci}, {Hicks}, {Genzel}, {Schreiber}, {Davies}, {Bouch{\'e}}, {Buschkamp}, {Genel}, {Shapiro}, {Tacconi}, {Sommer-Larsen}, {Burkert}, {Eisenhauer}, {Gerhard}, {Lutz}, {Naab}, {Sternberg}, {Cimatti}, {Daddi}, {Erb}, {Kurk}, {Lilly}, {Renzini}, {Shapley}, {Steidel} and {Caputi}}}}
\bibcite{delgadoserrano10}{{587}{2010}{{{Delgado-Serrano} \emph  {et~al.},}}{{{Delgado-Serrano}, {Hammer}, {Yang}, {Puech}, {Flores} and {Rodrigues}}}}
\bibcite{desmond12}{{588}{2012}{{Desmond}}{{}}}
\bibcite{drory08}{{589}{2008}{{{Drory} and {Alvarez}}}{{}}}
\bibcite{dutton11}{{590}{2011}{{{Dutton} \emph  {et~al.},}}{{{Dutton}, {van den Bosch}, {Faber}, {Simard}, {Kassin}, {Koo}, {Bundy}, {Huang}, {Weiner}, {Cooper}, {Newman}, {Mozena} and {Koekemoer}}}}
\bibcite{eisenstein96}{{591}{1996}{{{Eisenstein} and {Loeb}}}{{}}}
\bibcite{elbaz07}{{592}{2007}{{{Elbaz} \emph  {et~al.},}}{{{Elbaz}, {Daddi}, {Le Borgne}, {Dickinson}, {Alexander}, {Chary}, {Starck}, {Brandt}, {Kitzbichler}, {MacDonald}, {Nonino}, {Popesso}, {Stern} and {Vanzella}}}}
\bibcite{epinat09}{{593}{2009}{{{Epinat} \emph  {et~al.},}}{{{Epinat}, {Contini}, {Le F{\`e}vre}, {Vergani}, {Garilli}, {Amram}, {Queyrel}, {Tasca} and {Tresse}}}}
\bibcite{erb06}{{594}{2006}{{{Erb} \emph  {et~al.},}}{{{Erb}, {Shapley}, {Pettini}, {Steidel}, {Reddy} and {Adelberger}}}}
\bibcite{flores06}{{595}{2006}{{{Flores} \emph  {et~al.},}}{{{Flores}, {Hammer}, {Puech}, {Amram} and {Balkowski}}}}
\bibcite{fuentes10}{{596}{2010}{{{Fuentes-Carrera} \emph  {et~al.},}}{{{Fuentes-Carrera}, {Flores}, {Yang}, {Peirani}, {Hammer}, {Rodrigues} and {Balkowski}}}}
\bibcite{fukugita98}{{597}{1998}{{{Fukugita} \emph  {et~al.},}}{{{Fukugita}, {Hogan} and {Peebles}}}}
\bibcite{fukugita04}{{598}{2004}{{{Fukugita} and {Peebles}}}{{}}}
\bibcite{glazebrook13}{{599}{2013}{{Glazebrook}}{{}}}
\bibcite{gnerucci11}{{600}{2011}{{{Gnerucci} \emph  {et~al.},}}{{{Gnerucci}, {Marconi}, {Cresci}, {Maiolino}, {Mannucci}, {Calura}, {Cimatti}, {Cocchia}, {Grazian}, {Matteucci}, {Nagao}, {Pozzetti} and {Troncoso}}}}
\bibcite{hammer05}{{601}{2005}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Elbaz}, {Zheng}, {Liang} and {Cesarsky}}}}
\bibcite{Hammer97}{{602}{1997}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Lilly}, {Crampton}, {Le F{\`e}vre}, {Rola}, {Mallen-Ornelas}, {Schade} and {Tresse}}}}
\bibcite{hammer09}{{603}{2009{a}}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Puech}, {Yang}, {Athanassoula}, {Rodrigues} and {Delgado}}}}
\bibcite{hammer09b}{{604}{2009{b}}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Flores}, {Yang}, {Athanassoula}, {Puech}, {Rodrigues} and {Peirani}}}}
\bibcite{hammer07}{{605}{2007}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Puech}, {Chemin}, {Flores} and {Lehnert}}}}
\bibcite{hammer12}{{606}{2012}{{{Hammer} \emph  {et~al.},}}{{{Hammer}, {Yang}, {Flores} and {Puech}}}}
\bibcite{hopkins10a}{{607}{2010}{{{Hopkins} \emph  {et~al.},}}{{{Hopkins}, {Croton}, {Bundy}, {Khochfar}, {van den Bosch}, {Somerville}, {Wetzel}, {Keres}, {Hernquist}, {Stewart}, {Younger}, {Genel} and {Ma}}}}
\bibcite{kannappan04}{{608}{2004}{{{Kannappan} and {Barton}}}{{}}}
\bibcite{kannappan02}{{609}{2002}{{{Kannappan} \emph  {et~al.},}}{{{Kannappan}, {Fabricant} and {Franx}}}}
\bibcite{kassin07}{{610}{2007}{{{Kassin} \emph  {et~al.},}}{{{Kassin}, {Weiner}, {Faber}, {Koo}, {Lotz}, {Diemand}, {Harker}, {Bundy}, {Metevier}, {Phillips}, {Cooper}, {Croton}, {Konidaris}, {Noeske} and {Willmer}}}}
\bibcite{kauffmann03}{{611}{2003}{{{Kauffmann} \emph  {et~al.},}}{{{Kauffmann}, {Heckman}, {White}, {Charlot}, {Tremonti}, {Brinchmann}, {Bruzual}, {Peng}, {Seibert}, {Bernardi}, {Blanton}, {Brinkmann}, {Castander}, {Cs{\'a}bai}, {Fukugita}, {Ivezic}, {Munn}, {Nichol}, {Padmanabhan}, {Thakar}, {Weinberg} and {York}}}}
\bibcite{kennicutt98}{{612}{1998}{{Kennicutt}}{{}}}
\bibcite{kewley08}{{613}{2008}{{{Kewley} and {Ellison}}}{{}}}
\bibcite{kim01}{{614}{2001}{{{Kim} \emph  {et~al.},}}{{{Kim}, {Cristiani} and {D'Odorico}}}}
\bibcite{kobulnicky04}{{615}{2004}{{{Kobulnicky} and {Kewley}}}{{}}}
\bibcite{kroupa13}{{616}{2013}{{{Kroupa} \emph  {et~al.},}}{{{Kroupa}, {Weidner}, {Pflamm-Altenburg}, {Thies}, {Dabringhausen}, {Marks} and {Maschberger}}}}
\bibcite{lefevre00}{{617}{2000}{{{Le F{\`e}vre} \emph  {et~al.},}}{{{Le F{\`e}vre}, {Abraham}, {Lilly}, {Ellis}, {Brinchmann}, {Schade}, {Tresse}, {Colless}, {Crampton}, {Glazebrook}, {Hammer} and {Broadhurst}}}}
\bibcite{liang06a}{{618}{2006{a}}{{{Liang} \emph  {et~al.},}}{{{Liang}, {Hammer} and {Flores}}}}
\bibcite{liang06b}{{619}{2006{b}}{{{Liang} \emph  {et~al.},}}{{{Liang}, {Yin}, {Hammer}, {Deng}, {Flores} and {Zhang}}}}
\bibcite{lotz10}{{620}{2010{a}}{{{Lotz} \emph  {et~al.},}}{{{Lotz}, {Jonsson}, {Cox} and {Primack}}}}
\bibcite{lotz10b}{{621}{2010{b}}{{{Lotz} \emph  {et~al.},}}{{{Lotz}, {Jonsson}, {Cox} and {Primack}}}}
\bibcite{maiolino08}{{622}{2008}{{{Maiolino} \emph  {et~al.},}}{{{Maiolino}, {Nagao}, {Grazian}, {Cocchia}, {Marconi}, {Mannucci}, {Cimatti}, {Pipino}, {Ballero}, {Calura}, {Chiappini}, {Fontana}, {Granato}, {Matteucci}, {Pastorini}, {Pentericci}, {Risaliti}, {Salvati} and {Silva}}}}
\bibcite{mcgaugh05}{{623}{2005}{{McGaugh}}{{}}}
\bibcite{mcgaugh12}{{624}{2012}{{McGaugh}}{{}}}
\bibcite{mcgaugh00}{{625}{2000}{{{McGaugh} \emph  {et~al.},}}{{{McGaugh}, {Schombert}, {Bothun} and {de Blok}}}}
\bibcite{mcgaugh10}{{626}{2010}{{{McGaugh} \emph  {et~al.},}}{{{McGaugh}, {Schombert}, {de Blok} and {Zagursky}}}}
\bibcite{miller11}{{627}{2011}{{{Miller} \emph  {et~al.},}}{{{Miller}, {Bundy}, {Sullivan}, {Ellis} and {Treu}}}}
\bibcite{miller12}{{628}{2012}{{{Miller} \emph  {et~al.},}}{{{Miller}, {Ellis}, {Sullivan}, {Bundy}, {Newman} and {Treu}}}}
\bibcite{moustakas11}{{629}{2011}{{{Moustakas} \emph  {et~al.},}}{{{Moustakas}, {Zaritsky}, {Brown}, {Cool}, {Dey}, {Eisenstein}, {Gonzalez}, {Jannuzi}, {Jones}, {Kochanek}, {Murray} and {Wild}}}}
\bibcite{navarro00}{{630}{2000}{{{Navarro} and {Steinmetz}}}{{}}}
\bibcite{neichel08}{{631}{2008}{{{Neichel} \emph  {et~al.},}}{{{Neichel}, {Hammer}, {Puech}, {Flores}, {Lehnert}, {Rawat}, {Yang}, {Delgado}, {Amram}, {Balkowski}, {Cesarsky}, {Dannerbauer}, {Fuentes-Carrera}, {Guiderdoni}, {Kembhavi}, {Liang}, {Nesvadba}, {{\"O}stlin}, {Pozzetti}, {Ravikumar}, {di Serego Alighieri}, {Vergani}, {Vernet} and {Wozniak}}}}
\bibcite{noeske07}{{632}{2007}{{{Noeske} \emph  {et~al.},}}{{{Noeske}, {Weiner}, {Faber}, {Papovich}, {Koo}, {Somerville}, {Bundy}, {Conselice}, {Newman}, {Schiminovich}, {Le Floc'h}, {Coil}, {Rieke}, {Lotz}, {Primack}, {Barmby}, {Cooper}, {Davis}, {Ellis}, {Fazio}, {Guhathakurta}, {Huang}, {Kassin}, {Martin}, {Phillips}, {Rich}, {Small}, {Willmer} and {Wilson}}}}
\bibcite{peirani09}{{633}{2009}{{{Peirani} \emph  {et~al.},}}{{{Peirani}, {Hammer}, {Flores}, {Yang} and {Athanassoula}}}}
\bibcite{pizagno07}{{634}{2007}{{{Pizagno} \emph  {et~al.},}}{{{Pizagno}, {Prada}, {Weinberg}, {Rix}, {Pogge}, {Grebel}, {Harbeck}, {Blanton}, {Brinkmann} and {Gunn}}}}
\bibcite{portinari07}{{635}{2007}{{{Portinari} and {Sommer-Larsen}}}{{}}}
\bibcite{puech08}{{636}{2008}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Flores}, {Hammer}, {Yang}, {Neichel}, {Lehnert}, {Chemin}, {Nesvadba}, {Epinat}, {Amram}, {Balkowski}, {Cesarsky}, {Dannerbauer}, {di Serego Alighieri}, {Fuentes-Carrera}, {Guiderdoni}, {Kembhavi}, {Liang}, {{\"O}stlin}, {Pozzetti}, {Ravikumar}, {Rawat}, {Vergani}, {Vernet} and {Wozniak}}}}
\bibcite{puech10}{{637}{2010}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Hammer}, {Flores}, {Delgado-Serrano}, {Rodrigues} and {Yang}}}}
\bibcite{puech09}{{638}{2009}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Hammer}, {Flores}, {Neichel} and {Yang}}}}
\bibcite{puech12}{{639}{2012}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Hammer}, {Hopkins}, {Athanassoula}, {Flores}, {Rodrigues}, {Wang} and {Yang}}}}
\bibcite{puech14}{{640}{2014}{{{Puech} \emph  {et~al.},}}{{{Puech}, {Hammer}, {Rodrigues}, {Fouquet}, {Flores} and {Disseau}}}}
\bibcite{rauch97}{{641}{1997}{{{Rauch} \emph  {et~al.},}}{{{Rauch}, {Miralda-Escud{\'e}}, {Sargent}, {Barlow}, {Weinberg}, {Hernquist}, {Katz}, {Cen} and {Ostriker}}}}
\bibcite{ravikumar07}{{642}{2007}{{{Ravikumar} \emph  {et~al.},}}{{{Ravikumar}, {Puech}, {Flores}, {Proust}, {Hammer}, {Lehnert}, {Rawat}, {Amram}, {Balkowski}, {Burgarella}, {Cassata}, {Cesarsky}, {Cimatti}, {Combes}, {Daddi}, {Dannerbauer}, {di Serego Alighieri}, {Elbaz}, {Guiderdoni}, {Kembhavi}, {Liang}, {Pozzetti}, {Vergani}, {Vernet}, {Wozniak} and {Zheng}}}}
\bibcite{rawat08}{{643}{2008}{{{Rawat} \emph  {et~al.},}}{{{Rawat}, {Hammer}, {Kembhavi} and {Flores}}}}
\bibcite{renzini15}{{644}{2015}{{{Renzini} and {Peng}}}{{}}}
\bibcite{2015MNRASRodrigues}{{645}{2015}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Hammer}, {Flores} and {Puech}}}}
\bibcite{rodrigues08}{{646}{2008}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Hammer}, {Flores}, {Puech}, {Liang}, {Fuentes-Carrera}, {Nesvadba}, {Lehnert}, {Yang}, {Amram}, {Balkowski}, {Cesarsky}, {Dannerbauer}, {Delgado}, {Guiderdoni}, {Kembhavi}, {Neichel}, {{\"O}stlin}, {Pozzetti}, {Ravikumar}, {Rawat}, {di Serego Alighieri}, {Vergani}, {Vernet} and {Wozniak}}}}
\bibcite{rodrigues12}{{647}{2012}{{{Rodrigues} \emph  {et~al.},}}{{{Rodrigues}, {Puech}, {Hammer}, {Rothberg} and {Flores}}}}
\bibcite{scoville15}{{648}{2015}{{{Scoville} \emph  {et~al.},}}{{{Scoville}, {Sheth}, {Aussel}, {Vanden Bout}, {Capak}, {Bongiorno}, {Casey}, {Murchikova}, {Koda}, {Pope}, {Toft}, {Ivison}, {Sanders}, {Manohar} and {Lee}}}}
\bibcite{silk97}{{649}{1997}{{Silk}}{{}}}
\bibcite{tremonti04}{{650}{2004}{{{Tremonti} \emph  {et~al.},}}{{{Tremonti}, {Heckman}, {Kauffmann}, {Brinchmann}, {Charlot}, {White}, {Seibert}, {Peng}, {Schlegel}, {Uomoto}, {Fukugita} and {Brinkmann}}}}
\bibcite{tully77}{{651}{1977}{{{Tully} and {Fisher}}}{{}}}
\bibcite{vergani12}{{652}{2012}{{{Vergani} \emph  {et~al.},}}{{{Vergani}, {Epinat}, {Contini}, {Tasca}, {Tresse}, {Amram}, {Garilli}, {Kissler-Patig}, {Le F{\`e}vre}, {Moultaka}, {Paioro}, {Queyrel} and {L{\'o}pez-Sanjuan}}}}
\bibcite{verheijen01}{{653}{2001}{{Verheijen}}{{}}}
\bibcite{vogt96}{{654}{1996}{{{Vogt} \emph  {et~al.},}}{{{Vogt}, {Forbes}, {Phillips}, {Gronwall}, {Faber}, {Illingworth} and {Koo}}}}
\bibcite{vogt97}{{655}{1997}{{{Vogt} \emph  {et~al.},}}{{{Vogt}, {Phillips}, {Faber}, {Gallego}, {Gronwall}, {Guzm{\'a}n}, {Illingworth}, {Koo} and {Lowenthal}}}}
\bibcite{weidner13}{{656}{2013}{{{Weidner} \emph  {et~al.},}}{{{Weidner}, {Kroupa}, {Pflamm-Altenburg} and {Vazdekis}}}}
\bibcite{weinberg97}{{657}{1997}{{{Weinberg} \emph  {et~al.},}}{{{Weinberg}, {Miralda-Escud{\'e}}, {Hernquist} and {Katz}}}}
\bibcite{weiner06}{{658}{2006}{{{Weiner} \emph  {et~al.},}}{{{Weiner}, {Willmer}, {Faber}, {Harker}, {Kassin}, {Phillips}, {Melbourne}, {Metevier}, {Vogt} and {Koo}}}}
\bibcite{werk14}{{659}{2014}{{{Werk} \emph  {et~al.},}}{{{Werk}, {Prochaska}, {Tumlinson}, {Peeples}, {Tripp}, {Fox}, {Lehner}, {Thom}, {O'Meara}, {Ford}, {Bordoloi}, {Katz}, {Tejos}, {Oppenheimer}, {Dav{\'e}} and {Weinberg}}}}
\bibcite{white97}{{660}{1997}{{White}}{{}}}
\bibcite{yang09}{{661}{2009}{{{Yang} \emph  {et~al.},}}{{{Yang}, {Hammer}, {Flores}, {Puech} and {Rodrigues}}}}
\bibcite{yin07}{{662}{2007}{{{Yin} \emph  {et~al.},}}{{{Yin}, {Liang}, {Hammer}, {Brinchmann}, {Zhang}, {Deng} and {Flores}}}}
\bibcite{zahid13}{{663}{2013}{{{Zahid} \emph  {et~al.},}}{{{Zahid}, {Geller}, {Kewley}, {Hwang}, {Fabricant} and {Kurtz}}}}
\bibcite{zahid11}{{664}{2011}{{{Zahid} \emph  {et~al.},}}{{{Zahid}, {Kewley} and {Bresolin}}}}
\bibcite{zaritsky14}{{665}{2014}{{{Zaritsky} \emph  {et~al.},}}{{{Zaritsky}, {Courtois}, {Mu{\~n}oz-Mateos}, {Sorce}, {Erroz-Ferrer}, {Comer{\'o}n}, {Gadotti}, {Gil de Paz}, {Hinz}, {Laurikainen}, {Kim}, {Laine}, {Men{\'e}ndez-Delmestre}, {Mizusawa}, {Regan}, {Salo}, {Seibert}, {Sheth}, {Athanassoula}, {Bosma}, {Cisternas}, {Ho} and {Holwerda}}}}
\bibcite{ziegler02}{{666}{2002}{{{Ziegler} \emph  {et~al.},}}{{{Ziegler}, {B{\"o}hm}, {Fricke}, {J{\"a}ger}, {Nicklas}, {Bender}, {Drory}, {Gabasch}, {Saglia}, {Seitz}, {Heidt}, {Mehlert}, {M{\"o}llenhoff}, {Noll} and {Sutorius}}}}


==> epsfsafe.tex <==
%   EPSF.TEX macro file (modified for EPSF images with TIFF preview)
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%   Revised by Don Knuth, 3 Jan 1990.
%   Revised by Tomas Rokicki to accept bounding boxes with no
%	space after the colon, 18 Jul 1990.
%-%   Modified to deal with %%BoundingBox: (at end) as well as TIFF 
%-%	preview in EPSF format files, 1993 Jan 23 (see %-% comments).
%
%   TeX macros to include an Encapsulated PostScript graphic.
%   Works by finding the bounding box comment,
%   calculating the correct scale values, and inserting a vbox
%   of the appropriate size at the current position in the TeX document.
%
%   To use with the center environment of LaTeX, preface the \epsffile
%   call with a \leavevmode.  (LaTeX should probably supply this itself
%   for the center environment.)
%
%   To use, simply say
%   \input epsfsafe	  % somewhere early on in your TeX file
%   \epsfbox{filename.ps} % where you want to insert a vbox for a figure
%
%   Alternatively, you can type
%
%   \epsfbox[0 0 30 50]{filename.ps} % to supply your own BB
%
%   which will not read in the file, and will instead use the bounding
%   box you specify.
%
%   The effect will be to typeset the figure as a TeX box, at the
%   point of your \epsfbox command. By default, the graphic will have its
%   `natural' width (namely the width of its bounding box, as described
%   in filename.ps). The TeX box will have depth zero.
%
%   You can enlarge or reduce the figure by saying
%     \epsfxsize=<dimen> \epsfbox{filename.ps}
%   (or
%     \epsfysize=<dimen> \epsfbox{filename.ps})
%   instead. Then the width of the TeX box will be \epsfxsize and its
%   height will be scaled proportionately (or the height will be
%   \epsfysize and its width will be scaled proportiontally).  The
%   width (and height) is restored to zero after each use.
%
%   A more general facility for sizing is available by defining the
%   \epsfsize macro.  Normally you can redefine this macro
%   to do almost anything.  The first parameter is the natural x size of
%   the PostScript graphic, the second parameter is the natural y size
%   of the PostScript graphic.  It must return the xsize to use, or 0 if
%   natural scaling is to be used.  Common uses include:
%
%      \epsfxsize  % just leave the old value alone
%      0pt	   % use the natural sizes
%      #1	   % use the natural sizes
%      \hsize	   % scale to full width
%      0.5#1	   % scale to 50% of natural size
%      \ifnum#1>\hsize\hsize\else#1\fi	% smaller of natural, hsize
%
%   If you want TeX to report the size of the figure (as a message
%   on your terminal when it processes each figure), say `\epsfverbosetrue'.
%
\chardef\quoteleftcode=\catcode96	% remember catcode of `
\catcode96=12				% make sure ` is "ordinary"

\newread\epsffilein    % file to \read
\newif\ifepsffileok    % continue looking for the bounding box?
\newif\ifepsfbbfound   % success?
\newif\ifepsfverbose   % report what you're making?
\newdimen\epsfxsize    % horizontal size after scaling
\newdimen\epsfysize    % vertical size after scaling
\newdimen\epsftsize    % horizontal size before scaling
\newdimen\epsfrsize    % vertical size before scaling
\newdimen\epsftmp      % register for arithmetic manipulation
\newdimen\pspoints     % conversion factor
%
\pspoints=1bp	       % Adobe points are `big'
\epsfxsize=0pt	       % Default value, means `use natural size'
\epsfysize=0pt	       % ditto
%
\def\epsfbox#1{\global\def\epsfllx{72}\global\def\epsflly{72}%
   \global\def\epsfurx{540}\global\def\epsfury{720}%
   \def\lbracket{[}\def\testit{#1}\ifx\testit\lbracket
   \let\next=\epsfgetlitbb\else\let\next=\epsfnormal\fi\next{#1}}%
%
\def\epsfgetlitbb#1#2 #3 #4 #5]#6{\epsfgrab #2 #3 #4 #5 .\\%
   \epsfsetgraph{#6}}%
%
\def\epsfnormal#1{\epsfgetbb{#1}\epsfsetgraph{#1}}%
%
\def\epsfgetbb#1{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\epsffilein=#1
\ifeof\epsffilein\errmessage{I couldn't open #1, will ignore it}\else
%
%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%   start with %. We're looking for the bounding box comment.
%
   {\epsffileoktrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
%-% Neuter some more nasty characters
    \catcode`\^^L=9 \catcode`\^^?=9
    \loop
       \read\epsffilein to \epsffileline
       \ifeof\epsffilein\epsffileokfalse\else
%
%   We check to see if the first character is a % sign;
%   if not, we stop reading (unless the line was entirely blank);
%   if so, we look further and stop only if the line begins with
%   `%%BoundingBox:'.
%
	  \expandafter\epsfaux\epsffileline:. \\%
       \fi
   \ifepsffileok\repeat
   \ifepsfbbfound\else
    \ifepsfverbose\message{No bounding box comment in #1; using defaults}\fi\fi
   }\closein\epsffilein\fi}%
%
%   Now we have to calculate the scale and offset values to use.
%   First we compute the natural sizes.
%
\def\epsfclipstring{}% do we clip or not?  If so,
\def\epsfclipon{\def\epsfclipstring{ clip}}%
\def\epsfclipoff{\def\epsfclipstring{}}%
%
\def\epsfsetgraph#1{%
   \epsfrsize=\epsfury\pspoints
   \advance\epsfrsize by-\epsflly\pspoints
   \epsftsize=\epsfurx\pspoints
   \advance\epsftsize by-\epsfllx\pspoints
%
%   If `epsfxsize' is 0, we default to the natural size of the picture.
%   Otherwise we scale the graph to be \epsfxsize wide.
%
   \epsfxsize\epsfsize\epsftsize\epsfrsize
   \ifnum\epsfxsize=0 \ifnum\epsfysize=0
      \epsfxsize=\epsftsize \epsfysize=\epsfrsize
      \epsfrsize=0pt
%
%   We have a sticky problem here:  TeX doesn't do floating point arithmetic!
%   Our goal is to compute y = rx/t. The following loop does this reasonably
%   fast, with an error of at most about 16 sp (about 1/4000 pt).
%
     \else\epsftmp=\epsftsize \divide\epsftmp\epsfrsize
       \epsfxsize=\epsfysize \multiply\epsfxsize\epsftmp
       \multiply\epsftmp\epsfrsize \advance\epsftsize-\epsftmp
       \epsftmp=\epsfysize
       \loop \advance\epsftsize\epsftsize \divide\epsftmp 2
       \ifnum\epsftmp>0
          \ifnum\epsftsize<\epsfrsize\else
	     \advance\epsftsize-\epsfrsize \advance\epsfxsize\epsftmp \fi
       \repeat
       \epsfrsize=0pt
     \fi
   \else \ifnum\epsfysize=0
     \epsftmp=\epsfrsize \divide\epsftmp\epsftsize
     \epsfysize=\epsfxsize \multiply\epsfysize\epsftmp
     \multiply\epsftmp\epsftsize \advance\epsfrsize-\epsftmp
     \epsftmp=\epsfxsize
     \loop \advance\epsfrsize\epsfrsize \divide\epsftmp 2
     \ifnum\epsftmp>0
	\ifnum\epsfrsize<\epsftsize\else
	   \advance\epsfrsize-\epsftsize \advance\epsfysize\epsftmp \fi
     \repeat
     \epsfrsize=0pt
    \else
     \epsfrsize=\epsfysize
    \fi
   \fi
%
%  Finally, we make the vbox and stick in a \special that dvips can parse.
%
   \ifepsfverbose\message{#1: width=\the\epsfxsize, height=\the\epsfysize}\fi
   \epsftmp=10\epsfxsize \divide\epsftmp\pspoints
   \vbox to\epsfysize{\vfil\hbox to\epsfxsize{%
      \ifnum\epsfrsize=0\relax
        \special{PSfile=#1 llx=\epsfllx\space lly=\epsflly\space
            urx=\epsfurx\space ury=\epsfury\space rwi=\number\epsftmp
            \epsfclipstring}%
      \else
        \epsfrsize=10\epsfysize \divide\epsfrsize\pspoints
        \special{PSfile=#1 llx=\epsfllx\space lly=\epsflly\space
            urx=\epsfurx\space ury=\epsfury\space rwi=\number\epsftmp\space
            rhi=\number\epsfrsize \epsfclipstring}%
      \fi
      \hfil}}%
\global\epsfxsize=0pt\global\epsfysize=0pt}%
%
%   We still need to define the tricky \epsfaux macro. This requires
%   a couple of magic constants for comparison purposes.
%
{\catcode`\%=12 \global\let\epsfpercent=%\global\def\epsfbblit{%BoundingBox}}%
%
%   So we're ready to check for `%BoundingBox:' and to grab the
%   values if they are found.
%
\long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
   \def\testit{#2}\ifx\testit\epsfbblit
      \epsfgrab #3 . . . \\%
      \epsffileokfalse
      \global\epsfbbfoundtrue
%-% Don't stop if line does not start with %.  May be (at end) or binary stuff
%  \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%
   \fi\else\ifx#1\par\else\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\epsfempty{}%
\def\epsfgrab #1 #2 #3 #4 #5\\{%
\global\def\epsfllx{#1}\ifx\epsfllx\epsfempty
      \epsfgrab #2 #3 #4 #5 .\\\else
   \global\def\epsflly{#2}%
   \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%
%
%   We default the epsfsize macro.
%
\def\epsfsize#1#2{\epsfxsize}
%
%   Finally, another definition for compatibility with older macros.
%
\let\epsffile=\epsfbox

\catcode`\`=\quoteleftcode		% restore previous catcode
